Analytical Modeling of Nonlinear Fiber Propagation for Four Dimensional Symmetric Constellations

Coherent optical transmission systems naturally lead to a four dimensional (4D) signal space, i.e., two polarizations each with two quadratures. In this paper we derive an analytical model to quantify the impact of Kerr nonlinearity on such 4Dspaces, taking the interpolarization dependency into account. This is in contrast to previous models such as the GN and EGN models, which are valid for polarization multiplexed (PM)formats, where the two polarizations are seen as independent channels on which data is multiplexed. The proposed model agrees with the EGN model in the special case of independent two-dimensional modulation in each polarization. The model accounts for the predominant nonlinear terms in a WDM system, namely self-phase modulation and and cross-phase modulation. Numerical results show that the EGN model may inaccurately estimate the nonlinear interference of 4D formats. This nonlinear interference discrepancy between the results of the proposed model and the EGN model could be up to 2.8 dB for a system with 80 WDM channels. The derived model is validated by split-step Fourier simulations, and it is shown to follow simulations very closely.

==> Interpretation.tex <==
\section{Interpretation of key result and comparison with previous models}\label{interpretation}

The NLI PSD of channel $\kappa$ is computed (see \eqref{NLI_Power_Channel_Kappa}), by taking expectation of the product of the nonlinear electrical field of channel $\kappa$, i. e., $E_{\text{NLI,x},\kappa}$, and its complex conjugate, summed with the corresponding result for polarization y. The 3 spectral components $mf_0$, $nf_0$, and $kf_0$ of $E_{\text{NLI,x},\kappa}$ (see \eqref{NLI_elec_tot_detail}) in the limit of large signal period, i.e.,  ${f_0\rightarrow0}$, tend to three continuous frequencies of $f_1$,  $f_3-lR$, and $f_2$, resp, where $f_3=f_1+f_2-f$. %located in channels $\kappa_1$, $\kappa_2$, and $\kappa_1+\kappa_2-\kappa+l$, respectively. 
%Moreover, the summation over indices $i$, $m$, $n$, and $k$ will be replaced by integral with variables $f$, $f_1$, $f_2$, and $f_3$, respectively. 
These three $f_1$, $f_2$, and $f_3$ spectral components of the nonlinear electrical field interact and produce an interfering harmonic at frequency $f$, located in the COI. 
We now proceed with  interpretation of the different NLI terms introduced in \eqref{EGN_fixed} exploiting the same taxonomy used in \cite{Poggiolini2012,Pontus_JLT_modeling_2013}. Considering $G_{\text{NLI},\kappa}=\mathbb{E}\{E_{\text{NLI,x},\kappa}E^{*}_{\text{NLI,x},\kappa}\}$, the NLI PSD of the COI is computed by averaging over the product of a set of six spectral components, consisting of $f_1$, $f_2$, and $f_3$ %(shown on the vertical, horizontal, and diagonal axes, respectively) 
from the nonlinear electrical field, i. e., $E_{\text{NLI,x},\kappa}$, and $f'_1$, $f'_2$, and $f'_3$ from its complex conjugate, 
%(similarly shown on the vertical, horizontal, and diagonal axes, respectively)
 interacting to produce the nonlinear PSD spectral lines.
 
 We can compute all the NLI contributions on COI by means of \eqref{EGN_fixed}. The triple summation in this equation represents the integration regions with $(\kappa_1,\kappa_2,\kappa_1+\kappa_2-\kappa+l)$ coordinate, implying that the frequency pairs $(f_1,f_1')$, $(f_2,f_2')$, and $(f_3,f_3')$ are located in $\kappa_1$, $\kappa_2$, and $\tilde{\kappa}=\kappa_1+\kappa_2-\kappa+l$, resp. %These interfering frequencies can be located in different WDM channels, resulting in $D_\kappa$, $E_\kappa$, $F_\kappa$, $G_\kappa$, and $H_\kappa$ terms of \eqref{EGN_fixed}, which are triple, fourth-fold, fourth-fold, fourth-fold, and fifth-fold integrals, resp. 
The integration regions can be demonstrated in [$f_1,f_2$] plane. For instance, in Fig.~\ref{LT} we assume five Nyquist channels can accommodate in the  WDM spectrum. The grid lines in the horizontal($f_1$) and vertical ($f_2$) axes are determined with the five channels border lines. To determine grid lines in the diagonal axis since $f_3=f_1+f_2-f$ and $f'_3= f_1'+f_2'-f$, one can first start with the grid line of the COI channel, using the intersection of the COI grid lines from the horizontal and vertical axes, then the other grid lines of diagonal axis are drawn by the corresponding channel spacings shrank by a factor of $\sqrt{2}$, driven from the coordinates geometry. 






\begin{figure}
\centering
%\begin{tikzpicture}[scale=0.6]
%\draw [postaction={decorate,draw=red!40,fill=red!40}]
%(-0.2-1.15-0.6,0+2) -- (-0.2-1.15+1+0.6,0+2) --(-0.2-1.15+1+0.6,0.75+2)--(-0.2-1.15-0.6,0.75+2)node at (-0.2-1.15+1+0.6,-0.5+2) {\footnotesize{$\frac{R}{2}$}}node at (-0.2-1.4-1+0.6,-0.5+2) {\footnotesize{$-\frac{R}{2}$}};
%\draw [-latex,red, thick] (-0.975-0.5-1.15,0+2) -- (-0.6+3.5-0.55-1.15,0+2) node at (-0.6+3.5-0.55-1,-0.2+2) {$f$};
%\draw [-latex,dashed] (-0.2-1.15+1/2,0+2.25-2.25+2) -- (-0.2-1.15+1/2,0+2+1.7-2.25+2) node at (-0.2-1.15+1/2,0+2+1.7-2+2) {\footnotesize{$f=0$}};
%\draw [postaction={decorate,draw=red!40,fill=red!40}]
%(-0.2-1.15-0.6+1,0+2) -- (-0.2-1.15+1+0.6+1,0+2) --(-0.2-1.15+1+0.6+1,0.75+2)--(-0.2-1.15-0.6+1,0.75+2);
%\end{tikzpicture}
\begin{tikzpicture}[scale=0.6]
%\node at (-2,-2){a)};
 \draw[thick, blue!20]
 (0,2)--(1,2) -- (2,1)-- (2,0)--(1,0)--(0,1)--(0,2);
 \draw[thick, blue!20]
 (1.1,2) -- (2,1.1)--(2,2)--(1.1,2);
 \draw[thick, blue!20]
 (0,0) -- (0,0.9)--(0.9,0)--(0,0);
    \def\mypath{ (0,0) -- (0,0.9)--(0.9,0)--(0,0)}
\fill[purple]\mypath;

 
 
 \draw[thick, blue!20]
 (2.1,2)--(3.1,2) -- (4.1,1)-- (4.1,0)--(3.1,0)--(2.1,1)--(2.1,2);
 \draw[thick, blue!20]
 (3.2,2) -- (4.1,1.1)--(4.1,2)--(3.2,2);
 \draw[thick, blue!20]
 (2.1,0) -- (2.1,0.9)--(3,0)--(2.1,0);
     \def\mypath{ (2.1,0) -- (2.1,0.9)--(3,0)--(2.1,0)}
 \fill[purple]\mypath;
 
 
 \draw[thick, blue!20]
 (4.2,2)--(5.2,2) -- (6.2,1)-- (6.2,0)--(5.2,0)--(4.2,1)--(4.2,2);
 \draw[thick, blue!20]
 (5.3,2) -- (6.2,1.1)--(6.2,2)--(5.3,2);
    \def\mypath{ (5.3,2) -- (6.2,1.1)--(6.2,2)--(5.3,2)}
 \mypath;
\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 \draw[thick, blue!20]
 (4.2,0) -- (4.2,0.9)--(5.1,0)--(4.2,0);
   \def\mypath{(4.2,0) -- (4.2,0.9)--(5.1,0)--(4.2,0)}
 \fill[purple]\mypath;

 
 \draw[thick, blue!20]
 (6.3,2)--(7.3,2) -- (8.3,1)-- (8.3,0)--(7.3,0)--(6.3,1)--(6.3,2);
     \def\mypath{ (6.3,2)--(7.3,2) -- (8.3,1)-- (8.3,0)--(7.3,0)--(6.3,1)--(6.3,2)}
\mypath;
\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 \draw[thick, blue!20]
 (6.3,0) -- (6.3,0.9)--(7.2,0)--(6.3,0);
    \def\mypath{ (6.3,0) -- (6.3,0.9)--(7.2,0)--(6.3,0)}
 \fill[purple]\mypath;

 
 %%%%%%%%
% \draw [ -latex,red!100, thick, dashed] (-0.2,-1) -- (10.2,-1) 
%\node at ( 7.3,-1.1) [inner sep=0pt,minimum size=2mm,circle,fill=red!100] (3){\scriptsize {}};

\draw[thick, blue!20]
 (0,-0.1)--(1,-0.1) -- (2,-1.1)-- (2,-2.1)--(1,-2.1)--(0,-1.1)--(0,-0.1);
  \def\mypath{ (0,-0.1)--(1,-0.1) -- (2,-1.1)-- (2,-2.1)--(1,-2.1)--(0,-1.1)--(0,-0.1)}
\fill[purple] \mypath;

 
 \draw[thick, blue!20]
 (1.1,-0.1) -- (2,-1)--(2,-0.1)--(1.1,-0.1);
  \def\mypath{  (1.1,-0.1) -- (2,-1)--(2,-0.1)--(1.1,-0.1)}
\mypath;

    
 \draw[thick, blue!20]
 (2.1,-0.1)--(3.1,-0.1) -- (4.1,-1.1)-- (4.1,-2.1)--(3.1,-2.1)--(2.1,-1.1)--(2.1,-0.1);
 \def\mypath{ (2.1,-0.1)--(3.1,-0.1) -- (4.1,-1.1)-- (4.1,-2.1)--(3.1,-2.1)--(2.1,-1.1)--(2.1,-0.1)}
\fill[purple] \mypath;
\pattern[color=white,pattern=horizontal lines] \mypath;
    \def\mypath{ (2.1,-0.1)--(3.1,-0.1) -- (4.1,-1.1)-- (4.1,-2.1)--(3.1,-2.1)--(2.1,-1.1)--(2.1,-0.1)}
\fill[purple] \mypath;
\pattern[pattern color=purple,pattern=horizontal lines] \mypath;

 \draw[thick, blue!20]
 (3.2,-0.1) -- (4.1,-1)--(4.1,-0.1)--(3.2,-0.1);
 \draw[thick, blue!20]
 (2.1,-2.1) -- (2.1,-1.2)--(3,-2.1)--(2.1,-2.1);
 
 \draw[thick, blue!20]
 (4.2,-0.1)--(5.2,-0.1) -- (6.2,-1.1)-- (6.2,-2.1)--(5.2,-2.1)--(4.2,-1.1)--(4.2,-0.1);
   \def\mypath{ (4.2,-0.1)--(5.2,-0.1) -- (6.2,-1.1)-- (6.2,-2.1)--(5.2,-2.1)--(4.2,-1.1)--(4.2,-0.1)}
\fill[purple] \mypath;
\pattern[pattern color=purple,pattern=horizontal lines] \mypath;

 \draw[thick, blue!20]
 (5.3,-0.1) -- (6.2,-1)--(6.2,-0.1)--(5.3,-0.1);
 \def\mypath{ (5.3,-0.1) -- (6.2,-1)--(6.2,-0.1)--(5.3,-0.1)}
\mypath;
\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 \draw[thick, blue!20]
 (4.2,-2.1) -- (4.2,-1.2)--(5.1,-2.1)--(4.2,-2.1);
 
 \draw[thick, blue!20, fill=red]
 (6.3,-0.1)--(7.3,-0.1) -- (8.3,-1.1)-- (8.3,-2.1)--(7.3,-2.1)--(6.3,-1.1)--(6.3,-0.1)node at (6.8,-0.5) [black]{SCI} node at (7.8,-1.5) [black]{\scriptsize{COI}};
    \def\mypath{ (6.3,-0.1)--(7.3,-0.1) -- (8.3,-1.1)-- (8.3,-2.1)--(7.3,-2.1)--(6.3,-1.1)--(6.3,-0.1)}
\fill [fill=white] \mypath;
\pattern[pattern color=red,pattern=dots] \mypath;

 \draw[thick, blue!20, fill=black!40!green]
 (7.4,-0.1) -- (8.3,-1)--(8.3,-0.1)--(7.4,-0.1);
\def\mypath{ (7.4,-0.1) -- (8.3,-1)--(8.3,-0.1)--(7.4,-0.1)}
\fill [fill=black!40!green] \mypath;
\pattern[pattern color=white,pattern=grid] \mypath;
 
 \draw[thick, blue!20, fill=black!40!green]
 (6.3,-2.1) -- (6.3,-1.2)--(7.2,-2.1)--(6.3,-2.1);
 \def\mypath{ (6.3,-2.1) -- (6.3,-1.2)--(7.2,-2.1)--(6.3,-2.1)}
\fill [fill=black!40!green] \mypath;
\pattern[pattern color=white,pattern=grid] \mypath;
 
 \draw[thick, blue!20, fill=red]%pink balla
 (8.4,0) -- (8.4,0.9)--(9.3,0)--(8.4,0);
  \def\mypath{ (8.4,0) -- (8.4,0.9)--(9.3,0)--(8.4,0)}
\fill [fill=white] \mypath;
\pattern[pattern color=red,pattern=dots] \mypath;
 
\draw[thick, blue!20]
 (8.4,-0.1)--(9.4,-0.1) -- (10.4,-1.1)-- (10.4,-2.1)--(9.4,-2.1)--(8.4,-1.1)--(8.4,-0.1);
    \def\mypath{ (8.4,-0.1)--(9.4,-0.1) -- (10.4,-1.1)-- (10.4,-2.1)--(9.4,-2.1)--(8.4,-1.1)--(8.4,-0.1)}
 \fill[purple]\mypath;
\pattern[pattern color=purple,pattern=horizontal lines]\mypath;
%\draw[thick, blue!20]
% (9.5,-0.1) -- (10.4,-1)--(10.4,-0.1)--(9.5,-0.1);
\draw[thick, blue!20]
 (8.4,-2.1) -- (8.4,-1.2)--(9.3,-2.1)--(8.4,-2.1);
   \def\mypath{  (8.4,-2.1) -- (8.4,-1.2)--(9.3,-2.1)--(8.4,-2.1)}
 \mypath;
\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 %%%%%%%%%%
 \draw[thick, blue!20]
 (1.1,-2.2) -- (2,-3.1)--(2,-2.2)--(1.1,-2.2);
   \def\mypath{ (1.1,-2.2) -- (2,-3.1)--(2,-2.2)--(1.1,-2.2)}
\fill[purple]\mypath;
\pattern[pattern color=purple,pattern=horizontal lines]\mypath;

 
 \draw[thick, blue!20]
 (2.1,-2.2)--(3.1,-2.2) -- (4.1,-3.2)-- (4.1,-4.2)--(3.1,-4.2)--(2.1,-3.2)--(2.1,-2.2);
 \draw[thick, blue!20]
 (3.2,-2.2) -- (4.1,-3.1)--(4.1,-2.2)--(3.2,-2.2);
  \def\mypath{ (3.2,-2.2) -- (4.1,-3.1)--(4.1,-2.2)--(3.2,-2.2)}
\fill[purple]\mypath;
\pattern[pattern color=purple,pattern=horizontal lines]\mypath;
 
 \draw[thick, blue!20, fill=black!40!green]
 (4.2,-2.2)--(5.2,-2.2) -- (6.2,-3.2)-- (6.2,-4.2)--(5.2,-4.2)--(4.2,-3.2)--(4.2,-2.2);
    \def\mypath{ (4.2,-2.2)--(5.2,-2.2) -- (6.2,-3.2)-- (6.2,-4.2)--(5.2,-4.2)--(4.2,-3.2)--(4.2,-2.2)}
\fill [fill=black!40!green] \mypath;
\pattern[pattern color=white,pattern=grid] \mypath;
 
 \draw[thick, blue!20, fill=red]
 (5.3,-2.2) -- (6.2,-3.1)--(6.2,-2.2)--(5.3,-2.2);
   \def\mypath{(5.3,-2.2) -- (6.2,-3.1)--(6.2,-2.2)--(5.3,-2.2)}
\fill [fill=white] \mypath;
\pattern[pattern color=red,pattern=dots] \mypath;
 
 \draw[thick, blue!20, fill=black!40!green]
 (4.2,-4.2) -- (4.2,-3.3)--(5.1,-4.2)--(4.2,-4.2);
  \def\mypath{ (4.2,-4.2) -- (4.2,-3.3)--(5.1,-4.2)--(4.2,-4.2)}
\fill [fill=black!40!green] \mypath;
\pattern[pattern color=white,pattern=grid] \mypath;
 
 
 \draw[thick, blue!20]
 (6.3,-2.2)--(7.3,-2.2) -- (8.3,-3.2)-- (8.3,-4.2)--(7.3,-4.2)--(6.3,-3.2)--(6.3,-2.2);
 \def\mypath{ (6.3,-2.2)--(7.3,-2.2) -- (8.3,-3.2)-- (8.3,-4.2)--(7.3,-4.2)--(6.3,-3.2)--(6.3,-2.2)}
 \mypath;
\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 \draw[thick, blue!20]
 (7.4,-2.2) -- (8.3,-3.1)--(8.3,-2.2)--(7.4,-2.2);
 \def\mypath{ (7.4,-2.2) -- (8.3,-3.1)--(8.3,-2.2)--(7.4,-2.2)}
\fill[purple]\mypath;
\pattern[pattern color=purple,pattern=horizontal lines]\mypath;
 
 \draw[thick, blue!20]
 (6.3,-4.2) -- (6.3,-3.3)--(7.2,-4.2)--(6.3,-4.2);
 
\draw[thick, blue!20]
 (8.4,-2.2)--(9.4,-2.2) -- (10.4,-3.2)-- (10.4,-4.2)--(9.4,-4.2)--(8.4,-3.2)--(8.4,-2.2);
\draw[thick, blue!20]
 (9.5,-2.2) -- (10.4,-3.1)--(10.4,-2.2)--(9.5,-2.2);
 \def\mypath{(9.5,-2.2) -- (10.4,-3.1)--(10.4,-2.2)--(9.5,-2.2)}
 \fill[purple]\mypath;
\pattern[pattern color=purple,pattern=horizontal lines]\mypath;
 
\draw[thick, blue!20]
 (8.4,-4.2) -- (8.4,-3.3)--(9.3,-4.2)--(8.4,-4.2);
\def\mypath{ (8.4,-4.2) -- (8.4,-3.3)--(9.3,-4.2)--(8.4,-4.2)}
 \mypath;
\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 %%%%%%%%%%

 \draw[thick, blue!20, fill=black!40!green]
 (3.2,-4.3) -- (4.1,-5.2)--(4.1,-4.3)--(3.2,-4.3);
      \def\mypath{ (3.2,-4.3) -- (4.1,-5.2)--(4.1,-4.3)--(3.2,-4.3)}
\fill [fill=black!40!green] \mypath;
\pattern[pattern color=white,pattern=grid] \mypath;
 
 
 \draw[thick, blue!20]
 (4.2,-4.3)--(5.2,-4.3) -- (6.2,-5.3)-- (6.2,-6.3)--(5.2,-6.3)--(4.2,-5.3)--(4.2,-4.3);
 \draw[thick, blue!20]
 (5.3,-4.3) -- (6.2,-5.2)--(6.2,-4.3)--(5.3,-4.3);
     \def\mypath{(5.3,-4.3) -- (6.2,-5.2)--(6.2,-4.3)--(5.3,-4.3)}
\mypath;
\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 
 \draw[thick, blue!20]
 (6.3,-4.3)--(7.3,-4.3) -- (8.3,-5.3)-- (8.3,-6.3)--(7.3,-6.3)--(6.3,-5.3)--(6.3,-4.3);
    \def\mypath{ (6.3,-4.3)--(7.3,-4.3) -- (8.3,-5.3)-- (8.3,-6.3)--(7.3,-6.3)--(6.3,-5.3)--(6.3,-4.3)}
\mypath;
\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 \draw[thick, blue!20]
 (7.4,-4.3) -- (8.3,-5.2)--(8.3,-4.3)--(7.4,-4.3);
 \draw[thick, blue!20]
 (6.3,-6.3) -- (6.3,-5.4)--(7.2,-6.3)--(6.3,-6.3);
 
\draw[thick, blue!20]
 (8.4,-4.3)--(9.4,-4.3) -- (10.4,-5.3)-- (10.4,-6.3)--(9.4,-6.3)--(8.4,-5.3)--(8.4,-4.3);

 
\draw[thick, blue!20]
 (9.5,-4.3) -- (10.4,-5.2)--(10.4,-4.3)--(9.5,-4.3);
\draw[thick, blue!20]
 (8.4,-6.3) -- (8.4,-5.4)--(9.3,-6.3)--(8.4,-6.3);
  \def\mypath{ (8.4,-6.3) -- (8.4,-5.4)--(9.3,-6.3)--(8.4,-6.3)}
\mypath;
\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 %%%%%%%%%%

 \draw[thick, blue!20]
 (5.3,-6.4) -- (6.2,-7.3)--(6.2,-6.4)--(5.3,-6.4);
 \def\mypath{  (5.3,-6.4) -- (6.2,-7.3)--(6.2,-6.4)--(5.3,-6.4)}
\mypath;
\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 \draw[thick, blue!20]
 (6.3,-6.4)--(7.3,-6.4) -- (8.3,-7.4)-- (8.3,-8.4)--(7.3,-8.4)--(6.3,-7.4)--(6.3,-6.4);
  \def\mypath{ (6.3,-6.4)--(7.3,-6.4) -- (8.3,-7.4)-- (8.3,-8.4)--(7.3,-8.4)--(6.3,-7.4)--(6.3,-6.4)}\fill[blue];
\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 \draw[thick, blue!20]
 (7.4,-6.4) -- (8.3,-7.3)--(8.3,-6.4)--(7.4,-6.4);
 
\draw[thick, blue!20]
 (8.4,-6.4)--(9.4,-6.4) -- (10.4,-7.4)-- (10.4,-8.4)--(9.4,-8.4)--(8.4,-7.4)--(8.4,-6.4);
%\draw[thick, blue!20]
% (9.5,-6.4) -- (10.4,-7.3)--(10.4,-6.4)--(9.5,-6.4);
\draw[thick, blue!20]
 (8.4,-8.4) -- (8.4,-7.5)--(9.3,-8.4)--(8.4,-8.4);
  \def\mypath{(8.4,-8.4) -- (8.4,-7.5)--(9.3,-8.4)--(8.4,-8.4)}
\mypath;
\pattern[pattern color=blue,pattern=vertical lines] \mypath;

\draw[thick, blue!20]
(9.5,-6.4) -- (10.4,-7.3)--(10.4,-6.4)--cycle;

 
 
% \draw [ -latex,red, ultra thick, dashed] (-0.2,-1.1) -- (11.7,-1.1);
%\draw [ -latex,red,ultra thick,dashed] (7.3,-8.6) -- (7.3,3.8)node at (7.3,4.2) {axes of maximum FWM efficiency};

 \draw [ -latex,blue!50, thick] (-0.2-1,-3.2-5.2) -- (11.2,-3.2-5.2) node at (11.5,-3.4-5) {\tiny$ f_1$};
 
 % \draw [ -latex,blue!50, dashed] (-0.2-1,-3.2-5.3) -- (12.5,-3.2-5.3) node at (12.7,-3.2-5) {\small$\kappa_1$};
 
\draw [ -latex,blue!50, thick] (0,-8.6-1) -- (0,3) node at (0,3.3) {\tiny$f_2$};

%\draw [ -latex,blue!50, dashed] (-0.1,-8.6-1) -- (-0.1,4) node at (-0.1,4.3) {\small$\kappa_2$};

\draw [ -latex,blue!50, thick] (2.4-3,-6-3) -- (10.5,2.1) node at (10.5,2.5) {\tiny$ f_1+f_2$};


%\draw [ -latex,blue!50, dashed] (2.4-3+0.05,-6-3-0.05) -- (11+0.3,2.8-0.05) node at (11+0.3,3.3-0.05) {\small$\tilde{\kappa}$};

% \draw[thick, blue!40, fill=blue!40]
% (1.25,-4) -- (1.25,-3.75)--(1.5,-3.75)--(1.5,-4)-- (1.25,-4) node at (0.2,-3.87) [black]{XCI X1};
% 
% \draw[thick, blue!20, fill=blue!20]
% (1.25,-4.7) -- (1.25,-4.45)--(1.5,-4.45)--(1.5,-4.7)-- (1.25,-4.7)node at (0.2,-4.6) [black]{XCI X2};
% 
%\draw[thick, black!50!blue, fill=black!50!blue]
% (1.25,-5.4) -- (1.25,-5.15)--(1.5,-5.15)--(1.5,-5.4)-- (1.25,-5.4)node at (0.2,-5.34) [black]{XCI X3};
%
%\draw[thick, pink, fill=pink]
% (1.25,-6.1) -- (1.25,-5.85)--(1.5,-5.85)--(1.5,-6.1)-- (1.25,-6.1)node at (0.2,-6.08) [black]{XCI X4};
% 
% %%%%%
%  \draw[thick, black, fill=white]
% (1.75,-6.75) -- (1.75,-6.5)--(2,-6.5)--(2,-6.75)-- (1.75,-6.75) node at (3.2,-6.6) [black]{MCI M0};
% 
%  \draw[thick, yellow, fill=yellow]
% (1.75,-7.45) -- (1.75,-7.2)--(2,-7.2)--(2,-7.45)-- (1.75,-7.45)node at (3.2,-7.34) [black]{MCI M1};
% 
%  \draw[thick, red, fill=red]
% (1.75,-8.15) -- (1.75,-7.9)--(2,-7.9)--(2,-8.15)-- (1.75,-8.15)node at (3.2,-8.08) [black]{MCI M2};
%
%\draw[thick, black!50!green, fill=black!50!green]
% (1.75,-8.85) -- (1.75,-8.6)--(2,-8.6)--(2,-8.85)-- (1.75,-8.85)node at (3.2,-8.82) [black]{MCI M3};
\node at (0.9,1){\scriptsize{(1,5,2)}};
\node at (-1,-2){a)};

 \draw[thick, blue!20,fill=purple]{ 
 (1+0.75,-4-6.5) -- (1+0.75,-3-6.5)--(2+0.75,-3-6.5)--(2+0.75,-4-6.5)-- cycle node at (2.3,-4.2-5) [black]{\footnotesize{$E_\kappa$}}};
 %\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 \draw[thick, blue!20]{ (1+0.75+1.75,-4-6.5) -- (1+0.75+1.75,-3-6.5)--(2+0.75+1.75,-3-6.5)--(2+0.75+1.75,-4-6.5)-- cycle};
 \def\mypath{ (1+0.75+1.75,-4-6.5) -- (1+0.75+1.75,-3-6.5)--(2+0.75+1.75,-3-6.5)--(2+0.75+1.75,-4-6.5)-- cycle node at  (2.3+1.75,-4.2-5) [black]{\footnotesize{$F_\kappa$}}};
 \pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 \draw[thick, blue!20,fill=black!40!green]{(1+0.75+1.75+1.75,-4-6.5) -- (1+0.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75,-4-6.5)-- cycle node at (2.3+1.75+1.75,-4.2-5) [black]{\footnotesize{$G_\kappa$}}};
  \def\mypath{ (1+0.75+1.75+1.75,-4-6.5) -- (1+0.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75,-4-6.5)-- cycle};
     \pattern[pattern color=white,pattern=grid] \mypath;
  
  
 \draw[thick, blue!20]{ (1+0.75+1.75+1.75+1.75,-4-6.5) -- (1+0.75+1.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75+1.75,-4-6.5)-- cycle node at (2.3+1.75+1.75+1.75,-4.2-5) [black]{\footnotesize{$H_\kappa$}}};
  \def\mypath{(1+0.75+1.75+1.75+1.75,-4-6.5) -- (1+0.75+1.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75+1.75,-4-6.5)-- cycle};
\pattern[pattern color=red,pattern=dots] \mypath;
 
 
\end{tikzpicture}

\begin{tikzpicture}[scale=0.6]
\node at (-1,-2){b)};
 \draw[thick, blue!20]
 (0,2)--(1,2) -- (2,1)-- (2,0)--(1,0)--(0,1)--(0,2);
 \draw[thick, blue!20]
 (1.1,2) -- (2,1.1)--(2,2)--(1.1,2);
 \draw[thick, blue!20, fill=yellow]
 (0,0) -- (0,0.9)--(0.9,0)--(0,0);
 
 \draw[thick, blue!20]
 (2.1,2)--(3.1,2) -- (4.1,1)-- (4.1,0)--(3.1,0)--(2.1,1)--(2.1,2);
 \draw[thick, blue!20]
 (3.2,2) -- (4.1,1.1)--(4.1,2)--(3.2,2);
 \draw[thick, blue!20, fill=yellow]
 (2.1,0) -- (2.1,0.9)--(3,0)--(2.1,0);
 
 \draw[thick, blue!20]
 (4.2,2)--(5.2,2) -- (6.2,1)-- (6.2,0)--(5.2,0)--(4.2,1)--(4.2,2);
 \draw[thick, blue!20, fill=yellow]
 (5.3,2) -- (6.2,1.1)--(6.2,2)--(5.3,2);
 \draw[thick, blue!20, fill=yellow]
 (4.2,0) -- (4.2,0.9)--(5.1,0)--(4.2,0);
 
 \draw[thick, blue!20, fill=blue!40]
 (6.3,2)--(7.3,2) -- (8.3,1)-- (8.3,0)--(7.3,0)--(6.3,1)--(6.3,2);
 \draw[thick, blue!20, fill=blue!20]
 (6.3,0) -- (6.3,0.9)--(7.2,0)--(6.3,0);
 %%%%%%%%
% \draw [ -latex,red!100, thick, dashed] (-0.2,-1) -- (10.2,-1) 
%\node at ( 7.3,-1.1) [inner sep=0pt,minimum size=2mm,circle,fill=red!100] (3){\scriptsize {}};

\draw[thick, blue!20, fill=blue!40]
 (0,-0.1)--(1,-0.1) -- (2,-1.1)-- (2,-2.1)--(1,-2.1)--(0,-1.1)--(0,-0.1);
 \draw[thick, blue!20]
 (1.1,-0.1) -- (2,-1)--(2,-0.1)--(1.1,-0.1);
 
 \draw[thick, blue!20, fill=blue!40]
 (2.1,-0.1)--(3.1,-0.1) -- (4.1,-1.1)-- (4.1,-2.1)--(3.1,-2.1)--(2.1,-1.1)--(2.1,-0.1);
 \draw[thick, blue!20]
 (3.2,-0.1) -- (4.1,-1)--(4.1,-0.1)--(3.2,-0.1);
 \draw[thick, blue!20]
 (2.1,-2.1) -- (2.1,-1.2)--(3,-2.1)--(2.1,-2.1);
 
 \draw[thick, blue!20, fill=blue!40]
 (4.2,-0.1)--(5.2,-0.1) -- (6.2,-1.1)-- (6.2,-2.1)--(5.2,-2.1)--(4.2,-1.1)--(4.2,-0.1);
 \draw[thick, blue!20, fill=blue!20]
 (5.3,-0.1) -- (6.2,-1)--(6.2,-0.1)--(5.3,-0.1);
 \draw[thick, blue!20]
 (4.2,-2.1) -- (4.2,-1.2)--(5.1,-2.1)--(4.2,-2.1);
 
 \draw[thick, blue!20, fill=pink]
 (6.3,-0.1)--(7.3,-0.1) -- (8.3,-1.1)-- (8.3,-2.1)--(7.3,-2.1)--(6.3,-1.1)--(6.3,-0.1) node at (6.9,-0.8) [black]{\scriptsize{COI}};
 \draw[thick, blue!20, fill=black!50!blue]
 (7.4,-0.1) -- (8.3,-1)--(8.3,-0.1)--(7.4,-0.1);
 \draw[thick, blue!20, fill=black!50!blue]
 (6.3,-2.1) -- (6.3,-1.2)--(7.2,-2.1)--(6.3,-2.1);
 \draw[thick, blue!20, fill=pink]%pink balla
 (8.4,0) -- (8.4,0.9)--(9.3,0)--(8.4,0);
 
\draw[thick, blue!20, fill=blue!40]
 (8.4,-0.1)--(9.4,-0.1) -- (10.4,-1.1)-- (10.4,-2.1)--(9.4,-2.1)--(8.4,-1.1)--(8.4,-0.1);
%\draw[thick, blue!20]
% (9.5,-0.1) -- (10.4,-1)--(10.4,-0.1)--(9.5,-0.1);
\draw[thick, blue!20, fill=blue!20]
 (8.4,-2.1) -- (8.4,-1.2)--(9.3,-2.1)--(8.4,-2.1);
 %%%%%%%%%%
 \draw[thick, blue!20, fill=red]
 (1.1,-2.2) -- (2,-3.1)--(2,-2.2)--(1.1,-2.2);

 
 \draw[thick, blue!20]
 (2.1,-2.2)--(3.1,-2.2) -- (4.1,-3.2)-- (4.1,-4.2)--(3.1,-4.2)--(2.1,-3.2)--(2.1,-2.2);
 \draw[thick, blue!20, fill=red]
 (3.2,-2.2) -- (4.1,-3.1)--(4.1,-2.2)--(3.2,-2.2);
 
 \draw[thick, blue!20, fill=black!40!green]
 (4.2,-2.2)--(5.2,-2.2) -- (6.2,-3.2)-- (6.2,-4.2)--(5.2,-4.2)--(4.2,-3.2)--(4.2,-2.2);
 \draw[thick, blue!20, fill=pink]
 (5.3,-2.2) -- (6.2,-3.1)--(6.2,-2.2)--(5.3,-2.2);
 \draw[thick, blue!20, fill=black!40!green]
 (4.2,-4.2) -- (4.2,-3.3)--(5.1,-4.2)--(4.2,-4.2);
 
 \draw[thick, blue!20, fill=blue!40]
 (6.3,-2.2)--(7.3,-2.2) -- (8.3,-3.2)-- (8.3,-4.2)--(7.3,-4.2)--(6.3,-3.2)--(6.3,-2.2);
 \draw[thick, blue!20, fill=blue!20]
 (7.4,-2.2) -- (8.3,-3.1)--(8.3,-2.2)--(7.4,-2.2);
 \draw[thick, blue!20]
 (6.3,-4.2) -- (6.3,-3.3)--(7.2,-4.2)--(6.3,-4.2);
 
\draw[thick, blue!20]
 (8.4,-2.2)--(9.4,-2.2) -- (10.4,-3.2)-- (10.4,-4.2)--(9.4,-4.2)--(8.4,-3.2)--(8.4,-2.2);
\draw[thick, blue!20, fill=yellow]
 (9.5,-2.2) -- (10.4,-3.1)--(10.4,-2.2)--(9.5,-2.2);
\draw[thick, blue!20, fill=yellow]
 (8.4,-4.2) -- (8.4,-3.3)--(9.3,-4.2)--(8.4,-4.2);
 %%%%%%%%%%

 \draw[thick, blue!20, fill=black!40!green]
 (3.2,-4.3) -- (4.1,-5.2)--(4.1,-4.3)--(3.2,-4.3);
 
 \draw[thick, blue!20]
 (4.2,-4.3)--(5.2,-4.3) -- (6.2,-5.3)-- (6.2,-6.3)--(5.2,-6.3)--(4.2,-5.3)--(4.2,-4.3);
 \draw[thick, blue!20, fill=red]
 (5.3,-4.3) -- (6.2,-5.2)--(6.2,-4.3)--(5.3,-4.3);
 
 \draw[thick, blue!20, fill=blue!40]
 (6.3,-4.3)--(7.3,-4.3) -- (8.3,-5.3)-- (8.3,-6.3)--(7.3,-6.3)--(6.3,-5.3)--(6.3,-4.3);
 \draw[thick, blue!20]
 (7.4,-4.3) -- (8.3,-5.2)--(8.3,-4.3)--(7.4,-4.3);
 \draw[thick, blue!20]
 (6.3,-6.3) -- (6.3,-5.4)--(7.2,-6.3)--(6.3,-6.3);
 
\draw[thick, blue!20]
 (8.4,-4.3)--(9.4,-4.3) -- (10.4,-5.3)-- (10.4,-6.3)--(9.4,-6.3)--(8.4,-5.3)--(8.4,-4.3);
\draw[thick, blue!20]
 (9.5,-4.3) -- (10.4,-5.2)--(10.4,-4.3)--(9.5,-4.3);
\draw[thick, blue!20, fill=yellow]
 (8.4,-6.3) -- (8.4,-5.4)--(9.3,-6.3)--(8.4,-6.3);
 %%%%%%%%%%

 \draw[thick, blue!20, fill=red]
 (5.3,-6.4) -- (6.2,-7.3)--(6.2,-6.4)--(5.3,-6.4);
 
 \draw[thick, blue!20, fill=blue!40]
 (6.3,-6.4)--(7.3,-6.4) -- (8.3,-7.4)-- (8.3,-8.4)--(7.3,-8.4)--(6.3,-7.4)--(6.3,-6.4);
 \draw[thick, blue!20]
 (7.4,-6.4) -- (8.3,-7.3)--(8.3,-6.4)--(7.4,-6.4);
 
\draw[thick, blue!20]
 (8.4,-6.4)--(9.4,-6.4) -- (10.4,-7.4)-- (10.4,-8.4)--(9.4,-8.4)--(8.4,-7.4)--(8.4,-6.4);
\draw[thick, blue!20]
 (9.5,-6.4) -- (10.4,-7.3)--(10.4,-6.4)--(9.5,-6.4);
\draw[thick, blue!20, fill=yellow]
 (8.4,-8.4) -- (8.4,-7.5)--(9.3,-8.4)--(8.4,-8.4);
 
 
% \draw [ -latex,red, ultra thick, dashed] (-0.2,-1.1) -- (11.7,-1.1);
%\draw [ -latex,red,ultra thick,dashed] (7.3,-8.6) -- (7.3,3.8)node at (7.3,4.2) {axes of maximum FWM efficiency};

\draw [ -latex,blue!50, thick] (-0.2-1,-3.2-5.2) -- (11.2,-3.2-5.2) node at (11.5,-3.4-5) {\tiny$ f_1$};
 
 % \draw [ -latex,blue!50, dashed] (-0.2-1,-3.2-5.3) -- (12.5,-3.2-5.3) node at (12.7,-3.2-5) {\small$\kappa_1$};
 
\draw [ -latex,blue!50, thick] (0,-8.6-1) -- (0,3) node at (0,3.3) {\tiny$f_2$};

%\draw [ -latex,blue!50, dashed] (-0.1,-8.6-1) -- (-0.1,4) node at (-0.1,4.3) {\small$\kappa_2$};

\draw [ -latex,blue!50, thick] (2.4-3,-6-3) -- (10.5,2.1) node at (10.5,2.5) {\tiny$ f_1+f_2$};


%\draw [ -latex,blue!50, dashed] (2.4-3+0.05,-6-3-0.05) -- (11+0.3,2.8-0.05) node at (11+0.3,3.3-0.05) {\small$\tilde{\kappa}$};

 \draw[thick, blue!40, fill=blue!40]
 (1.25+3,-4-6) -- (1.25+3,-3.75-6)--(1.5+3,-3.75-6)--(1.5+3,-4-6)-- (1.25+3,-4-6) node at (0.2+3,-3.87-6) [black]{XCI X1};
 
 \draw[thick, blue!20, fill=blue!20]
 (1.25+3,-4.7-6) -- (1.25+3,-4.45-6)--(1.5+3,-4.45-6)--(1.5+3,-4.7-6)-- (1.25+3,-4.7-6)node at (0.2+3,-4.6-6) [black]{XCI X2};
 
\draw[thick, black!50!blue, fill=black!50!blue]
 (1.25+3,-5.4-6) -- (1.25+3,-5.15-6)--(1.5+3,-5.15-6)--(1.5+3,-5.4-6)-- (1.25+3,-5.4-6)node at (0.2+3,-5.34-6) [black]{XCI X3};

\draw[thick, pink, fill=pink]
 (1.25+3,-6.1-6) -- (1.25+3,-5.85-6)--(1.5+3,-5.85-6)--(1.5+3,-6.1-6)-- (1.25+3,-6.1-6)node at (-0.4+3,-6.08-6) [black]{SCI, XCI X4};
 
 %%%%%
  \draw[thick, black, fill=white]
 (1.75+5,-6.75-3.25) -- (1.75+5,-6.5-3.25)--(2+5,-6.5-3.25)--(2+5,-6.75-3.25)-- (1.75+5,-6.75-3.25) node at (3.2+5,-6.6-3.25) [black]{MCI M0};
 
  \draw[thick, yellow, fill=yellow]
 (1.75+5,-7.45-3.25) -- (1.75+5,-7.2-3.25)--(2+5,-7.2-3.25)--(2+5,-7.45-3.25)-- (1.75+5,-7.45-3.25)node at (3.2+5,-7.34-3.25) [black]{MCI M1};
 
  \draw[thick, red, fill=red]
 (1.75+5,-8.15-3.25) -- (1.75+5,-7.9-3.25)--(2+5,-7.9-3.25)--(2+5,-8.15-3.25)-- (1.75+5,-8.15-3.25)node at (3.2+5,-8.08-3.25) [black]{MCI M2};

\draw[thick, black!50!green, fill=black!50!green]
 (1.75+5,-8.85-3.25) -- (1.75+5,-8.6-3.25)--(2+5,-8.6-3.25)--(2+5,-8.85-3.25)-- (1.75+5,-8.85-3.25)node at (3.2+5,-8.82-3.25) [black]{MCI M3};

\end{tikzpicture}
\caption{
Demonstrating regions of the EGN model terms integrands, the GN model, and the correction terms of (\ref{EGN_fixed}), for a five-channel fiber-optic spectrum (rectangular Nyquist) and its fourth channel as the COI ($\kappa=4$). The white islands (polygons) are representing the regions, where NLI contribution to the COI is present only based on the GN model term, whereas the colored islands are contributing NLI to the COI based on both GN model and correction terms. $l=-1$ and $l=+1$ indicate the lower and upper triangle islands, resp, while $l=0$ indicates the lozenge shape islands.
}
\label{LT}
\end{figure}

Here for a fiber-optic link with five spectrum channels ($M$ = 5), where the fourth channel ($\kappa=4$) is assumed to be the COI, islands with different colors and patterns are illustrated in Fig.~\ref{LT}, indicating the areas of spectral components where their interaction gives rise to a certain NLI, either the GN model term or one of the correction terms on the COI. For instance, the island, marked with ``(1, 5, 2)", indicates the NLI contribution on the COI caused by the nonlinear interaction among the spectral components $(f_1,f_1')$, $(f_2,f_2')$, and $(f_1+f_2-f,f_1'+f_2'-f)$ located in channels $1$, $5$, and $2$, respectively, producing a PSD spectral line at frequency $f$ of the COI (channel 4). As seen in Fig.~\ref{LT}, these islands categorized into white and colored islands, where the white islands only produce the GN model term and the colored islands generate both GN model and correction terms.  It is worth mentioning that $l=0$ is demonstrates the lozenge-shaped islands, while $l=\pm 1$ demonstrates the triangle islands. The five introduced terms in \eqref{EGN_fixed} represent the nonlinear interaction between the spectral components $f_1, f_1', f_2, f_2', f_1+f_2-f, f_1'+f_2'-f$ from different island, producing the NLI contributions on the COI (frequency $f$). In the following, we shed more light on these terms as well as their corresponding originating islands.

\subsection{The GN Model term--$D_{\kappa}$}

The GN model term, denoted by $D_{\kappa}$ (see Tabel~\ref{DEFGH}) represents the GN model NLI contribution coefficient on the COI from all the islands (either white islands consisting of only GN model term or the other colored islands with both GN model and correction terms). In fact, this NLI contribution is caused by nonlinear interaction between the spectral lines when the pairs $(f_1,f_1')$, $(f_2,f_2')$, and $(f_3,f_3')$ are located in (i) three different channels, (ii) only two of these pairs are located in the same channel, while the third pair is located in a different channel, or (iii) all the three pairs are located in the same channel. Since in all the above cases each pair is described with only a single spectral line, i. e., $f_1=f_1'$, $f_2=f_2'$, and $f_3=f'_3$, this nonlinear interaction gives rise to the second order moments of the involved channels $\kappa_1$, $\kappa_1+\kappa_2-\kappa+l$, and ${\kappa_2}$ transmit symbols.

\subsection{The first EGN correction term--$E_{\kappa}$}

The first EGN correction term denoted by $E_{\kappa}$ (see Tabel~\ref{DEFGH}) represents the NLI contribution coefficient on the COI stems from the islands with the same channel as the COI as well as the adjacent channel of the COI in the $f_2$ axis, fulfilling the condition of $\kappa_1=\kappa_1+\kappa_2-\kappa+l$. These islands are colored with purple in Fig.~\ref{LT}(a), categorized in the following two groups: 

\begin{enumerate}[(i)]
\item
The  lozenge-shaped islands ($l=0$) filled with blue in Fig. \ref{LT} (b) where spectral lines $f_2$ and $f'_2$ are located in the the same channel as the COI, while spectral lines $f_1$, $f'_1$, $f_3$, and $f_3'$ are co-located in a single interfering channel.
\item
The triangle islands ($l=\pm 1$) filled with red, light blue and yellow in Fig. \ref{LT}(b) where spectral lines $f_2$ and $f'_2$ are co-located in the adjacent channels of the COI, while spectral lines $f_1$, $f'_1$, $f_3$, and $f_3'$ are co-located in a single interfering channel.
\end{enumerate}
The NLI contribution caused by nonlinear interaction between the spectral pair components leads to the second and fourth order moments of the two involved channels transmit symbols.  

\subsection{The second EGN correction term--$F_{\kappa}$}

The second EGN correction term denoted by $F_{\kappa}$ (see Table~\ref{DEFGH}) represents the NLI contribution coefficient on the COI from the islands with the same channel as the COI as well as the adjacent channels of the COI in the $f_1$ axis, fulfilling the condition of $\kappa_2=\kappa_1+\kappa_2-\kappa+l$. These islands are marked with blue vertical lines pattern in Fig.~\ref{LT} (a), categorized in the following two groups: 

\begin{enumerate}[(i)]
\item
The lozenge-shaped islands filled with blue in Fig. \ref{LT}(b) where spectral lines $f_1$ and $f'_1$ are located in the the same channel as the COI, while spectral lines $f_2$, $f'_2$, $f_3$, and $f_3'$ are co-located in a single interfering channel.
\item
The triangle islands filled with red, light blue and yellow in Fig. \ref{LT}(b) where spectral lines $f_1$ and $f'_1$ are co-located in the adjacent channels of the COI, while spectral lines $f_2$, $f'_2$, $f_3$, and $f_3'$ are co-located in a single interfering channel.
\end{enumerate}
The NLI contribution caused by nonlinear interaction between the spectral components pairs leads to the second and fourth order moments of the two involved channels transmit symbols. 

\subsection{The third EGN correction term--$G_{\kappa}$}

The third EGN correction term denoted by $G_{\kappa}$ (see Tabel~\ref{DEFGH}) represents the NLI contribution on the COI from the islands with the same channel on  $f_1$ and $f_2$ axes, i.e., fulfilling the condition of $\kappa_1=\kappa_2$. These islands are marked with green grid pattern in Fig.~\ref{LT} (a), categorized in the following two groups: 

\begin{enumerate}[(i)]
\item
The lozenge-shaped and triangle islands filled with green in Fig.~\ref{LT} (b) where spectral lines pairs $(f_1,f'_1)$ and $(f_2,f'_2)$ are located in a certain interfering channel, while the last pair $(f_3,f'_3)$ located in the channel adjacent to this channel.
\item
The triangle islands filled with dark blue in Fig. \ref{LT} (b) are the subset of the previous category where spectral lines pairs $(f_1,f'_1)$ and $(f_2,f'_2)$ are located in the same channel as the COI.
\end{enumerate}
Therefore, the NLI contribution caused by nonlinear interaction between the spectral pair components leads to second and fourth order moments of the two involved channels transmit symbols. 

\subsection{The fourth EGN correction term--$H_{\kappa}$}
The last EGN correction term denoted by $H_{\kappa}$ (see Tabel~\ref{DEFGH}) represents the NLI contribution coefficient on the COI from the islands with the same channel on all the axes, i.e., $\kappa_1=\kappa_2=\kappa_1+\kappa_2-\kappa+l$. In these islands, marked with dotted pattern in Fig.~\ref{LT} (a) or equivalently filled pink in Fig.~\ref{LT} (b), the six spectral lines with the assumption of $\kappa_1=\kappa_2=\kappa_1+\kappa_2-\kappa+l$ results in six order moments of the involved channel transmit symbols. Here $l=0$ and $l=\pm 1$ indicate the COI and the pink triangle-shaped islands, respectively.


\section{Interpretation of SCI, XCI, and MCI  contributions}\label{interpretation_NLIN_contribution}
Eq.~(\ref{EGN_fixed}) is introduced to evaluate the NLI power on the COI, caused by the following three types of interference: 
\begin{enumerate}[(i)]
\item SCI: The NLI produced by the COI on itself, i. e., all the interfering spectral components are located in the COI
\item XCI: The NLI generated by the interfering spectral components located in two different channels such that one of these channels is the COI and the other one is a different interfering channel
\item MCI: The NLI created by the interfering spectral components located in three different channels. 
\end{enumerate}
As shown in Fig.~\ref{LT}(b), XCI terms can be categorized into X1 (blue lozenge-shaped islands), X2 (light blue triangle-shaped islands around COI), X3 (dark blue triangle-shaped islands around COI), and X4 (pink triangle-shaped islands) terms. Among these nonlinear terms X1 terms are dominant, also called XPM nonlinear effects. In fact, the XPM terms are the result of nonlinear interaction of spectral pair components $(f_1,f_1')$, $(f_2,f_2')$, and $(f_1+f_2-f,f_1'+f_2'-f)$ when one of these pairs are located in the COI and the other two pairs are co-located in a different interfering channel. As shown in Fig.~\ref{LT}(b), the MCI nonlinear contributions are classified in four M0, M1 M2, and M3 groups. Using the above classification of the nonlinear interference types, we show here that how these NLI contributions can be obtained through (\ref{EGN_fixed}).    
\subsubsection{SCI}
To obtain an expression for the SCI contributed NLI, we need to consider the NLI caused by the  the COI on itself, leading to solely keep the terms in \eqref{EGN_fixed} generated by spectral lines located in the COI. Therefore, one may need to consider $\kappa_1=\kappa_2=\kappa_1+\kappa_2-\kappa+l=\kappa$, leading to $l=0$ and $\kappa_1=\kappa_2=\kappa$ in (\ref{EGN_fixed}). 

\subsubsection{XCI}
To compute the XCI terms through (\ref{EGN_fixed}), we proceed with the above addressed four types of XCI as follows: 
\begin{enumerate}
\item [X1:] The first XCI nonlinear contributions, X1, known as the XPM nonlinear terms, can be obtained from (\ref{EGN_fixed}) by considering islands with \{$\kappa_1=\kappa_1+\kappa_2-\kappa+l\neq \kappa$, $\kappa_2 = \kappa$\} and \{$\kappa_2=\kappa_1+\kappa_2-\kappa+l\neq \kappa$, $\kappa_1 = \kappa$\}, to realize the above mentioned XPM nonlinear interaction scenarios. Equivalently, we have \{$\kappa_2=\kappa$, $l=0$\} and \{$\kappa_1=\kappa$, $l=0$\}. As a simple example, the XPM NLI contribution on channel $\kappa$ stems from interfering channel $\kappa1$ is obtained by summing up as  
\eqlab{}
{
\sigma_{\text{XPM},\kappa}^{2}=&D_{\kappa}(\kappa_1,\kappa,0)+D_{\kappa}(\kappa,\kappa_1,0)+\Phi_{\kappa_1}\nonumber\\&E_\kappa(\kappa_1,\kappa,0)+\Phi_{\kappa_1}F_\kappa(\kappa,\kappa_1,0).
}

\item [X2:] The second XCI type nonlinear contribution can be obtained by considering islands with \{$\kappa_1=\kappa_1+\kappa_2-\kappa+l= \kappa$, $\kappa_2 \neq \kappa$\} and \{$\kappa_2=\kappa_1+\kappa_2-\kappa+l= \kappa$, $\kappa_1 \neq\kappa$\}. Equivalently, this nonlinear term caused by the interfering channel located at the left of the COI can be computed using \eqref{EGN_fixed} by considering islands with \{$l=1$, $\kappa_1=\kappa$,  $\kappa_2=\kappa-1$\} and \{$l=1$, $\kappa_2=\kappa$, $\kappa_1 =\kappa-1$\}. For instance, when channel $\kappa_1=\kappa-1$ at the left side of the COI ($l=1$) is interfering on the COI, the X2 terms is summed up as  
\eqlab{}
{
\sigma_{\text{X2},\kappa}^{2}=&D_{\kappa}(\kappa,\kappa-1,1)+D_{\kappa}(\kappa-1,\kappa,1)+\nonumber\\&\Phi_{\kappa}E_\kappa(\kappa,\kappa-1,1)+\Phi_{\kappa}F_\kappa(\kappa-1,\kappa,1).
}
For the X2 nonlinear term originated from the interfering channel located at the right of the COI ($l=-1$), we have
 \eqlab{}
{
\sigma_{\text{X2},\kappa}^{2}=&D_{\kappa}(\kappa,\kappa+1,-1)+D_{\kappa}(\kappa+1,\kappa,-1)+\nonumber\\&\Phi_{\kappa}E_\kappa(\kappa,\kappa+1,-1)+\Phi_{\kappa}F_\kappa(\kappa+1,\kappa,-1).
}
We notice here that $l=-1$ and $l=1$ represent the lower and upper triangle islands of each lozenge-shaped islands, respectively. 
\item [X3:] The third XCI type nonlinear contribution can be obtained by considering islands with \{$\kappa_1= \kappa_2=\kappa$, $\kappa_1+\kappa_2-\kappa+l= \kappa-1$\} and \{$\kappa_1= \kappa_2=\kappa$, $\kappa_1+\kappa_2-\kappa+l=\kappa+1$\}. Equivalently, this nonlinear term can be obtained from \eqref{EGN_fixed} by considering islands originating X3 terms \{$l=-1$, $\kappa_1=\kappa_2=\kappa$\} and  \{$l=1$, $\kappa_1=\kappa_2=\kappa$\}, resulting in 
\eqlab{}
{
\sigma_{\text{X3},\kappa}^{2}=D_{\kappa}(\kappa,\kappa,-1)+\Phi_{\kappa}G_\kappa(\kappa,\kappa,-1)
} 
and 
\eqlab{}
{
\sigma_{\text{X3},\kappa}^{2}=D_{\kappa}(\kappa,\kappa,+1)+\Phi_{\kappa}G_\kappa(\kappa,\kappa,+1),
}
respectively, for the above simple example.

\item [X4:] This nonlinear term  originated from islands with \{$\kappa_1= \kappa_2=\kappa_1+\kappa_2-\kappa+l= \kappa-1$\} and \{$\kappa_1= \kappa_2=\kappa_1+\kappa_2-\kappa+l= \kappa+1$\} or equivalently can be obtained from \eqref{EGN_fixed} by considering islands with \{$l=1$, $\kappa_1=\kappa_2=\kappa-1$\} and \{$l=-1$, $\kappa_1=\kappa_2=\kappa+1$\}, respectively, resulting in 
 \eqlab{}
{
&\sigma_{\text{X4},\kappa}^{2}=D_{\kappa}(\kappa-1,\kappa-1,1)+\Phi_{\kappa-1}\nonumber\\&E_\kappa(\kappa-1,\kappa-1,+1)+\Phi_{\kappa-1}F_\kappa(\kappa-1,\kappa-1,+1)+\nonumber\\&\Phi_{\kappa-1}G_{\kappa-1}(\kappa-1,\kappa-1,+1)+\Psi_{\kappa_1-1}\nonumber\\&H_\kappa(\kappa-1,\kappa-1,+1),
}
and 
 \eqlab{}
{
&\sigma_{\text{X4},\kappa}^{2}=D_{\kappa}(\kappa+1,\kappa+1,-1)+\Phi_{\kappa+1}\nonumber\\&E_\kappa(\kappa+1,\kappa+1,-1)+\Phi_{\kappa+1}F_\kappa(\kappa+1,\kappa+1,-1)+\nonumber\\&\Phi_{\kappa+1}G_\kappa(\kappa+1,\kappa+1,-1)+\Psi_{\kappa+1}\nonumber\\&H_\kappa(\kappa+1,\kappa+1,-1),
}
respectively, for the simple example.
\end{enumerate}
\subsubsection{MCI} 
To address this NLI contribution, we proceed with four types of MCI as follows: 
\begin{enumerate}
\item [M0:] The M0 NLI effect is originated form interfering spectral components located in three different channels, i. e.,  ($\kappa_1$, $\kappa_2$, $\kappa_1+\kappa_2-\kappa+l$), where $\kappa_1\neq \kappa_2$, $\kappa_1\neq\kappa_1+\kappa_2-\kappa+l$, and $\kappa_2\neq\kappa_1+\kappa_2-\kappa+l$. In other words, the M0 nonlinear contributions can be obtained from \eqref{EGN_fixed} considering islands with ($\kappa_1,\kappa_2$, $l$), where $\kappa_1\neq\kappa_2$, $\kappa\neq\kappa_2+l$, $\kappa\neq\kappa_1+l$.

\item [M12:] The M1 and M2 NLI effects are originated form interfering spectral components located in two different channels (which are different from the COI), i. e.,  ($\kappa_1$, $\kappa_2$, $\kappa_1+\kappa_2-\kappa+l$), where \{$\kappa_1=\kappa_1+\kappa_2-\kappa+l\neq\kappa_2$, $\kappa_1\neq\kappa$, $\kappa_2\neq\kappa$\} and \{$\kappa_2=\kappa_1+\kappa_2-\kappa+l\neq\kappa_1$, $\kappa_2\neq\kappa$, $\kappa_1\neq\kappa$\}. As a simple example,
the M1 and M2 nonlinear contributions can be obtained from \eqref{EGN_fixed} by considering islands with \{$l=-1$, $\kappa_2=\kappa+1\neq\kappa_1$, $\kappa_1\neq\kappa$\}, \{$l=1$, $\kappa_2=\kappa-1\neq\kappa_1$, $\kappa_1\neq\kappa$\}, \{$l=-1$, $\kappa_1=\kappa+1\neq\kappa_2$, $\kappa_2\neq\kappa$\}, and \{$l=1$, $\kappa_1=\kappa-1\neq\kappa_2$, $\kappa_2\neq\kappa$\} in  Fig.~\ref{LT} (b). In this case, the M1 and M2 terms are summing up as   
\eqlab{}
{
&\sigma_{\text{M1,M2},\kappa}^{2}=D_{\kappa}(\kappa_1,\kappa_1+1,-1)+D_{\kappa}(\kappa_1,\kappa-1,1)\nonumber\\&+\Phi_{\kappa_1}E_\kappa(\kappa_1,\kappa_1+1,-1)+\Phi_{\kappa_1-1}F_\kappa(\kappa_1,\kappa-1,1)\nonumber\\&+D_{\kappa}(\kappa+1,\kappa_2,-1)+D_{\kappa}(\kappa-1,\kappa_2,1)\nonumber\\&+\Phi_{\kappa_1}E_\kappa(\kappa_1,\kappa-1,1)+\Phi_{\kappa-2}F_\kappa(\kappa-1,\kappa_2,1).
}
 
\item [M3:]This last MCI term contributions can be obtained from \eqref{EGN_fixed} by considering islands with \{$\kappa_1=\kappa_2$, $\kappa_1+\kappa_2-\kappa+l>\kappa+1$, $\kappa_1+\kappa_2-\kappa+l<\kappa-1$\}. Equivalently, the M3 nonlinear contribution can be obtained from \eqref{EGN_fixed} by considering islands with \{$l=0$, $\kappa_1=\kappa_2$, $|\kappa-\kappa_1+\kappa_2-\kappa+l|>1$\}, \{$l=-1$, $\kappa_1=\kappa_2$, $|\kappa-\kappa_1+\kappa_2-\kappa+l|>1$\}, \{$l=1$, $\kappa_1=\kappa_2$, $|\kappa-\kappa_1+\kappa_2-\kappa+l|>1$\} in Fig.~\ref{LT}(b). For the example with two interfering channels located at the left of COI, where channels $\kappa_1$ and $\kappa_1+\kappa_2-\kappa+l=\kappa-2$ are interfering on the COI, and two interfering channels at the right of COI, namely channels $\kappa_1$ and $\kappa_1+\kappa_2-\kappa+l=\kappa+2$ are interfering on the COI, the M3 terms are summing up as 
\eqlab{}
{
&\sigma_{\text{M3},\kappa}^{2}=D_{\kappa}(\kappa-1,\kappa-1,0)+\Phi_{\kappa-1}G_\kappa(\kappa-1,\kappa-1,0)\nonumber\\&+D_{\kappa}(\kappa+1,\kappa+1,0)+\Phi_{\kappa+1}G_\kappa(\kappa+1,\kappa+1,0).
}
\end{enumerate}
\subsection{Comparison with previously introduced SRS models}

\subsubsection{The frequency domain SRS GN model proposed by Semrau et. al \cite{semrau2018gaussian}}

Interestingly, the terms $E_\kappa$, $F_\kappa$, $G_\kappa$, and $H_\kappa$ in this model are manifesting as correction terms to the GN model. More precisely, by considering the Gaussian assumption, the EGN model boils down to the GN model \cite{semrau2018gaussian}, resulting in disappearance of these correction terms and solely retaining the term ${D}_\kappa$.

\subsubsection{The modulation format dependent model proposed by Semrau et. al \cite{semrau2019modulation}}

Authors of \cite{semrau2019modulation} considered only SCI for  Gaussian signals and XPM for non-Gaussian signal. The SCI term for Gaussian signal therefore obtained through \eqref{EGN_fixed} by ignoring $E_\kappa$, $F_\kappa$, $G_\kappa$, and $H_\kappa$ terms and the interpretation of SCI described in the previous section. The XPM term for non-Gaussian signal is obtained from \eqref{EGN_fixed} by means of the interpretation presented in the previous section.

\subsubsection{The frequency domain EGN model introduced by Carena et. al \cite{carena2014egn}}

This model can be reduced to the EGN model presented in \cite{carena2014egn}, which is valid for C-band transmission, by putting $C_r\rightarrow 0$ and $\beta_3\rightarrow 0$ in $\mu(\cdot)$ and $\Phi(\cdot)$, resulting in 
\eqlab{mu_identical_nosrs}
{
&\mu(f_1,f_2,f)=\gamma\frac{1-e^{-2\alpha L}e^{j4\pi^{2}\beta_{2} (f_1-f)(f_2-f)L}}{2\alpha-j4\pi^{2}\beta_{2}(f_1-f)(f_2-f)}.
}

\subsubsection{The time domain EGN model introduced by Dar et. al \cite{dar2013properties}}

The closed form expression for the XPM nonlinear term along with a correction term which takes into account the non-Gaussianity of signal was proposed in \cite[Eqs.(25)--(27)]{dar2013properties}. The extraction of this equation through (\ref{EGN_fixed}) completely coincides with the extraction of X1 terms explained in the previous section with \eqref{mu_identical_nosrs}.

%Fig.~\ref{fig_MDS} shows the NLC of WDM channels  propagated within a link that composed of three different spans, namely two SMF fibers with different lengths and one non-zero dispersion shifted fiber (NZDSF) fiber.
%\section{Conclusion}\label{conclusion}
%An alternative EGN model expression was derived in order to take into account the combined nonlinear effects of SRS and Kerr-nonlinearity for lumped amplification systems with constant attenuation coefficient. The derived model is capable of accounting for the frequency dependent attenuation coefficient. This model can be applied for systems including both C and L bands, namely optical bandwidths beyond Stokes shift, and hybrid amplification systems as well. It was shown that the NLI being increased for channels endure net SRS gain and being decreased for channels endure net SRS loss. Moreover, we found that the nonlinear interference (NLI) varience deviation is increased and decreased exponentially, for low frequency and high frequency channels when the input launch power increases. On the other hand, the NLI variance deviations remain invariable except for high launch powers.

%The model is accurate for a wide range of modulation formats. Indeed, we remove the Gaussianity assumption of signal to derive an exact modulation format dependent EGN model in the presence of SRS. We show that Gaussian modulation experiences higher NLI than the other modulation formats, i.e., SRS GN model overestimates the nonlinear interference.
%The general EGN model has opened up a new horizon for efficient optimization of ultra-widebands systems.

==> Lemma1.2.tex <==
\section{Proof of Theorem \ref{main.result}}\label{AppendixB}

This appendix contains two sections. In the first section, we derive the nonlinear electrical field in \eqref{MAN_NLI_sol} at the end of a link with multiple different spans. The second section provides the derivation of the NLI PSD in \eqref{SpecDensityDP_Def}, which is then used to compute the nonlinear power via \eqref{NLI_Power_Channel_Kappa}.
%This appendix addresses derivation of the the NLI power of a certain channel \eqref{NLI_Power_Channel_Kappa}, starting from the NLI PSD on polarization x \eqref{G_x_Def}.
%\eqlab{G_x_Def}
%{
%G_{\small{\text{NLI}},\text{x},\kappa}(f)=\mathbb{E}\big\{E_{\text{x},\kappa}^{(1)}(f)\text{e}^{(1)*}_{\text{x},\kappa}(f)\big\},
%}
 %where $E_{\text{x},\kappa}^{(1)}(f)$ is provided assuming that the nonlinear electrical filed of each span propagates solely linearly until arrives at the output of the link. This assumption is driven by the perturbation approach. The linear propagation of the nonlinear electrical fields of the different link spans at the receiver are summed up coherently.
 \subsection{Nonlinear Electrical Field}% at the end of fiber}
 
In this section we first derive the nonlinear electrical field at the end of first span (Lemma~\ref{NLI_field_first_span} ahead). We then extend it to multiple different spans (Lemma~\ref{multiple.span.extention} ahead).
\begin{lemma}[Nonlinear Field: First Span]\label{NLI_field_first_span}
The nonlinear electrical field at the end of the first span of length $L_1$ is given by
\begin{equation}\label{NLIN_expression}
\begin{split}
&E_{\text{x},\kappa}^{(1)}(L_{1},f)=-j\gamma\frac{8}{9}f_0^{3/2}\text{e}^{\tilde{\Gamma}(L_{1},f)}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\\&\cdot\delta(f-if_0-(\kappa-l)R)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\\&\cdot\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\zeta_{\kappa_1,\kappa_2,\kappa}(m,n,k),
\end{split}
\end{equation}
where  
 \begin{equation}\label{Zeta_ENL}
 \begin{split}
\zeta_{\kappa_1,\kappa_2,\kappa}(m,n,k)=&\int_{0}^{L_{1}}\text{d}z'\sqrt{\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')}\\&\cdot \text{e}^{j\phi_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')},
\end{split}
\end{equation}
in which
\begin{equation}\label{varrho}
\begin{split}
&\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')=\rho(z',mf_0+\kappa_1 R)\\&\cdot\frac{\rho(z',nf_0+(\kappa_1+\kappa_2-\kappa+l)R)\rho(z',kf_0+\kappa_2 R)}{\rho(z',(m+k-n)f_0+(\kappa-l)R)},
\end{split}
\end{equation}
and
 \begin{equation}\label{phi}
 \begin{split}
&\phi_{m,n,k}(\kappa_1,\kappa_2,\kappa)=4\pi^{2}\Big((m-n)f_0+(\kappa-\kappa_2-l)R\Big)\\&\cdot\Big((k-n)f_0+(\kappa-\kappa_1-l)R\Big)\Big[\beta_{2,1}+\pi\beta_{3,1}\\&\cdot\big[(m+k)f_0+(\kappa_1 +\kappa_2 )R\big]\Big]z',
\end{split}
 \end{equation}
 where $\tilde{\Gamma}(\cdot)$, $\xi$, and $\rho(\cdot)$ defined in \eqref{gamma.tilde}, \eqref{FourierSerisCoef1}, and \eqref{rho}, respectively.
\end{lemma}
\begin{IEEEproof}
The nonlinear electrical field ${\boldsymbol{E}}^{(1)}(z,f)$ is given by \eqref{MAN_NLI_sol}, which depends on the Kerr term ${\boldsymbol{Q}}(z,f)$ in \eqref{F_kerr}, which in turn depends on the linear solution of the Manakov equation ${\boldsymbol{E}}^{(0)}(z,f)$. The x-polarization part of the latter can be expressed as
\eqlab{Lin_electrical_z}{
E_{\text{x}}^{(0)}(z,f)=\sqrt{f_0}\text{e}^{\tilde{\Gamma}(z,f)}\sum_{\kappa=1}^{M}\sum_{n=-\infty}^{\infty}\xi_{\text{x},\kappa,n}\delta(f-nf_0-\kappa R),
}
where we used \eqref{FouierSeries} in \eqref{E_input} and in \eqref{MAN_LIN_sol}.

By using \eqref{Lin_electrical_z} into \eqref{F_kerr}  yields
\eqlab{eq_6_1}{
&Q_{\text{x},\kappa}(z,f)=-j\gamma\frac{8}{9}\Big[\nonumber\\
&f_0\Big(\text{e}^{\tilde{\Gamma}(z,f)}\sum_{\kappa_1=1}^{M}\sum_{m=-\infty}^{\infty}\xi_{\text{x},\kappa_1,m}\delta(f-mf_0-\kappa_1R)\Big)\nonumber\\
&*\Big(\text{e}^{\tilde{\Gamma}^*(z,f)}\sum_{\kappa'=1}^{M}\sum_{n=-\infty}^{\infty}\xi^*_{\text{x},\kappa',n}\delta(-f-nf_0-\kappa'R)\Big)+ \nonumber\\
&f_0\Big(\text{e}^{\tilde{\Gamma}(z,f)}\sum_{\kappa_1=1}^{M}\sum_{m=-\infty}^{\infty}\xi_{\text{y},\kappa_1,m}\delta(f-mf_0-\kappa_1R)\Big)\nonumber\\
&\Big(\text{e}^{\tilde{\Gamma}^*(z,f)}\sum_{\kappa'=1}^{M}\sum_{m=-\infty}^{\infty}\xi^*_{\text{y},\kappa',n}\delta(-f-nf_0-\kappa'R)\Big)\Big]*\nonumber\\
&\sqrt{f_0}\Big(\text{e}^{\tilde{\Gamma}(z,f)}\sum_{\kappa_2=1}^{M}\sum_{k=-\infty}^{\infty}\xi_{\text{x},\kappa_2,k}\delta(f-kf_0-\kappa_2R)\Big).
}
We now use the property
\eqlab{delta.property}{
&a(f)\delta(f-f_a)*b(f)\delta(-f-f_b)*c(f)\delta(f-f_c)=\nonumber\\&a(f_a)b(f_b)c(f_c)\delta(f-(f_a-f_b+f_c)),
}
to express \eqref{eq_6_1} as
\begin{equation}\label{eq_6_1_1}
\begin{split}
&Q_{\text{x},\kappa}(z,f)=-j\gamma\frac{8}{9}f_0^{3/2}\sum_{\kappa_1=1}^{M}\sum_{\kappa'=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{ m=-\infty}^{\infty}\sum_{n=-\infty}^{\infty}\sum_{ k=-\infty}^{\infty}\\&\cdot\delta\big(f-(m-n+k)f_0-(\kappa_1-\kappa'+\kappa_2) R\big)\\&\cdot\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa',n}^{*}\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa',n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\\&\cdot \text{e}^{\tilde{\Gamma}(z,mf_0+\kappa_1 R)+\tilde{\Gamma}^*(z,nf_0+\kappa' R)+\tilde{\Gamma}(z,kf_0+\kappa_2 R)}.
\end{split}
\end{equation}
We are interested in the NLI in channel $\kappa$, which imposes the  constraint on the interfering  frequency $if_0+\tau R$ 
%Similar to \cite{carena2014egn,MecozziEssiambre2012,Pontus_JLT_modeling_2013} we remove the triplets 
%where $m=n$ and $n=k$ because they create bias and non-fluctuating terms (see Lemma~\ref{bias.terms} ahead in the next section). We therefore define the non-bias triplets as
\begin{equation}\label{si}
\mathcal{S}_i=\left\{(m,n,k)\in\mathbb{Z}^3:\kappa R-\frac{R}{2}\leq if_0+\tau R\leq \kappa R+\frac{R}{2}\right\},
\end{equation}
where $i=m-n+k$ and $\tau=\kappa_1-\kappa'+\kappa_2$.
%\eqlab{f.constraint}{
%\kappa R-R/2\leq f \leq\kappa R +R/2.} 
In other words, for given values of $\kappa_1,\kappa',\kappa_2$,  only certain values of $m,n,k$ are allowed, namely those in the set $\mathcal{S}_i$.
 Using \eqref{si}, \eqref{eq_6_1_1} is expressed as
\begin{equation}\label{eq_6_si}
\begin{split}
&Q_{\text{NLI,x},\kappa}(z,f)=
-j\gamma\frac{8}{9}f_0^{3/2}\sum_{\kappa_1=1}^{N}\sum_{\kappa'=1}^{N}\sum_{\kappa_2=1}^{N}\sum_{i=-\infty}^{\infty}\\
&\cdot\delta(f-if_0-\tau R)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa',n}^{*}\xi_{\text{x},\kappa_2,k}+\\
&\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa',n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\\
&\cdot \text{e}^{\tilde{\Gamma}(z,mf_0+\kappa_1 R)+\tilde{\Gamma}^*(z,nf_0+\kappa' R)+\tilde{\Gamma}(z,kf_0+\kappa_2 R)}.
\end{split}
\end{equation}
%Since $-R/2\leq nf_0\leq R/2$, we find that $-3/2R\leq(m-n+k)f_0\leq3/2R$, and hence
%According to \eqref{FouierSeries}--\eqref{f0.constraint} given in Sec.~\ref{preliminaries},  $nf_0+\kappa R$ is a frequency component within channel $\kappa$. The same is true for \eqref{eq_6_1} in which $mf_0+\kappa_1R$, $nf_0+\kappa'R$, and $kf_0+\kappa_2R$ are the frequency components within channels $\kappa_1$, $\kappa'$, and $\kappa_2$, respectively, where
The expression \eqref{FourierSerisCoef1} shows that $nf_0+\kappa R$ corresponds to the frequency components within channel $\kappa$. Because of this, $nf_0$ should satisfy \eqref{f0.constraint}. A similar interpretation can be used on $mf_0+\kappa_1R$, $nf_0+\kappa'R$, and $kf_0+\kappa_2R$ in \eqref{eq_6_1}, and thus,
\begin{align*}
-\frac{R}{2}\leq mf_0 \leq \frac{R}{2},\quad
-\frac{R}{2}\leq nf_0 \leq\frac{R}{2},\quad
-\frac{R}{2}\leq kf_0 \leq\frac{R}{2}.
\end{align*}
By combining these inequalities we get $-3/2R\leq(m-n+k)f_0 \leq3/2R$, which implies that
%We now combine \eqref{f0.constraint} and \eqref{f.constraint} to obtain $-3/2R\leq(m-n+k)f_0\leq3/2R$ [THIS IS NOT TRUE. PLEASE FIX IT. What equations do you combine to get $-3/2R\leq(m-n+k)f_0\leq3/2R$?]
\begin{equation}\label{interference_limit}
-\frac{3}{2}R
+\tau R \leq if_0+\tau R \leq \frac{3}{2}R
+\tau R.
\end{equation}
Combining the inequalities in the definition of the set $\mathcal{S}_i$ in \eqref{si} with \eqref{interference_limit}, we obtain\footnote{To obtain \eqref{boundary.kappa'}, we use the fact that for any $a,b,c,x
\in\mathbb{R}$ the two inequalities $b-a/2\leq x \leq b+a/2$ and $-3a/2+c\leq x \leq 3a/2+c$, imply that $b>-2a+c$ and $b<2a+c$.}
% \begin{equation}\label{interfernce_bound}
% \begin{split}
% &\kappa R+\frac{R}{2}>-\frac{3}{2}R
% +(\kappa_1-\kappa'+\kappa_2)R,\\&\kappa R-\frac{R}{2}<\frac{3}{2}R
% +(\kappa_1-\kappa'+\kappa_2)R,
% \end{split}
% \end{equation}
% and thus,
\eqlab{boundary.kappa'}{
&\kappa-2<\kappa_1-\kappa'+\kappa_2<\kappa+2.
}
The expression in \eqref{boundary.kappa'} in turn implies that for given values of $\kappa,\kappa_1,$ and $\kappa_2$, $\kappa'$ can only take the following three values
\eqlab{kappa'.l}{
\kappa'=\kappa_1+\kappa_2-\kappa+l, \quad l=-1,0,1.%\\&
%\kappa'=\kappa_1+\kappa_2-\kappa+0,\\&
%\kappa'=\kappa_1+\kappa_2-\kappa+1,
}
% thereby 
% (\ref{eq_6_si}) which has the overall form
% \eqlab{eq_6_si_alternative1}{
% Q_{\text{NLI,x},\kappa}(z,f)=\sum_{\kappa_1=1}^{N}\sum_{\kappa'=1}^{N}\sum_{\kappa_2=1}^{N}X_{\kappa_1}(z,f)Y_{\kappa'}(z,f)Z_{\kappa_2}(z,f),
% }
% can be written as
% \eqlab{eq_6_si_alternative2}{
% Q_{\text{NLI,x},\kappa}(z,f)=&\sum_{\kappa_1=1}^{N}\sum_{\kappa_2=1}^{N}\sum_{\l=-1}^{1}X_{\kappa_1}(z,f)Y_{\kappa_1+\kappa_2-\kappa+l}(z,f)\nonumber\\&Z_{\kappa_2}(z,f),
% }
Using \eqref{kappa'.l}, we express \eqref{eq_6_si} as
\begin{equation}\label{qx_2}
\begin{split}
&Q_{\text{x},\kappa}(z,f)=-j\gamma\frac{8}{9}f_0^{3/2}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\\&\delta\big(f-if_0-(\kappa-l)R\big)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\\&\cdot\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\\&\cdot \text{e}^{\tilde{\Gamma}(z,mf_0+\kappa_1 R)+\tilde{\Gamma}^*(z,nf_0+(\kappa_1+\kappa_2-\kappa+l) R)+\tilde{\Gamma}(z,kf_0+\kappa_2 R)}.
\end{split}
\end{equation}
%and its y-polarization counterpart is
%\footnote{Without loss of generality we indexed the second terms of \eqref{qx_2} and \eqref{qy_2} in the following form
%\eqlab{indexing}{
%&\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k},\nonumber\\&
%\xi_{\text{y},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k},
%}
%because in the next section we show that to calculate the NLI PSD the first and second terms of \eqref{indexing} result in 
%\eqlab{indexing.moments1}{
%&\mathbb{E}\{\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{y},\kappa_1,m}^{*}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}\}\nonumber\\&\cdot\mathbb{E}\{\xi_{\text{x},\kappa_2,k}\xi_{\text{x},\kappa_2,k}^{*}\},
%}
%and
%\eqlab{indexing.moments2}{
%&\mathbb{E}\{\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1,m'}^{*}\}\cdot\nonumber\\&\mathbb{E}\{\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n'}^{*}\xi_{\text{x},\kappa_1,k}\xi_{\text{x},\kappa_1,k'}^{*}\},
%}
%respectively. As can be seen in \eqref{indexing.moments1} the second expectation, which yields the second order moments, is taken over channel $\kappa_2$, whereas in \eqref{indexing.moments2} the first expectation that results in the second order moments, is taken over channel $\kappa_1$.
%}
%\begin{equation}\label{qy_2}
%\begin{split}
%&Q_{\text{y},\kappa}(z,f)=-j\gamma\frac{8}{9}f_0^{3/2}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\\&\cdot\delta\big(f-if_0-(\kappa-l)R\big)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\\&\cdot\xi_{\text{y},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\\&\cdot \text{e}^{\tilde{\Gamma}(z,mf_0+\kappa_1 R)+\tilde{\Gamma}^*(z,nf_0+(\kappa_1+\kappa_2-\kappa+l) R)+\tilde{\Gamma}(z,kf_0+\kappa_2 R)}.
%\end{split}
%\end{equation}
We now use \eqref{qx_2} in \eqref{MAN_NLI_sol} to obtain the nonlinear electrical field on x-polarization at the end of the first fiber span of length $L_{1}$, which gives
%\eqref{NLIN_expression_x_1}.
%\eqref{NLIN_expression}.
%\begin{figure*}
%\small
\begin{equation}\label{NLIN_expression_x_1}
\begin{split}
&E_{\text{x},\kappa}^{(1)}(L_{1},f)=-j\gamma\frac{8}{9}f_0^{3/2}\text{e}^{\tilde{\Gamma}(L_{1},f)}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\\&\cdot\delta(f-if_0-(\kappa-l)R)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\\&\cdot\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}
\Big)\int_{0}^{L_1}\text{d}z'\\&\cdot \text{e}^{\tilde{\Gamma}(z',mf_0+\kappa_1 R)}\cdot\text{e}^{\tilde{\Gamma}^*(z',nf_0+(\kappa_1+\kappa_2-\kappa+l) R)}\\&\cdot\text{e}^{\tilde{\Gamma}(z',kf_0+\kappa_2 R)}\cdot\text{e}^{-\tilde{\Gamma}(z',(m-n+k)f_0+(\kappa-l)R)},
\end{split}
\end{equation}
where in the last exponential we replaced $f$ by $(m-n+k)f_0+(\kappa-l)R$ due to the delta function $\delta(f-if_0-(\kappa-l)R)$ multiplying the sum and integral in \eqref{NLIN_expression_x_1}. 

The last part of the proof is to show that the integral in \eqref{NLIN_expression_x_1} can be expressed as \eqref{Zeta_ENL} and \eqref{varrho}. We do this by first 
%\hrulefill
%\end{figure*}
substituting \eqref{gamma} into \eqref{gamma.tilde}, and taking exponentials on both sides of the resulting equation gives
% we have
% \eqlab{gamma.tilde.expansion}{
% \tilde{\Gamma}(z,f)=\int_{0}^{z}\text{d}z'\Big[\frac{g(z',f)}{2}+j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3\Big],
% }
% and therefore,
\begin{align}
\label{exp.gamma.tilde.expansion}
\text{e}^{\tilde{\Gamma}(z,f)}&=\text{e}^{\frac{1}{2}\int_{0}^{z}\text{d}z'g(z',f)}\cdot\text{e}^{\int_{0}^{z}\text{d}z'[j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3]}\\
\label{exp.gamma.tilde.expansion.2}
&=\sqrt{\rho(z,f)} \cdot\text{e}^{[j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3]z}
\end{align}
where the first term in \eqref{exp.gamma.tilde.expansion.2} follows from the definition of the normalized signal power profile definition in \eqref{rho.1} and the second from the fact that $\beta_{2,1}$ and $\beta_{3,1}$ are $z$-indepent.% the first term is equal to
%\eqlab{first.term.gamma.tilde}{
%\text{e}^{\int_{0}^{z}\text{d}z'\frac{g(z',f)}{2}}=, %\quad \text{and}\nonumber\\&
%\text{e}^{-\int_{0}^{z}\text{d}z'\frac{g(z',f)}{2}}=\frac{1}{\sqrt{\rho(z,f)}},
%}

%and the second term is 
%\eqlab{second.third.exp.gamma.tilde}{
%\text{e}^{\int_{0}^{z}\text{d}z'[j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3]}=\text{e}^{[j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3]z}.
%%}
%By inserting \eqref{first.term.gamma.tilde} and \eqref{second.third.exp.gamma.tilde} into \eqref{exp.gamma.tilde.expansion}, we get
%\eqlab{exp.gamma.tilde.expansion.2}{
%\text{e}^{\tilde{\Gamma}(z,f)}=\sqrt{\rho(z,f)}\cdot \text{e}^{[j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3]z},
%}

We now use \eqref{exp.gamma.tilde.expansion.2} to express the integral in \eqref{NLIN_expression_x_1} as
\eqlab{last.four.terms.exp.gamma}{
&\int_{0}^{L_1}\text{d}z'\text{e}^{\tilde{\Gamma}(z',mf_0+\kappa_1 R)}\cdot\text{e}^{\tilde{\Gamma}^*(z',nf_0+(\kappa_1+\kappa_2-\kappa+l) R)}\nonumber\\&\cdot\text{e}^{\tilde{\Gamma}(z',kf_0+\kappa_2 R)}\cdot\text{e}^{-\tilde{\Gamma}(z',(m-n+k)f_0+(\kappa-l)R)}=\nonumber\\&
\int_{0}^{L_1}\text{d}z'\sqrt{\rho(z',mf_0+\kappa_1 R)}\nonumber\\&\cdot\frac{\sqrt{\rho(z',nf_0+(\kappa_1+\kappa_2-\kappa+l)R)}\sqrt{\rho(z',kf_0+\kappa_2 R)}}{\sqrt{\rho(z',(m-n+k)f_0+(\kappa-l)R)}}\nonumber\\&\cdot
\text{e}^{[j2\pi^{2}\beta_{2,1} (mf_0+\kappa_1R)^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}(mf_0+\kappa_1R)^3]z'}
\nonumber\\&
\text{e}^{[-j2\pi^{2}\beta_{2,1} (nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{2}-j\frac{4}{3}\pi^3 \beta_{3,1}(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^3]z'}
\nonumber\\&
\text{e}^{[j2\pi^{2}\beta_{2,1} (kf_0+\kappa_1R)^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}(kf_0+\kappa_2R)^3]z'}
\nonumber\\&
\text{e}^{[-j2\pi^{2}\beta_{2,1} (( m-n+k)f_0+(\kappa-l)R)^{2}-j\frac{4}{3}\pi^3 \beta_{3,1}((m-n+k)f_0+(\kappa-l)R)^3]z'}.
}
% in which we are using the fact that
% \eqlab{exp.gamma.tilde.expansion.3.minus}{
% \text{e}^{-\tilde{\Gamma}(z,f)}= \frac{\text{e}^{[j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3]z}}{\sqrt{\rho(z,f)}}.
% }
We recognize the $\rho(\cdot)$ terms in the right hand side of \eqref{last.four.terms.exp.gamma} as $\sqrt{\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')}$,
% \eqlab{last.four.terms.exp.gamma.rho.terms}{
% &
% \sqrt{\rho(z',mf_0+\kappa_1 R)}\cdot\sqrt{\rho(z',nf_0+(\kappa_1+\kappa_2-\kappa+l)}\nonumber\\&\cdot\frac{\sqrt{\rho(z',kf_0+\kappa_2 R)}}{\sqrt{\rho(z',(m-n+k)f_0+(\kappa-l)R)}}=\nonumber\\&\sqrt{\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')},
% }
where $\varrho(\cdot)$ is given by \eqref{varrho}. In view of \eqref{Zeta_ENL}, the last step in the proof is therefore to show that
%Considering \eqref{rho}, it is straightforward that
%\eqlab{e.rho}{
%&\text{e}^{\int_{0}^{z’}\text{d}z” \frac{g(z”,mf_0+\kappa_1R)}{2}
%+\int_{0}^{z’}\text{d}z” \frac{g(z”,mf_0+\kappa_1R)}{2}+\int_{0}^{z’}\text{d}z” \frac{g(z”,mf_0+\kappa_1R)}{2}}\nonumber\\&\cdot
%\text{e}^{\int_{0}^{z’}\text{d}z” \frac{g(z”,(m-n+k)f_0+(\kappa-l)R)}{2}
%}
%\nonumber\\&=\int_{0}^{L_{1}}\text{d}z'\sqrt{\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')},
%}
%where $\varrho(\cdot)$ is given by \eqref{varrho}.
%On the other hand, using the fact that
%\eqlab{beta2.beta3.expansion}{
%& A^2-B^2+C^2-(A-B+C)^2=\nonumber\\&
%2(A-B)(C-B),\nonumber\\&
%A^3-B^3+C^3-(A-B+C)^3=\nonumber\\&3(A+C)(A-B)(C-B),
%}
%it is found that
the arguments of the four exponentials in \eqref{last.four.terms.exp.gamma} corresponds to \eqref{phi}. We do this by first grouping the quadratic and cubic terms in the exponentials in \eqref{last.four.terms.exp.gamma} as
\eqlab{beta2.beta3.expon}{
%&\text{e}^{[j2\pi^{2}\beta_2 (mf_0+\kappa_1R)^{2}+j\frac{4}{3}\pi^3 \beta_3(mf_0+\kappa_1R)^3]z’}
%\nonumber\\&
%\text{e}^{[-j2\pi^{2}\beta_2 (nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{2}-j\frac{4}{3}\pi^3 \beta_3(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^3]z’}
%\nonumber\\&
%\text{e}^{[j2\pi^{2}\beta_2 (kf_0+\kappa_1R)^{2}+j\frac{4}{3}\pi^3 \beta_3(kf_0+\kappa_2R)^3]z’}
%\nonumber\\&
%&\text{e}^{[-j2\pi^{2}\beta_2 (( m-n+k)f_0+(\kappa-l)R)^{2}-j\frac{4}{3}\pi^3 \beta_3( m-n+k)f_0+(\kappa-l)R)^3]z’}\nonumber\\&=
&\text{exp}\Big(j2\pi^{2}\beta_{2,1}z'\Big[ (mf_0+\kappa_1R)^{2}- (nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{2}\nonumber\\&+ (kf_0+\kappa_1R)^{2}- (( m-n+k)f_0+(\kappa-l)R)^{2}\Big]\Big)\nonumber\\&\cdot
\text{exp}\Big(j\frac{4}{3}\pi^3 \beta_{3,1}z'\Big[(mf_0+\kappa_1R)^3-\nonumber\\&(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^3+(kf_0+\kappa_2R)^3\nonumber\\&-( m-n+k)f_0+(\kappa-l)R)^3\Big]\Big).
}
We now use the equality
\begin{align*}
& A^2-B^2+C^2-(A-B+C)^2=
2(A-B)(C-B),
\end{align*}
to express the first exponential term in \eqref{beta2.beta3.expon} as
\eqlab{first.exponential.beta2}{
&\text{exp}\Big(j4\pi^{2}\beta_{2,1}z'\Big[ 
\Big((m-n)f_0+(\kappa-\kappa_2-l)R\Big)\nonumber\\&\cdot\Big((k-n)f_0+(\kappa-\kappa_1-l)R\Big)\Big]\Big).
}
We also use
\begin{align*}
A^3-B^3+C^3-&(A-B+C)^3\\
&=3(A-B)(C-B)(A+C),
\end{align*}
to express the second exponential term in \eqref{beta2.beta3.expon} as
\eqlab{second.exponential.beta2}{
&\text{exp}\Big(j4\pi^3\beta_{3,1}z'\Big[\Big((m-n)f_0+(\kappa-\kappa_2-l)R\Big)\nonumber\\&\cdot\Big((k-n)f_0+(\kappa-\kappa_1-l)R\Big)\nonumber\\&\cdot\Big((m+k)f_0+(\kappa_1 +\kappa_2 )R\Big)\Big]\Big).
}
The proof is completed by multiplying \eqref{first.exponential.beta2} and  \eqref{second.exponential.beta2} yielding the required exponential in \eqref{phi}.

%terms of %\eqref{beta2.beta3.expon}, 
%we find that \eqref{beta2.beta3.expon} can be rewritten as
% \eqlab{e.phi}{
%  \text{e}^{j\phi_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')},
%  }
% %\text{e}^{j\phi_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')}
% where $\phi(\cdot)$ is given by \eqref{phi}, and hence \eqref{last.four.terms.exp.gamma} is expressed as \eqref{Zeta_ENL}
% As a result, replacing the integral term of \eqref{NLIN_expression_x_1} (i.e., \eqref{last.four.terms.exp.gamma.rho.terms}) by \eqref{Zeta_ENL}  results in \eqref{NLIN_expression}.
%Now, considering \eqref{e.rho}, \eqref{beta2.beta3.expon}, and \eqref{exp.expression} and substituting \eqref{exp.expression} in \eqref{NLIN_expression_x_1}, we obtain \eqref{NLIN_expression}. 
%This completes the proof.
\end{IEEEproof}
%\begin{equation}\label{NLIN_expression}
%\begin{split}
%&E_{\text{x},\kappa}^{(1)}(L_{1},f)=-j\gamma\frac{8}{9}f_0^{3/2}\text{e}^{\tilde{\Gamma}(L_{1},f)}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\\&\cdot\delta(f-if_0-(\kappa-l)R)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\\&\cdot\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\zeta_{\kappa_1,\kappa_2,\kappa}(m,n,k),
%\end{split}
%\end{equation}
%where  
% \begin{equation}\label{Zeta_ENL}
% \begin{split}
%\zeta_{\kappa_1,\kappa_2,\kappa}(m,n,k)=&\int_{0}^{L_{1}}\text{d}\varsigma\sqrt{\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,\varsigma)}\\&\cdot \text{e}^{j\phi_{\kappa_1,\kappa_2,\kappa}(m,n,k,\varsigma)},
%\end{split}
%\end{equation}
%in which
%\begin{equation}
%\begin{split}
%&\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,\varsigma)=\rho(\varsigma,mf_0+\kappa_1 R)\\&\cdot\rho(\varsigma,nf_0+(\kappa_1+\kappa_2-\kappa+l)R)\rho(\varsigma,kf_0+\kappa_2 R)\\&\cdot\frac{1}{\rho(\varsigma,(m+k-n)f_0+(\kappa-l)R)},
%\end{split}
%\end{equation}
%with
%\begin{equation}
%\rho(z,f)=\text{e}^{\int_{0}^{z}\text{d}z' g(z',f)},
%\end{equation}
%and
 %\begin{equation}\label{phi}
 %\begin{split}
%&\phi_{m,n,k}(\kappa_1,\kappa_2,\kappa)=4\pi^{2}\Big((m-n)f_0+(\kappa-\kappa_2-l)R\Big)\\&\cdot\Big((k-n)f_0+(\kappa-\kappa_1-l)R\Big)\Big[\beta_{2,1}+\pi\beta_{3,1}\\&\cdot(mf_0+kf_0+\kappa_1 R+\kappa_2 R)\Big]\varsigma.
%\end{split}
% \end{equation}

 We now extend Lemma~\ref{NLI_field_first_span} to multiple different spans.
 \begin{lemma}[Nonlinear Field: Multiple Spans]\label{multiple.span.extention}
 The total nonlinear electrical field at the end of a link with $N$ multiple different spans can be written as
%\subsubsection{Nonlinear Electrical Field}\label{nonlinear solution}
%\eqlab{E_f}
%{
%{\bf E}_{\text{LIN}}(0,f)=\sum_{\kappa=1}^{N}{\bf A}_{\kappa}(f).
%} 
%To compensate for the fiber attenuation, an Erbium doped fiber amplifier (EDFA) is exploited at the end of each span, e. g., an EDFA with a gain of $g_{s}$ at span $s$. The nonlinear electrical field of channel $\kappa$ on x-polarization (readily can be written for y-polarization as well), denoted by $E_{\text{NLI},\text{x},\kappa}$, at the output of the link, i. e., is computed after the last EDFA amplifier in the last span $N$, as depicted in Fig.~\ref{Multi_span}. The derivation details of $E_{\text{NLI},\text{x},\kappa}$ is provided in Appendix \ref{AppendixA}, resulting in 
\eqlab{NLI_elec_tot_detail}
{
&E_{\text{x},\kappa}^{(1)}({\scriptstyle{\sum_{s'=1}^{N}\!L_{s'}}},f)\!=\!-j\frac{8}{9}f_0^{3/2}  \sum_{\kappa_1=1}^{M}
\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}
\sum_{i=-\infty}^{\infty}\nonumber\\&\delta\big(f\!-\!if_0\!-(\kappa-l)\big)\!\!\sum_{m,n,k\in \mathcal{S}_i}
\big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}+\nonumber\\&\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\big)\varsigma_{{\kappa_1},\kappa_2,\kappa}(m,n,k)\nonumber\\&\
\text{e}^{-j2\pi^{2}(if_0+(\kappa-1)R)^{2}\sum_{s=1}^{N}(\beta_{2,s}L_{s}+\frac{2}{3}\pi(if_0+(\kappa-1)R)L_{s})} ,
}
where $\sum_{s'=1}^{N}\!L_{s'}$ is the total length of link and
\eqlab{varsigma}
{
&\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,k)=\sum_{s=1}^{N}\gamma_{s}g_{s}^{1/2}\sqrt{\rho(z,if_0+(\kappa-l)R)}\nonumber\\&\prod_{s'=1}^{s-1}[g_{s'}\cdot\rho(L_{s'},f)]^{3/2}\prod_{s'=s}^{N}[g_{s'}\cdot\rho(L_{s'},f)]^{1/2}\zeta_{\kappa_1,\kappa_2,\kappa}^{s}(m,n,k)\nonumber\\&\text{exp}\Big(j4\pi^{2}\big((m-n)f_0+(\kappa-\kappa_2-l)R\big) \big((k-n)f_0+\nonumber\\&(\kappa-\kappa_1-l)R\big)\sum_{s'=1}^{s-1}\beta_{2,s'}L_{s'}+\pi[(m+k)f_0+\nonumber\\&(\kappa_1+\kappa_2)R]\beta_{3,s'}L_{s'}\Big),
}
in which
\eqlab{Zeta_ENL_s}{
\zeta^{s}_{\kappa_1,\kappa_2,\kappa}(m,n,k)=&\int_{0}^{L_{s}}\text{d}z'\sqrt{\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')}\\&\cdot \text{e}^{j\phi_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')},
}
where $g_{s}$ is the gain of amplifier located at the end of span $s$, $\varrho(\cdot)$ and $\phi(\cdot)$ are given in \eqref{varrho} and \eqref{phi}, respectively.
\end{lemma}
 
 \begin{IEEEproof}
 To evaluate the nonlinear electrical field of channel $\kappa$ at the end of the link with multiple different spans, similar to \cite{Carena2012}, we assume that the nonlinear contributions that distort channel $\kappa$ in each span propagate linearly in the following spans until arrive at the receiver. 
%Two approaches can be attended to sum all these nonlinear contributions at the receiver. One may sum the nonlinear contributions generated in each span at the receiver in power, namely in incoherent manner, 
%while the other way which is considered in this paper,
We sum all the nonlinear contributions generated in each span at the receiver coherently. In other words, the nonlinear electrical field of channel $\kappa$ at the end of the link with $N$ different spans is equal to
\eqlab{NLI_elec_tot}
{
E_{\text{x},\kappa}^{(1)}({\scriptstyle\sum_{s'=1}^{N}L_{s'}},f)=\sum_{s=1}^{N}E_{s,\text{x},\kappa}^{(1)}({\scriptstyle\sum_{s'=1}^{N}L_{s'}},f),
}
where $E_{s,\text{x},\kappa}^{(1)}({\scriptstyle\sum_{s'=1}^{N}L_{s'}},f)$ is the nonlinear electrical field of channel $\kappa$ at the receiver that generated in span $s$.
In order to evaluate the nonlinear electrical field of channel $\kappa$ that generated in span $s$, we assume that the signal propagates linearly in the first $s-1$  spans, namely the linear electrical field at the input of span $s$ is
\eqlab{LIN_elec_span}{
E_{s,\text{x}}^{(0)}({\scriptstyle\sum_{s'=1}^{s-1}L_{s'}},f)&=\prod_{s'=1}^{s-1}\sqrt{g_{s'}}\cdot\text{e}^{\tilde{\Gamma}_s(L_{s'},f)}E_{\text{x}}(0,f),
}
where
\eqlab{gamma.tilde.s}{
\tilde{\Gamma}_s(z,f)=\int_{0}^{z}\text{d}z'{\Gamma}_s(z',f),
}
in which
\begin{equation}\label{gamma.s}
{\Gamma}_s(z,f)=\frac{g(z,f)}{2}+j2\pi^{2}\beta_{2,s} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,s}f^3. 
\end{equation}
and $E_{\text{x}}(0,f)$ is given by \eqref{E_input} and \eqref{FouierSeries}.
This equation represents that the electrical field that passes through $s-1$ spans simply influenced by dispersions of spans, span losses, and amplifier gains. The linear field in the span $s$ can then be written as
\eqlab{LIN_elec_z}{
&E_{s,\text{x}}^{(0)}(z,f)=\text{e}^{\tilde{\Gamma}_s(z,f)}E_{s,\text{x}}^{(0)}({\scriptstyle\sum_{n_s'=1}^{s-1}L_{s'}},f),
}
By inserting \eqref{LIN_elec_z} %$\text{e}^{\tilde{\Gamma}(z,f)}$ %from \eqref{exp.gamma.tilde.expansion} 
into \eqref{F_kerr},
%we obtain 
%\eqlab{Lin.elec.z.expansion}{
%&
%E_{s,\text{x}}^{(0)}(z,f)=\nonumber\\&\text{e}^{-j2\pi^{2} f^{2}[\sum_{s'=1}^{s-1}(\beta_{2,s}L_{s'}+\frac{2}{3}\pi f \beta_{3,s'}L_{s'})+(\beta_{2,s'}z+\frac{2}{3}\pi f \beta_{3,s'}z)]}\nonumber\\&\prod_{s'=1}^{s-1}g_{s'}^{1/2}\text{e}^{\alpha_{s'}L_{s'}}\cdot\sqrt{\rho(z,f)}E_{\text{x}}(0,f).
%}
%We now substitute \eqref{Lin.elec.z.expansion} into the Kerr term \eqref{F_kerr}, and
we get
\eqlab{Kerr-term2}
{
&{\boldsymbol{Q}}_s(z,f)=j\gamma_s\frac{8}{9}\Big[E_{s,\text{x}}^{(0)}(z,f)*E_{s,\text{x}}^{(0)\scriptsize{*}}(z,-f)+\nonumber\\&E_{s,\text{y}}^{(0)}(z,f)*E_{s,\text{y}}^{(0)\scriptsize{*}}(z,-f)\Big]*{\boldsymbol{E}_s}^{(0)}(z,f).
}
Using \eqref{kappa'.l} the Kerr term in span $s$ \eqref{Kerr-term2} can be expressed like \eqref{qx_2}, with two minor differences. One is the the product term in \eqref{kerr.ter.span.s}, which is responsible for taking into account the amplifiers' gain and loss of previous spans. The second is the last exponential term in \eqref{kerr.ter.span.s} which is responsible for taking into account the second and third order dispersion of the previous spans.
\begin{figure*}[t]
\scriptsize
\eqlab{kerr.ter.span.s}{
&Q_{s,\text{x},\kappa}(z,f)=-j\gamma_{s}\frac{8}{9}f_0^{3/2}\prod_{s'=1}^{s-1}[g_{s'}\cdot\rho(L_{s'},f)]^{3/2} %\text{e}^{\Gamma(z,if_0+(\kappa-l))}
\sum_{\kappa_1=1}^{M}
\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}
\sum_{i=-\infty}^{\infty}\delta\big(f\!-\!if_0\!-(\kappa-l)\big)\sum_{m,n,k\in \mathcal{S}_i}\big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\nonumber\\&+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\big)\text{e}^{\tilde{\Gamma}_s(z,mf_0+\kappa_1 R)+\tilde{\Gamma}_s^*(z,nf_0+(\kappa_1+\kappa_2-\kappa+l) R)+\tilde{\Gamma}_s(z,kf_0+\kappa_2 R)} \nonumber\\&
\cdot\text{e}^{-j2\pi^{2}\big((mf_0+\kappa_1R)^2-(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{2}+(kf_0+\kappa_2R)^{2}\big)\sum_{s'=1}^{s-1}\beta_{2,s'}L_{s'}-j\frac{4}{3}\pi^{3}\big((mf_0+\kappa_1R)^3-(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{3}+(kf_0+\kappa_2R)^{3}\big)\sum_{s'=1}^{s-1}\beta_{3,s'}L_{s'}}
}.
\hrulefill
\end{figure*}
%=\nonumber\\&
%-j\gamma_s\frac{8}{9}f_0^{3/2}\prod_{s'=1}^{s-1}g_{s'}^{3/2}\text{e}^{-3\alpha_{s'}L_{s'}}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\\&\delta\big(f-if_0-(\kappa-l)R\big)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\nonumber\\&\cdot\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\nonumber\\&\cdot \sqrt{\rho(z,(mf_0+\kappa_1R))}\sqrt{\rho(z,(nf_0+(\kappa_1+\kappa_2-\kappa+l)R))}\nonumber\\&\cdot\sqrt{\rho(z,(mf_0+\kappa_2R))},
%}
%\begin{equation}\label{kerr.ter.span.s}
%\begin{split}
%&Q_{s,\text{x},\kappa}(z,f)=-j\gamma_s\frac{8}{9}f_0^{3/2}\prod_{s'=1}^{s-1}g_s^{3/2}\text{e}^{-3\alpha_sL_s}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\\&\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\\&\cdot\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\\&\cdot \text{e}^{\tilde{\Gamma}_s(z,mf_0+\kappa_1 R)+\tilde{\Gamma}_s^*(z,nf_0+(\kappa_1+\kappa_2-\kappa+l) R)+\tilde{\Gamma}_s(z,kf_0+\kappa_2 R)}.
%\end{split}
%\end{equation}
We now insert \eqref{kerr.ter.span.s} into (\ref{MAN_NLI_sol}) to find the nonlinear electrical field of channel $\kappa$ in span $s$, which is equal to
\eqref{NLI_elec_kappa_z}.
\begin{figure*}[t]
\scriptsize
\eqlab{NLI_elec_kappa_z}{
&E_{\text{NLI,\text{x}},\kappa}^{s}(z,f)=-j\gamma_{s}\frac{8}{9}f_0^{3/2}\prod_{s'=1}^{s-1}[g_{s'}\cdot\rho(L_{s'},f)]^{3/2}
\sum_{\kappa_1=1}^{M}
\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}
\sum_{i=-\infty}^{\infty}\delta\big(f\!-\!if_0\!-(\kappa-l)\big)\text{e}^{\Gamma(z,if_0+(\kappa-l))}\sum_{m,n,k\in \mathcal{S}_i}\big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\nonumber\\&+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\big)\zeta^s_{\kappa_1,\kappa_2,\kappa}(m,n,k)\nonumber\\&
\text{e}^{-j2\pi^{2}\big((mf_0+\kappa_1R)^2-(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{2}+(kf_0+\kappa_2R)^{2}\big)\sum_{s'=1}^{s-1}\beta_{2,s'}L_{s'}-j\frac{4}{3}\pi^{3}\big((mf_0+\kappa_1R)^3-(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{3}+(kf_0+\kappa_2R)^{3}\big)\sum_{s'=1}^{s-1}\beta_{3,s'}L_{s'}}
}
\hrulefill
\end{figure*}.
Considering the amplifier gain at the end of span $s$, we have 
\eqlab{NLI_elec_kappa_end_ns}{
&E_{s,\text{x},\kappa}^{(1)}({\scriptstyle\sum_{s'=1}^{s}L_{s'}},f)=g_{s}^{1/2}E_{s,\text{x},\kappa}^{(1)}(z,f)|_{z=L_{s}}.
}
%where $\zeta^{n_s}$ for $\gamma_{n_s}$, $L_{n_s}$, and $\beta_{n_s}$ is in analogy with (\ref{Zeta_ENL}) for $\gamma$, $L_s$, and $\beta$. 
To evaluate the nonlinear electrical filed of channel $\kappa$ at the end of link, we assume the nonlinear electrical field that generated in each span propagate linearly in the following spans until receive at the receiver, namely
\eqlab{}{
&E_{s,\text{x},\kappa}^{(1)}({\scriptstyle\sum_{s'=1}^{N}L_{s'}},f)=\prod_{s'=s+1}^{N}[{g_{s'}\cdot\rho(L_{s'},f)}]^{1/2}\nonumber\\& \text{e}^{-j2\beta_2\pi^{2}L_s\big(if_0+(\kappa-l)\big)^{2}\sum_{s'=s+1}^{N}(\beta_{2,s'}L_{s'}+\frac{2}{3}\pi(if_0+(\kappa-l)\beta_{2,s'}L_{s'})}\nonumber\\&E_{s,\text{x},\kappa}^{(1)}({\scriptstyle\sum_{s'=1}^{s}L_{s'}},f),
}
and, hence, this equation is equal to \eqref{NLI_elec_kappa_end_ns}.
\begin{figure*}[t]
\scriptsize
\eqlab{NLI_elec_kappa_end_ns}{
&-j\gamma_{s}\frac{8}{9}f_0^{3/2}\prod_{s'=1}^{s-1}[g_{s'}\cdot\rho(L_{s'},f)]^{3/2}g_{s}^{1/2}\!\!\! \prod_{s'=s+1}^{N}\!\!\! [g_{s'}\cdot\rho(L_{s'},f)]^{1/2} \sum_{\kappa_1=1}^{M}
\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}
\sum_{i=-\infty}^{\infty}\delta\big(f\!-\!if_0\!-(\kappa-1)\big)\nonumber\\&\text{e}^{-j2\pi^{2}(if_0+(\kappa-l)R)^{2}\sum_{s'=1}^{N_s}(\beta_2L_{s'}+\frac{2}{3}\pi(if_0+(\kappa-l)R)\beta_{3,s'}L_{s'})}\!\!\!\!\! \nonumber\\&\sum_{m,n,k\in s_i}\!\!\!\!\! \big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\big)\sqrt{\rho(L_{s},if_0+(\kappa-l))}\zeta^s_{\kappa_1,\kappa_2,\kappa}(m,n,k)\nonumber\\&
\text{e}^{-j2\pi^{2}\big((mf_0+\kappa_1R)^2-(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{2}+(kf_0+\kappa_2R)^{2}\big)\sum_{s'=1}^{s-1}\beta_{2,s'}L_{s'}-j\frac{4}{3}\pi^{3}\big((mf_0+\kappa_1R)^3-(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{3}+(kf_0+\kappa_2R)^{3}\big)\sum_{s'=1}^{s-1}\beta_{3,s'}L_{s'}
},
}
\hrulefill
\end{figure*}

 Based on (\ref{NLI_elec_tot}), the total nonlinear electrical field at the end of link can be written as \eqref{NLI_elec_tot_detail}. This completes the proof.
 \end{IEEEproof}
%As seen in this equation, the three spectral components $mf_0$, $kf_0$, and $mf_0+kf_0-if_0$ located in channels $\kappa_1$, $\kappa_2$, $\kappa_1+\kappa_2-\kappa+l$, respectively, interact with each other and produce the nonlinear interference at $if_0$. The efficiency of this non-degenerate four wave mixing (FWM), denoted by \eqref{Zeta_ENL}, is taking place among these spectral components.
%\section{Derivation of the NLI power}\label{AppendixB}
%This appendix addresses derivation of the the NLI power of a certain channel, starting from the NLI PSD on polarization x 
%\eqlab{G_x_Def}
%{
%G_{\text{\small{NLI}},\text{x},\kappa}(f)=\mathbb{E}\big\{E_{\text{NLI,x},\kappa}(f)\text{e}^{*}_{\text{NLI,x},\kappa}(f)\big\}.
%}

==> NumericalRsults.tex <==
\section{Numerical Results}\label{numerical results}

In this section, we validate our model with numerical simulations and compare the results with previously published models. For the validation, the models are compared with split-step Fourier method (SSFM) simulations, a reference assumed to accurately account for the fiber propagation effects. The simulations are conducted for a transmission in a single span in the C band with an artificially increased Raman coefficient. The span loss was fully compensated in the end of the link by a noiseless amplifier. We therefore consider {\it{Corollary}}~\ref{main.result.identical} instead of {\it{Theorem}}~\ref{main.result} to generate the results.

% \subsection{Numerical validation}\label{numerical_a}
The SSFM is used to solve the Manakov equation numerically, and presents high computational complexity for C+L transmissions. Due to this restriction, a C band transmission of $1.01$ THz WDM bandwidth is considered. The system parameters for the simulations are shown in Table~\ref{system_parameters_table}. We assumed $101$ WDM channels with symbol rate of $R=10$ GHz each, spaced by $10.001$ GHz. Each channel was shaped by an ideal root-raised-cosine with $0.01\%$ roll-off factor. The launch power was set to $-1$ dBm per channel, yielding a total launch power of $19$ dBm. To mimic the SRS effect of a C+L transmission of $10$ THz and have substantial power transfer between channels, the Raman gain slope $C_r$ was set to $1.12$ 1/W/km/THz, which is $40$ times a more conventional value of $0.028$ 1/W/km/THz. The 40 times higher $C_r$ allowed us to obtain a power profile gap of 8.2 dB between the outermost channels, in  consistence with the approach employed in \cite[Sec.~III]{semrau2018gaussian}. The SSFM simulations were performed using an adaptive step approach, where a maximum nonlinear phase rotation per step of 3 mmrad was used. This number proved to be enough to obtain accurate estimates of the NLI power. 

The transmitted symbols were randomly chosen from one of the following modulation formats: polarization multiplexed quadrature phase shift keying (PM-QPSK), polarization multiplexed 16 ary quadrature amplitude modulation (PM-16QAM), and Gaussian modulation. Their respective values of $\Phi_b$ and $\Psi_b$ can be found on Table~\ref{tab2}.  
 The received signal was ideally compensated for chromatic dispersion. After the dispersion compensation, the receiver applies matched filtering and sampling to the signal, resulting in the received symbols. With these symbols, the signal-to-noise ratio (SNR) is calculated. The SNR for a constellation with $M$ symbols is defined as
\begin{equation}
    \text{SNR} = \dfrac{\sum_{i=1}^{M}|\tau_i|^2}{\sum_{i=1}^{M}E[| Y_i - \tau_i|^2]},
\end{equation}
where $Y_i$ and $\tau_i$ are the random variable and the conditional mean related to the received symbols from the $i$-th constellation point, respectively. The SNR$_\kappa$ for the $\kappa$-th channel is used for the calculation of $\sigma_{\text{NLI},\kappa}^2$ in the SSFM simulations. The relation between these two variables when all channels have the same launch power $P$ is approximately given by
\begin{equation}\label{eq:snr}
\text{SNR}_\kappa \approx \dfrac{P}{P_{\text{ASE}}+\sigma_{\text{NLI},\kappa}^2} = \dfrac{P}{P_{\text{ASE}}+\eta_\kappa P^3},
\end{equation}
where $\eta_\kappa \triangleq \sigma_{\text{NLI},\kappa}^2/P^3$ is the nonlinear interference coefficient for the $\kappa$-th channel.  $\eta_\kappa$ is by definition the normalized NLI variance, and is the metric used to validate the results in this paper. Furthermore, \eqref{eq:snr} is simplified by assuming $P_{\text{ASE}}=0$ due to the noiseless amplifier consideration.






% Due to the high computational complexity of solving the Manakov equation using the split-step Fourier method for C+L band transmissions, a $1.01$ THz WDM bandwidth with an artificially increased Raman gain slope is considered.  We assume $101$ Nyquist rectangular spectral-shaped channels with symbol rate of $R=10$ GHz can be accommodated in the spectrum and therefore the numerical results were carried out with an artificially ten-fold increased Raman gain slope. The same assumption employed in \cite[Sec.~III]{semrau2018gaussian}. In other words, the Raman gain slope for C+L band (approximately 10 THz) applied in \cite{semrau2018gaussian} is 0.028 1/W/km/THz, so that we scale this by 10 for bandwidth $B_{\text{opt}}=101\times10$ GHz. This scaling would be necessary to have the substantial power transfer equivalent to the ultra-wideband systems power transfer.


%Eq.~(\ref{EGN_fixed}) can be written as
%\begin{equation}\label{eq33_alt}
%\begin{split}
%\sigma_{\tiny{\text{NLI}_{\kappa}}}^{2}=&\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}P_{\kappa_1}P_{\kappa_2}P_{\kappa_1+\kappa_2-\kappa+l}\hspace{1mm}\nonumber\\&\cdot\eta_\kappa(\kappa_1,\kappa_2,l),
%\end{split}
%\end{equation}
%where the NLC of channel $\kappa$ is
%\begin{equation}\label{eq33_NLC}
%\begin{split}
%&\text{NLC}_\kappa=\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\eta_\kappa(\kappa_1,\kappa_2,l).
%\end{split}
%\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%  As shown in this figure, the normalized NLI variance is computed in the absence of SRS and in the presence of SRS for 4 different modulation formats such as: polarization multiplexed quadrature phase shift keying (PM-QPSK), polarization multiplexed 16 ary quadrature amplitude modulation (PM-16QAM), polarization multiplexed 64 ary quadrature amplitude modulation (PM-64QAM), and Gaussian modulation. The results  show that the NLI spectrum in the absence of SRS (solid blue curve) is symmetric namely the normalized NLI variance for channels at the edge of spectrum is lower than the other part of spectrum, while the normalized NLI variance for channels in the middle of spectrum is higher than the other parts. On the other hand, the NLI spectrum in the presence of SRS is no longer symmetric such that channels that undergo SRS gain experience higher NLI, and channels that undergo SRS loss experience lower NLI. When the total input launch power is increased, the discrepancy between the nonlinear interference with and without SRS becomes greater, i.e., for increasing input launch power, the normalized NLI variance beings to tilt.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%\begin{table}[!t]
%\begin{center}
%\caption{System parameters}
%\label{tab:System_parameter}
%\begin{tabular}{ll}
%\noalign{\hrule height 2pt}
%\small {Symbol rate $R$} &\small {50 Gbaud} \\
%\small {Nonlinear coefficient $\gamma$}&\small {$1.3~\text{W}^{-1}\text{km}^{-1}$}\\
%\small {Loss $\alpha$} &\small {$0.2$ dB/km}\\
%\small {Dispersion coefficient $D$} &\small {16.7 ps/nm/km}\\
%\small {Dispersion slope $S$} &\small {0 ps/$\text{nm}^{2}$/km}\\
%\small {Raman gain slope $C_r$} &\small {0.28 1/W/km/THz}\\
%\small {Optical center wavelength $\lambda$} &\small {$1550$ nm} \\
%\small {EDFA noise figure $F_n$} &\small {5 dB} \\
%\small {Span length $L_s$} &\small {100 km} \\
%%\small {Effective span length $L_{\text{eff}}$} & ${(1-e^{\alpha L_s})}/{(2\alpha)}$ \\
%\small {WDM channel spacing $\Delta f$} &\small {50 GHz} \\
%\small {Number of channels} &\small {20} \\
%\small {Optical Bandwidth (GHz)} &\small {200} \\
%\hline
%\end{tabular}
%\end{center}
%\end{table}


%\begin{figure*}[!t]
%\pgfplotsset{compat=1.3}
%\begin{center}
%\begin{tikzpicture}[scale=1]
%\begin{axis}[grid=major,
%width=9.5cm,height=7.5cm,ymin=29,ymax=37,ylabel=Normalized NLI variance (dB), xmin=1,xmax=20, xlabel=Channel Number, title=PM-QPSK,legend style={at={(0.05,0.25)},anchor=west},
%%ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
%%$16$,
%%$18$,
%%$20$, 
%%$22$, 
%%$24$, 
%%$26$,
%%$28$,  
%%}, 
%]
%%ymin=1,ymax=1.07, 
%%%%%ytick={16,18,20,22,24,26,28},
%%yticklabels={
%%$16$,
%%$18$,
%%$20$, 
%%$22$, 
%%$24$, 
%%$26$,
%%$28$,  
%%},
%\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_QPSK_noSRS.dat};
%%\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_QPSK_15.dat};
%%\addplot [red, line width=0.4mm,dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_175.dat};
%\addplot [red, line width=0.4mm, mark=*] table[x index=0,y index=1] {Dat/NLIN_QPSK_2.dat};
%\addplot [black, line width=0.3mm,mark=asterisk]table[x index=0,y index=1] {Dat/NLIN_QPSK_225.dat};
%\addplot [green!60!green, line width=0.6mm, mark=halfdiamond*]table[x index=0,y index=1] {Dat/NLIN_QPSK_25.dat};
%\addplot [magenta, line width=0.4mm, mark=halfcircle*]table[x index=0,y index=1] {Dat/NLIN_QPSK_275.dat};
%\legend{no SRS, $20$ dBm, $22.5$ dBm, $25$ dBm,$27.5$ dBm}
%\end{axis}
%\end{tikzpicture}
%\hspace{-3mm}
%\begin{tikzpicture}[scale=1]
%\begin{axis}[grid=major,
%width=9.5cm,height=7.5cm,ymin=31,ymax=39, xmin=1,xmax=20, xlabel=Channel Number,title=PM-16QAM,legend style={at={(0.05,0.25)},anchor=west},
%%ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
%%$16$,
%%$18$,
%%$20$, 
%%$22$, 
%%$24$, 
%%$26$,
%%$28$,  
%%}, 
%]
%%ymin=1,ymax=1.07, 
%%%%%ytick={16,18,20,22,24,26,28},
%%yticklabels={
%%$16$,
%%$18$,
%%$20$, 
%%$22$, 
%%$24$, 
%%$26$,
%%$28$,  
%%},
%\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_16QAM_noSRS.dat};
%%\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_QPSK_15.dat};
%%\addplot [red, line width=0.4mm,dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_175.dat};
%\addplot [red, line width=0.4mm, mark=*] table[x index=0,y index=1] {Dat/NLIN_16QAM_2.dat};
%\addplot [black, line width=0.3mm,mark=asterisk]table[x index=0,y index=1] {Dat/NLIN_16QAM_225.dat};
%\addplot [green!60!green, line width=0.6mm, mark=halfdiamond*]table[x index=0,y index=1] {Dat/NLIN_16QAM_25.dat};
%\addplot [magenta, line width=0.4mm, mark=halfcircle*]table[x index=0,y index=1] {Dat/NLIN_16QAM_275.dat};
%\legend{no SRS, $20$ dBm, $22.5$ dBm, $25$ dBm,$27.5$ dBm}
%\end{axis}
%\end{tikzpicture}
%\hspace{-3mm}
%\begin{tikzpicture}[scale=1]
%\begin{axis}[grid=major,
%width=9.5cm,height=7.5cm, ymin=31,ymax=39, ylabel=Normalized NLI variance (dB),xmin=1,xmax=20, xlabel=Channel Number, title=PM-64QAM,legend style={at={(0.05,0.25)},anchor=west},
%%ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
%%$16$,
%%$18$,
%%$20$, 
%%$22$, 
%%$24$, 
%%$26$,
%%$28$,  
%%}, 
%]
%%ymin=1,ymax=1.07, 
%%%%%ytick={16,18,20,22,24,26,28},
%%yticklabels={
%%$16$,
%%$18$,
%%$20$, 
%%$22$, 
%%$24$, 
%%$26$,
%%$28$,  
%%},
%\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_64QAM_noSRS.dat};
%%\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_QPSK_15.dat};
%%\addplot [red, line width=0.4mm,dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_175.dat};
%\addplot [red, line width=0.4mm, mark=*] table[x index=0,y index=1] {Dat/NLIN_64QAM_2.dat};
%\addplot [black, line width=0.3mm,mark=asterisk]table[x index=0,y index=1] {Dat/NLIN_64QAM_225.dat};
%\addplot [green!60!green, line width=0.6mm, mark=halfdiamond*]table[x index=0,y index=1] {Dat/NLIN_64QAM_25.dat};
%\addplot [magenta, line width=0.4mm, mark=halfcircle*]table[x index=0,y index=1] {Dat/NLIN_64QAM_275.dat};
%\legend{no SRS, $20$ dBm, $22.5$ dBm, $25$ dBm,$27.5$ dBm}
%\end{axis}
%\end{tikzpicture}
%\hspace{-3mm}
%\begin{tikzpicture}[scale=1]
%\begin{axis}[grid=major,
%width=9.5cm,height=7.5cm,ymin=34,ymax=41, xmin=1,xmax=20, xlabel=Channel Number, title=Gaussian,legend style={at={(0.075,0.25)},anchor=west},
%%ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
%%$16$,
%%$18$,
%%$20$, 
%%$22$, 
%%$24$, 
%%$26$,
%%$28$,  
%%}, 
%]
%%ymin=1,ymax=1.07, 
%%%%%ytick={16,18,20,22,24,26,28},
%%yticklabels={
%%$16$,
%%$18$,
%%$20$, 
%%$22$, 
%%$24$, 
%%$26$,
%%$28$,  
%%},
%\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_Gaussian_noSRS.dat};
%%\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_QPSK_15.dat};
%%\addplot [red, line width=0.4mm,dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_175.dat};
%\addplot [red, line width=0.4mm, mark=*] table[x index=0,y index=1] {Dat/NLIN_Gaussian_2.dat};
%\addplot [black, line width=0.3mm,mark=asterisk]table[x index=0,y index=1] {Dat/NLIN_Gaussian_225.dat};
%\addplot [green!60!green, line width=0.6mm, mark=halfdiamond*]table[x index=0,y index=1] {Dat/NLIN_Gaussian_25.dat};
%\addplot [magenta, line width=0.4mm, mark=halfcircle*]table[x index=0,y index=1] {Dat/NLIN_Gaussian_275.dat};
%\legend{no SRS, $20$ dBm, $22.5$ dBm, $25$ dBm,$27.5$ dBm}
%\end{axis}
%\end{tikzpicture}
%%\\
%%\vspace*{2pt}
%%\ref{named}
%\end{center}
%\setlength{\belowcaptionskip}{-12pt}
%\caption{The nonlinear coefficient as a function of channel number after three spans for various spectrally flat input power profile with PM-QPSK, PM-16QAM, PM-64QAM, and Gaussian modulations. In fact, we assume the fiber-optic link is composed of three different spans such that the fiber types and lengths of these spans are as follows. Span 1: fiber type=SMF, length=120km; Span 2: fiber type=NZDSF, length=80km; Span 3: fiber type=SMF, length=100km.} 
%\label{fig_MDS}
%\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  As seen in these figures, the NLI that PM-QPSK experiences is lower than the other modulation formats. By contrast, the experienced nonlinear interference of Gaussian modulation is higher than the others. Intuitively, this is due to the fact that, PM-QPSK is composed of four symbols, while Gaussian modulation has an infinitive number of symbols and, hence, Gaussian modulation receives higher NLI than PM-QPSK. Theoretically, the fourth order modulation format $\Phi_b$ appears as a coefficient of non-Gaussianity correction term when more than two interfering frequency components located in a single channel. On the other hand, $\Psi_b$ appears when all interfering frequency components located in a single channel. The FWM efficiency of the no-Gaussianity correction terms whose coefficient is $\Phi_b$ is also higher than the a non-Gaussianity correction term whose coefficient is $\Psi_b$.  As summarized in Table.~\ref{tab2}, the absolute value of $\Phi_b$ for PM-QPSK is larger than the other modulation formats, whereas for Gaussian modulation is equal to zero.  It is also found that the NLI that omitted from Gaussian modulation in order to yield the modulation format dependent EGN model for PM-QPSK is higher than PM-16QAM and PM-64QAM.

%  In Fig.~\ref{nlc_deviation_fig_hetroMod}, we are considering heterogeneous modulation formats across the WDM spectrum such as PM-QPSK, PM-16QAM, nad PM-64QAM. As mentioned earlier the impact of SRS on Kerr nonlinearity causes the NLI spectrum tilt. To reduce the NLI tilt, it is assumed that a various modulation formats were transmitted in different parts of spectrum. As seen in Fig.~\ref{nlc_fig}, the lower and higher frequency channels experience the lower and higher NLI, respectively. We therefore assume that the lower and higher frequency channels transmitted using PM-QPSK and PM-64QAM, respectively, and the channels located in the middle of spectrum transmitted using PM-16QAM. This is because the frequency channels that experience higher NLI transmitted using the modulation format which undergoes the lowest NLI, i.e., PM-QPSK, and frequency channels with lower NLI transmitted using the modulation format which undergoes the highest NLI, i.e., PM-64QAM. And the frequency channels in the middle of spectrum experience the average NLI and therefore transmitted using PM-16QAM.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





\begin{table}[t]
\begin{center}
\caption{Values of $\Phi_b$ and $\Psi_b$}
\label{tab2}
\begin{tabular}{lll}
\noalign{\hrule height 2pt}
\small {Format} &\small {$\Phi_b$} & \small{$\Psi_b$}\\
\hline
\small {PM-QPSK} &\small {-1} & \small{4}\\
\small {PM-16QAM} &\small {-0.68} & \small{2.08}\\
% \small {PM-64QAM} &\small {-0.619} & \small{1.7972}\\
\small {Gaussian} &\small {0} & \small{0}\\
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\begin{center}
    \caption{System Parameters}
    \label{system_parameters_table}
    \begin{tabular}{l|c}
\noalign{\hrule height 2pt}
    \bf{Parameters} & \textbf{Values}\\ 
\noalign{\hrule height 1.5pt}
    \multicolumn{1}{l|}{Loss ($\alpha$) [dB/km]}& 0.2 \\ \hline
    
     \multicolumn{1}{l|}{Dispersion ($D$) [ps/nm/km]}&  17\\ \hline
     
      \multicolumn{1}{l|}{Dispersion slope ($S$) [ps/nm\textsuperscript{2}/km]}&  0\\ \hline
       
         \multicolumn{1}{l|}{NL coefficient ($\gamma$) [1/W/km]}&  1.2\\ \hline
         
          \multicolumn{1}{l|}{Raman gain slope ($C_r$) [1/W/km/THz]}&  1.12\\ \hline
           
          \multicolumn{1}{l|}{Fiber length ($L$) [km]}& 100 \\ \hline  
           
          \multicolumn{1}{l|}{Symbol rate ($R$) [GBd]}&  10 \\ \hline  
    \multicolumn{1}{l|}{Channel spacing ($R$) [GHz]}&  10.001 \\ \hline
    
    \multicolumn{1}{l|}{Number of channels}&  101 \\ \hline

   \multicolumn{1}{l|}{Roll-off factor ($\%$)}&  0.01 \\ \hline

  \multicolumn{1}{l|}{Optical bandwidth ($B$) [THz]} & 1.01 \\ \hline

    \end{tabular}
    \center
    \end{center}
 \end{table}




% \begin{table}
%     \caption{System Parameters}
%     \label{system_parameters_table}
%     \begin{tabular}{l|c|c}
% \noalign{\hrule height 2pt}
%     \bf{Parameters}&{(a)}&(b)\\ 
%     \hline
%         \bf{For section}&{\ref{numerical_a}}&{\ref{numerical_b}}\\
% \noalign{\hrule height 1.5pt}
%     \multicolumn{1}{l|}{Loss ($\alpha$) [dB/km]}&  \multicolumn{2}{c}{0.2}\\ \cline{1-3}
    
%      \multicolumn{1}{l|}{Dispersion ($D$) [ps/nm/km]}&  \multicolumn{2}{c}{17}\\ \cline{1-3}
     
%       \multicolumn{1}{l|}{Dispersion slope (S) [ps/nm\textsuperscript{2}/km]}&  \multicolumn{2}{c}{17}\\ \cline{1-3}
       
%          \multicolumn{1}{l|}{NL coefficient ($\gamma$) [1/W/km]}&  \multicolumn{2}{c}{1.2}\\ \cline{1-3}
         
%           \multicolumn{1}{l|}{Raman gain slope ($C_r$) [1/W/km/THz]}&  \multicolumn{1}{c|}{0.28}&  \multicolumn{1}{c}{0.028}\\ \cline{1-3}
           
%           \multicolumn{1}{l|}{Fiber length ($L$) [km]}&  \multicolumn{2}{c}{100}\\ \cline{1-3}  
           
%           \multicolumn{1}{l|}{Symbol rate ($R$) [GBd]}&  \multicolumn{1}{c|}{10}&  \multicolumn{1}{c}{50}\\ \cline{1-3}  
%     \multicolumn{1}{l|}{Channel spacing ($R$) [GHz]}&  \multicolumn{1}{c|}{10}&  \multicolumn{1}{c}{50}\\ \cline{1-3}
    
%     \multicolumn{1}{l|}{Number of channels}&  \multicolumn{1}{c|}{101}&  \multicolumn{1}{c}{201}\\ \cline{1-3}

%   \multicolumn{1}{l|}{Optical bandwidth (B) [THz]}&  \multicolumn{1}{c|}{1.01}&  \multicolumn{1}{c}{10.05}\\ \cline{1-3}

%     \end{tabular}
%     \center
%  \end{table}

%%%% sigma^2_{NLI} vs channel idx SRS/no SRS
\begin{figure*}[!t]
\pgfplotsset{compat=1.3}
\begin{center}
\begin{tikzpicture}[scale=1]
\begin{groupplot}[group style={
group name=my plots, group size=2 by 2,horizontal sep=6pt,vertical sep=8.5pt},
width=10cm,height=8.5cm]


\nextgroupplot%%%%%PQ-16QAM
[
%xticklabels={},
legend columns=1,
legend entries={PM-QPSK (\textit{Corollary }\ref{main.result.identical}), PM-16QAM (\textit{Corollary }\ref{main.result.identical}), ISRS GN Model \cite{semrau2018gaussian}, SSFM Simulations},
ylabel={$\eta_\kappa \ [\text{dB} \ W^{-2}]$},
grid=major,
ymin=22,ymax=43, 
xmin=1,xmax=101,
%title=With SRS ($P_{\text{tot}}=25$ dBm),
xlabel=Channel Number $\kappa$, 
legend style={at={(0.0,0.125)},anchor=west,font=\footnotesize},
title=Without SRS,
%ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
%$16$,
%$18$,
%$20$, 
%$22$, 
%$24$, 
%$26$,
%$28$,  
%}, 
]

\draw[->,>=stealth,thick] (51,98) -- (51,136);
\node at (58,123) {\footnotesize{$4.1$ dB}};


\draw[->,>=stealth,thick] (18,94) -- (18,109);
\node at (25,104) {\footnotesize{$1.6$ dB}};


\addplot [red, line width=0.4mm, solid] table[x index=0,y index=1]
{Dat/NLIN_QPSK_noSRS_101ch_6mil.dat};
\addplot [blue, line width=0.5mm, solid] table[x index=0,y index=1]
{Dat/NLIN_16QAM_noSRS_101ch_6mil.dat};
\addplot [black, line width=0.9mm, dotted] table[x index=0,y index=1]
{Dat/NLIN_16QAM_25dBm_100ch_2mil.dat};
\addplot [black, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_Gaussain_noSRS_101ch_6mil.dat};
% \addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_Gaussain_noSRS_101ch_6mil.dat};

\addlegendimage{black,only marks,solid, mark=*,mark size = 1pt, line width = 0.8, mark options={fill=white,solid,scale=1.5}}
\addlegendentry{PM-QPSK (\textit{Corollary }\ref{main.result.identical})}
\addlegendentry{ PM-16QAM (\textit{Corollary }\ref{main.result.identical})}

\addlegendentry{ISRS GN Model \cite{semrau2018gaussian}}
\addlegendentry{SSFM Simulations}



\addplot [red,only marks,solid, mark=*,each nth point={3}, mark size = 1pt, line width = 0.8, mark options={fill=white,solid,scale=1.5}]table[x index=0,y index=1] {Dat/ssfm_qpsk_no_srs.dat};


\addplot [blue,only marks,solid, mark=*,each nth point={3},  mark size = 1pt, line width = 0.8, mark options={fill=white,solid,scale=1.5}]table[x index=0,y index=1] {Dat/ssfm_16qam_no_srs.dat};


\nextgroupplot
[
legend columns=1,
legend entries={PM-QPSK (\textit{Corollary }\ref{main.result.identical}), PM-16QAM (\textit{Corollary }\ref{main.result.identical}), ISRS GN Model \cite{semrau2018gaussian}, PM-QPSK (SCI+XPM Model \cite{semrau2019modulation}), PM-16QAM \cite{semrau2019modulation}},
%legend to name=benchmarkfigc1,
%xticklabels={},
% ylabel={$\eta_\kappa \ [\text{dB} \ W^{-2}]$},
grid=major,
ymin=22,ymax=43, 
xmin=1,xmax=101,
%title=With SRS ($P_{\text{tot}}=25$ dBm),
xlabel=Channel Number $\kappa$, 
legend style={at={(0.002,0.215)},anchor=west,font=\footnotesize},
title=With SRS,
yticklabels={,,}
%($P_{\text{tot}}=25$ dBm),
%legend enteries={no SRS, $19$ dBm, $23$ dBm, $25$ dBm, $27.5$ dBm, $27.5$ dBm \cite{semrau2019modulation}},
%legend to name=benchmarkfigc,
%xticklabels={},
%ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
%$16$,
%$18$,
%$20$, 
%$22$, 
%$24$, 
%$26$,
%$28$,  
%}, 
]

\draw[->,>=stealth,thick] (51,98) -- (51,135.5);
\node at (58,122.5) {\footnotesize{$3.9$ dB}};


\draw[->,>=stealth,thick] (39-19.5,63+8) -- (39-19.5,101+10);
\node at (45-20,78+4+1) {\footnotesize{$4$ dB}};

\draw[->,>=stealth,thick] (20-9,100+8) -- (20-9,127+2);
\node at (26-9,112.25+5+2) {\footnotesize{$2.1$ dB}};


\addplot [red, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLI_101CH_10GHZ_25DBM.dat};
\addplot [green, line width=0.5mm, blue]table[x index=0,y index=1] {Dat/NLI_16QAM_101CH_10GHZ_25DBM.dat};
%\addplot [purple, line width=0.4mm, dotted]table[x index=0,y index=1] {Dat/NLI_64QAM_101CH_10GHZ_25DBM.dat};
\addplot [line width=0.5mm, black]table[x index=0,y index=1] {Dat/NLI_GN_101CH_10GHZ_25DBM.dat};
%\addplot [red, line width=0.5mm, dotted]table[x index=0,y index=1] {Dat/NLI_QPSK_101CH_10GHZ_25DBM_DAN.dat};
%\addplot [blue, line width=0.5mm, dotted]table[x index=0,y index=1] {Dat/NLI_16QAM_101CH_10GHZ_25DBM_DAN.dat};
\addplot [blue, line width=0.5mm, dotted]table[x index=0,y index=1] {Dat/NLIN_Dan_16qam_closedform.dat};
\addplot [red, line width=0.5mm, dotted]table[x index=0,y index=1] {Dat/NLIN_DAN_QPSK_CLOSEDFORM.dat};
%\addplot [pink,line width=0.5mm]table[x index=0,y index=1] {Dat/NL_test_qpsk.dat};
%\addplot [green, line width=0.5mm]table[x index=0,y index=1] {Dat/nlinSure.dat};


\addlegendimage{black,only marks,solid, mark=*,mark size = 1pt, line width = 0.8, mark options={fill=white,solid,scale=1.5}}
\addlegendentry{\scriptsize PM-QPSK (\textit{Corollary }\ref{main.result.identical})}
\addlegendentry{\scriptsize PM-16QAM (\textit{Corollary }\ref{main.result.identical})}

\addlegendentry{\scriptsize ISRS GN Model \cite{semrau2018gaussian}}

%\addlegendentry{PM-QPSK (SCI+XPM Model \cite{semrau2019modulation})}

\addlegendentry{\scriptsize PM-16QAM (with factor 2 \cite{semrau2019modulation})}

%\addlegendentry{PM-16QAM (analytical \cite{semrau2019modulation})}

\addlegendentry{\scriptsize PM-QPSK (with factor 2 \cite{semrau2019modulation})}


\addlegendentry{\scriptsize SSFM Simulations}

\addplot [red,only marks,solid, mark=*,each nth point={3}, mark size = 1pt, line width = 0.8, mark options={fill=white,solid,scale=1.5}]table[x index=0,y index=1] {Dat/ssfm_qpsk_srs.dat};


\addplot [blue,only marks,solid, mark=*,each nth point={3},  mark size = 1pt, line width = 0.8, mark options={fill=white,solid,scale=1.5}]table[x index=0,y index=1] {Dat/ssfm_16qam_srs.dat};







\end{groupplot}
\end{tikzpicture}
\\
\vspace*{7pt}
%\ref{benchmarkfigc1}
\end{center}
\setlength{\belowcaptionskip}{-12pt}
\caption{$\eta_\kappa$  as a function of channel number $\kappa$ after one span in the absence of SRS and in the presence of SRS with a spectrally flat input power profile for PM-QPSK, PM-16QAM, PM-64QAM, and Gaussian modulations. SSFM simulations are represented by circle markers and numerical results using \textit{Corollary }\ref{main.result.identical} are represented by solid lines.} 
\label{nlc_fig}
\end{figure*}




% \begin{figure}
% \pgfplotsset{compat=1.3}
% \begin{center}
% \begin{tikzpicture}[scale=1]
% \begin{axis}[grid=major,
% width=9cm,height=7.5cm,ymin=33,ymax=40,ylabel={$\eta_\kappa \ [\text{dB} \ W^{-2}]$}, xmin=1,xmax=101, xlabel=Channel Number $\kappa$, legend style={at={(0.01,0.12)},anchor=west},
% ytick={27,29,31,33,35,37,39,41},yticklabels={
% $27$,
% $29$,
% $31$, 
% $33$, 
% $35$, 
% $37$,
% $39$,  
% $41$,  
% }, 
% ]
% %ymin=1,ymax=1.07, 
% %%%%ytick={16,18,20,22,24,26,28},
% %yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %},
% %\addplot [blue, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_VariableModulation_25dBm_101.dat};

% \addplot [green, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLI_HET_25DBM_1THZ_wSRS.dat};
% \addplot [pink, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLI_HETRO_NOSRS_101CH_10GHZ_25DBM.dat};

% \addplot [red,only marks,solid, mark=*,each nth point={3}, mark size = 1pt, line width = 0.8, mark options={fill=white,solid,scale=1.5}]table[x index=0,y index=1] {Dat/ssfm_diff_mod_no_srs.dat};


% \addplot [blue,only marks,solid, mark=*,each nth point={3}, mark size = 1pt, line width = 0.8, mark options={fill=white,solid,scale=1.5}]table[x index=0,y index=1] {Dat/ssfm_diff_mod_srs.dat};


% %\addplot [blue, line width=0.4mm, dotted]table[x index=0,y index=1] {Dat/NLIN_Gaussian_275.dat};
% \legend{w/o SRS, $P_{\text{tot}}=25$ dBm};
% \end{axis}
% \draw [latex-latex, black] (0,5) -- (2.5,5) node [sloped,midway,above] {\footnotesize{PM-QPSK}} ;
% \draw [latex-latex, black] (0+2.55,5) -- (2.5+2.6,5) node [sloped,midway,above] {\footnotesize{PM-16QAM}} ;
% \draw [latex-latex, black] (0+2.55+2.6,5) -- (2.5+2.6+2.3,5) node [sloped,midway,above] {\footnotesize{PM-64QAM}} ;
% %\draw [latex-latex, black, thick] (3.5,3.4) -- (3.5,4.8) node [sloped,midway,below] {\small{$\approx 4$ dB}} ;




% \end{tikzpicture}
% \end{center}
% \setlength{\belowcaptionskip}{-12pt}
% \caption{$\eta_\kappa$ as a function of channel number after one span. The first 34 WDM channels use PM-QPSK, the second 34 WDM channels use PM-16QAM, and the last 33 WDM channels use PM-64QAM.}
% \label{nlc_deviation_fig_hetroMod}
% \end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%  \subsection{C+L band Transmission}\label{numerical_b}

%  Using the proposed general analytical model \eqref{EGN_fixed} and parameters listed in Tabel~\ref{system_parameters_table}(b), the effects of SRS and Kerr nonlinearity is investigated in C+L band transmission systems covering almost 10 THz WDM bandwidth. The normalized NLI as a function of channel number is shown in Fig.~\ref{nlc_fig_c+l}. We assume 200 WDM channels with bandwidth of 50 GHz co-propagated in a fiber link and the NLC is computed at the end of a span with length of 100 km. Here, the third order dispersion ($\beta_3$) is considered. In the following subsection we show that for 50 GHz WDM channels the dominant NLI terms are SCI and XPM terms, and hence, in this section we only consider these dominant NLI terms. Similar to what mentioned earlier, in Fig.~\ref{nlc_fig_c+l}, Gaussian modulation and PM-QPSK are faced with the highest and lowest NLI, respectively.
% As can be seen in this figure the NLI tilt is modulation format independent because the effect of SRS depends on the frequency components and total launch power.

%  Two heterogeneous modulation format scenarios were considered in Fig.~\ref{nlc__fig_c+l_heterogeneous} to balance the NLI tilt resulted from the effect of SRS. In the first scenario it is assumed that the channels located in the first, second and last one-third of WDM spectrum transmitted through PM-QPSK, PM-16QAM, and PM-64QAM, respectively. The second scenario assumes that the channels located in the first, second, third, and last quarter of WDM spectrum transmitted through PM-QPSK, PM-16QAM, PM-64QAM, and Gaussian modulation formats, respectively. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{figure}
% \pgfplotsset{compat=1.3}
% \begin{center}
% \begin{tikzpicture}[scale=1]
% \begin{axis}[grid=major,
% width=9cm,height=7.5cm,ymin=15,ymax=32,ylabel=Normalized NLI variance (dB), xmin=1,xmax=201, xlabel=Channel Number, legend style={at={(0.01,0.17)},anchor=west},
% %ytick={27,29,31,33,35,37,39,41},yticklabels={
% %$27$,
% %$29$,
% %$31$, 
% %$33$, 
% %$35$, 
% %$37$,
% %$39$,  
% %$41$,  
% %}, 
% ]
% %ymin=1,ymax=1.07, 
% %%%%ytick={16,18,20,22,24,26,28},
% %yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %},
% \addplot [red, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_CL_QPSK.dat};
% \addplot [green, line width=0.4mm, solid, mark repeat=10, mark=*]table[x index=0,y index=1] {Dat/NLIN_CL_16QAM.dat};
% \addplot [purple, line width=0.4mm, dotted]table[x index=0,y index=1] {Dat/NLIN_CL_64QAM.dat};
% \addplot [blue, line width=0.4mm, solid]table[x index=0,y index=1] {Dat/NLIN_CL_Gaussian.dat};
% %\addplot [blue, line width=0.4mm, dotted]table[x index=0,y index=1] {Dat/NLIN_CL_HyberidModulation_T.dat};
% %\addplot [blue, line width=0.4mm, dotted]table[x index=0,y index=1] {Dat/NLIN_Gaussian_275.dat};
% \legend{\small{PM-QPSK}, \small{PM-16QAM}, \small{PM-64QAM}, \small{Gaussian Modulation}};
% \end{axis}
% %\draw [latex-latex, black, thick] (3.5,3.4) -- (3.5,4.8) node [sloped,midway,below] {\small{$\approx 4$ dB}} ;
% \end{tikzpicture}
% \end{center}
% \setlength{\belowcaptionskip}{-12pt}
% \caption{The normalized NLI variance as a function of channel number after one span for a flat launch power of 25 dBm.}
% \label{nlc_fig_c+l}
% \end{figure}


% \begin{figure}
% \pgfplotsset{compat=1.3}
% \begin{center}
% \begin{tikzpicture}[scale=1]
% \begin{axis}[grid=major,
% width=9cm,height=7.5cm,ymin=19,ymax=26,ylabel=Normalized NLI variance (dB), xmin=1,xmax=201, xlabel=Channel Number, legend style={at={(0.01,0.17)},anchor=west},
% %ytick={27,29,31,33,35,37,39,41},yticklabels={
% %$27$,
% %$29$,
% %$31$, 
% %$33$, 
% %$35$, 
% %$37$,
% %$39$,  
% %$41$,  
% %}, 
% ]
% %ymin=1,ymax=1.07, 
% %%%%ytick={16,18,20,22,24,26,28},
% %yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %},
% \addplot [blue,line width=0.4mm, solid]table[x index=0,y index=1] {Dat/NLIN_CL_AllHyberidModulation_T.dat};
% \addplot [red, line width=0.4mm, dotted]table[x index=0,y index=1] {Dat/NLIN_CL_HyberidModulation_T.dat};
% %\addplot [blue, line width=0.4mm, dotted]table[x index=0,y index=1] {Dat/NLIN_Gaussian_275.dat};
% %\legend{\small{PM-QPSK}, \small{PM-16QAM}, \small{PM-64QAM}, \small{Gaussian Modulation}};
% \end{axis}
% \draw [latex-latex, red] (0,5-2) -- (2.5,5-2) node [sloped,midway,below] {\scriptsize{PM-QPSK}} ;
% \draw [latex-latex, red] (0+2.55,5-2) -- (2.5+2.4,5-2) node [sloped,midway,below] {\scriptsize{PM-16QAM}} ;
% \draw [latex-latex, red] (2.5+2.41,5-2) -- (2.5+2.6+2.3,5-2) node [sloped,midway,below] {\scriptsize{PM-64QAM}};

% \draw [latex-latex, blue] (0,5+0.35) -- (1.8,5+0.35) node [sloped,midway,above] {\scriptsize{PM-QPSK}} ;
% \draw [latex-latex, blue] (0+1.81,5+0.35) -- (3.7,5+0.35) node [sloped,midway,above] {\scriptsize{PM-16QAM}} ;
% \draw [latex-latex, blue] (0+3.71,5+0.35) -- (3.71+1.8,5+0.35) node [sloped,midway,above] {\scriptsize{PM-64QAM}};
% \draw [latex-latex, blue] (3.71+1.81,5+0.35) -- (3.71+1.81+1.9,5+0.35) node [sloped,midway,above] {\scriptsize{Gaussian}};
% %\draw [latex-latex, black, thick] (3.5,3.4) -- (3.5,4.8) node [sloped,midway,below] {\small{$\approx 4$ dB}} ;
% \end{tikzpicture}
% \end{center}
% \setlength{\belowcaptionskip}{-12pt}
% \caption{The normalized NLI variance as a function of channel number after one span for 2 different scenarios. The solid blue curve indicates the scenario in which the first, second, and third 50 WDM channels use PM-QPSK, PM-16QAM, PM-64QAM, resp., and the last 51 WDM channels use Gaussian modulation. The red dotted curve indicates the scenario where the first and second 34 WDM channels use PM-QPSK and PM-16QAM, resp., and the last 33 WDM channels use PM-64QAM.}
% \label{nlc__fig_c+l_heterogeneous}
% \end{figure}

% \subsection{Benchmarking against previously published models}


% \begin{figure*}[!t]
% \pgfplotsset{compat=1.3}
% \begin{center}
% \begin{tikzpicture}[scale=1]
% \begin{groupplot}[group style={
% group name=my plots, group size=3 by 2,horizontal sep=6pt,vertical sep=6pt},
% width=6.75cm,height=6.5cm]
% \nextgroupplot
% [
% legend columns=-1,
% legend entries={Our Model, SRS GN model \cite{semrau2018gaussian}, SCI+XPM model \cite{semrau2019modulation}},
% legend to name=benchmarkfigc,
% xticklabels={},
% grid=major,
% ymin=30,ymax=42,ylabel=Normalized NLI variance (dB), xmin=1,xmax=101,
% %xlabel=Channel Number, 
% title=PM-QPSK,legend style={at={(0.05,0.25)},anchor=west},
% %legend enteries={no SRS, $19$ dBm, $23$ dBm, $25$ dBm, $27.5$ dBm, $27.5$ dBm \cite{semrau2019modulation}},
% %legend to name=benchmarkfigc,
% %xticklabels={},
% %ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %}, 
% ]
% %ymin=1,ymax=1.07, 
% %%%%ytick={16,18,20,22,24,26,28},
% %yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %},
% %\addplot [green, line width=0.4mm, solid, mark repeat=10, mark=*] table[x index=0,y index=1] {Dat/NLIN_QPSK_noSRS_101ch_6mil.dat};
% \addplot [green, line width=0.4mm, solid, mark repeat=10, mark=*]table[x index=0,y index=1] {Dat/NLIN_QPSK_25dBm_101ch_5mil.dat};
% %\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_QPSK_15.dat};
% %\addplot [red, line width=0.4mm,dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_175.dat};
% %\addplot [red, line width=0.4mm, mark=*] table[x index=0,y index=1] {Dat/NLIN_QPSK_2.dat};
% %\addplot [green!60!black, line width=0.3mm]table[x index=0,y index=1] {Dat/NLIN_Gaussain_noSRS_101ch_6mil.dat};
% \addplot [blue, line width=0.4mm]table[x index=0,y index=1] {Dat/NLIN_Gaussian_25dBm_101ch_5mil.dat};
% \addplot [red, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_25dBm_101ch_5mil_Dan.dat};
% \nextgroupplot
% [
% xticklabels={},
% yticklabels={},
% grid=major,ymin=32,ymax=42, xmin=1,xmax=101,
% %xticklabels={},
% %xlabel=Channel Number,
% %ylabel=Normalized NLI variance
% %(dB),
% title=PM-16QAM,legend style={at={(0.05,0.25)},anchor=west},
% %ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %}, 
% ]
% %ymin=1,ymax=1.07, 
% %%%%ytick={16,18,20,22,24,26,28},
% %yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %},
% %\addplot [green, line width=0.4mm, solid, mark repeat=10, mark=*] table[x index=0,y index=1] {Dat/NLIN_16QAM_noSRS_101ch_6mil.dat};
% \addplot [green, line width=0.4mm, solid, mark repeat=10, mark=*]table[x index=0,y index=1] {Dat/NLIN_16QAM_25dBm_101ch_5mil.dat};
% %\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_QPSK_15.dat};
% %\addplot [red, line width=0.4mm,dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_175.dat};
% %\addplot [green!60!black, line width=0.3mm]table[x index=0,y index=1] {Dat/NLIN_Gaussain_noSRS_101ch_6mil.dat};
% \addplot [blue, line width=0.4mm]table[x index=0,y index=1] {Dat/NLIN_Gaussian_25dBm_101ch_5mil.dat};
% \addplot [red, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_16QAM_25dBm_101ch_5mil_Dan.dat};
% %\addplot [brown, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_275_16QAM_Sem_2019.dat};
% %\legend{no SRS, $19$ dBm, $23$ dBm, $25$ dBm, $27.5$ dBm, $27.5$ dBm \cite{semrau2019modulation}}
% \nextgroupplot
% [
% xticklabels={},
% yticklabels={},
% grid=major,ymin=33,ymax=42, xmin=1,xmax=101,
% %xticklabels={},%xlabel=Channel Number,
% %ylabel=Normalized NLI variance
% %(dB),
% title=PM-64QAM,
% legend style={at={(0.05,0.25)},anchor=west},
% %ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %}, 
% ]
% %ymin=1,ymax=1.07, 
% %%%%ytick={16,18,20,22,24,26,28},
% %yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %},
% %\addplot [green, line width=0.4mm, solid, mark repeat=10, mark=*] table[x index=0,y index=1] {Dat/NLIN_16QAM_noSRS_101ch_6mil.dat};
% \addplot [green, line width=0.4mm, solid, mark repeat=10, mark=*]table[x index=0,y index=1] {Dat/NLIN_64QAM_25dBm_101ch_5mil.dat};
% %\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_QPSK_15.dat};
% %\addplot [red, line width=0.4mm,dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_175.dat};
% %\addplot [green!60!black, line width=0.3mm]table[x index=0,y index=1] {Dat/NLIN_Gaussain_noSRS_101ch_6mil.dat};
% \addplot [blue, line width=0.4mm]table[x index=0,y index=1] {Dat/NLIN_Gaussian_25dBm_101ch_5mil.dat};
% \addplot [red, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_64QAM_25dBm_101ch_5mil_Dan.dat};
% %\addplot [brown, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_275_16QAM_Sem_2019.dat};
% %\legend{no SRS, $19$ dBm, $23$ dBm, $25$ dBm, $27.5$ dBm, $27.5$ dBm \cite{semrau2019modulation}}
% \nextgroupplot
% [
% grid=major,ymin=31,ymax=41,ylabel=Normalized NLI variance (dB), xmin=1,xmax=101, xlabel=Channel Number, 
% %title=PM-QPSK,
% legend style={at={(0.05,0.25)},anchor=west},
% %ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %}, 
% ]
% %ymin=1,ymax=1.07, 
% %%%%ytick={16,18,20,22,24,26,28},
% %yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %},
% \addplot [green, line width=0.4mm, solid, mark repeat=10, mark=*] table[x index=0,y index=1] {Dat/NLIN_QPSK_noSRS_101ch_6mil.dat};
% \addplot [red, line width=0.5mm, dashed] table[x index=0,y index=1] {Dat/NLIN_QPSK_noSRS_101ch_6mil_Dan.dat};
% %\addplot [black, line width=0.4mm]table[x index=0,y index=1] {Dat/NLIN_QPSK_25dBm_101ch_5mil.dat};
% %\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_QPSK_15.dat};
% %\addplot [red, line width=0.4mm,dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_175.dat};
% %\addplot [red, line width=0.4mm, mark=*] table[x index=0,y index=1] {Dat/NLIN_QPSK_2.dat};
% \addplot [blue, line width=0.3mm]table[x index=0,y index=1] {Dat/NLIN_Gaussain_noSRS_101ch_6mil.dat};
% %\addplot [green!60!black, line width=0.4mm]table[x index=0,y index=1] {Dat/NLIN_Gaussian_25dBm_101ch_5mil.dat};
% %\addplot [brown, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_25dBm_101ch_5mil_Dan.dat};
% %\legend{no SRS, $19$ dBm, $23$ dBm, $25$ dBm, $27.5$ dBm, $27.5$ dBm \cite{semrau2019modulation}}
% \nextgroupplot
% [
% yticklabels={},
% grid=major,ymin=34,ymax=41, xmin=1,xmax=101, xlabel=Channel Number,
% %ylabel=Normalized NLI variance
% %(dB),
% %title=PM-16QAM,
% legend style={at={(0.05,0.25)},anchor=west},
% %ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %}, 
% ]
% %ymin=1,ymax=1.07, 
% %%%%ytick={16,18,20,22,24,26,28},
% %yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %},
% \addplot [green, line width=0.4mm, solid, mark repeat=10, mark=*] table[x index=0,y index=1] {Dat/NLIN_16QAM_noSRS_101ch_6mil.dat};
% \addplot [red, line width=0.5mm, dashed] table[x index=0,y index=1] {Dat/NLIN_16QAM_noSRS_101ch_6mil_Dan.dat};
% %\addplot [black, line width=0.4mm]table[x index=0,y index=1] {Dat/NLIN_16QAM_25dBm_101ch_5mil.dat};
% %\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_QPSK_15.dat};
% %\addplot [red, line width=0.4mm,dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_175.dat};
% \addplot [blue, line width=0.3mm]table[x index=0,y index=1] {Dat/NLIN_Gaussain_noSRS_101ch_6mil.dat};
% %\addplot [green!60!black, line width=0.4mm]table[x index=0,y index=1] {Dat/NLIN_Gaussian_25dBm_101ch_5mil.dat};
% %\addplot [brown, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_16QAM_25dBm_101ch_5mil_Dan.dat};
% %\addplot [brown, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_275_16QAM_Sem_2019.dat};
% %\legend{no SRS, $19$ dBm, $23$ dBm, $25$ dBm, $27.5$ dBm, $27.5$ dBm \cite{semrau2019modulation}}
% \nextgroupplot
% [
% yticklabels={},
% grid=major,ymin=34,ymax=41, xmin=1,xmax=101, xlabel=Channel Number,
% %ylabel=Normalized NLI variance
% %(dB),
% %title=PM-16QAM,
% legend style={at={(0.05,0.25)},anchor=west},
% %ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %}, 
% ]
% %ymin=1,ymax=1.07, 
% %%%%ytick={16,18,20,22,24,26,28},
% %yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %},
% \addplot [green, line width=0.4mm, solid, mark repeat=10, mark=*] table[x index=0,y index=1] {Dat/NLIN_64QAM_noSRS_101ch_6mil.dat};
% \addplot [red, line width=0.5mm, dashed] table[x index=0,y index=1] {Dat/NLIN_64QAM_noSRS_101ch_6mil_Dan.dat};
% %\addplot [black, line width=0.4mm]table[x index=0,y index=1] {Dat/NLIN_16QAM_25dBm_101ch_5mil.dat};
% %\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_QPSK_15.dat};
% %\addplot [red, line width=0.4mm,dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_175.dat};
% \addplot [blue, line width=0.3mm]table[x index=0,y index=1] {Dat/NLIN_Gaussain_noSRS_101ch_6mil.dat};
% %\addplot [green!60!black, line width=0.4mm]table[x index=0,y index=1] {Dat/NLIN_Gaussian_25dBm_101ch_5mil.dat};
% %\addplot [brown, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_16QAM_25dBm_101ch_5mil_Dan.dat};
% %\addplot [brown, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_275_16QAM_Sem_2019.dat};
% %\legend{no SRS, $19$ dBm, $23$ dBm, $25$ dBm, $27.5$ dBm, $27.5$ dBm \cite{semrau2019modulation}}
% \end{groupplot}
% \end{tikzpicture}
% \\
% \vspace*{7pt}
% \ref{benchmarkfigc}
% \end{center}
% \setlength{\belowcaptionskip}{-12pt}
% \caption{The normalized NLI variance as a function of channel number after one span in the presence of SRS (top row) for 25 dBm falt launch power and in the absence of SRS (bottom row) with PM-QPSK, PM-16QAM, and PM-64QAM modulations.} 
% \label{benchmarking_fig_cband}
% \end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%  We are benchmarking our numerical results against the recently published works \cite{semrau2018gaussian,semrau2019modulation}. As seen in Fig.~\ref{benchmarking_fig_cband}, the deviation between our model and the SRS GN model proposed in \cite{semrau2018gaussian} is about 4 dB for PM-QPSK modulation format in both scenarios (with and without SRS). This remarkable discrepancy stems from the fact that in \cite{semrau2018gaussian} all NLI terms such as SCI, XCI, and MCI evaluated for Gaussian modulation, while our model enables us to evaluate all these terms for non-Gaussian signals. In other words, by adding correction terms to all NLI terms we reduce the overestimation of NLI resulted form the Gaussianity assumption of signal. Fig.~\ref{benchmarking_fig_cband} also shows that the gap between our model and the modulation format dependent model proposed in \cite{semrau2019modulation} for PM-QPSK in both scenarios (with and without SRS) is about 2 dB. This is because the model proposed in \cite{semrau2019modulation} considers only SCI and XPM nonlinear terms and ignores the other XCI and MCI terms and therefore underestimates NLI. This gap becomes greater for smaller symbol rates. We thus find that one of the recently proposed model substantially overestimates NLI and the other underestimates NLI. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  \section{Discussion}

%  Our main objective in this section is to find an accurate nonlinearity model which is capable of correctly measuring NLI across a wide verity of scenarios. Authors of \cite{poggiolini2016analytical} simulatively and analytically investigated the prediction performance of some well-known nonlinearity models in the absence of SRS by evaluating the NLI impinging on the center WDM channels in scenarios with very different symbol rates. They found that using higher symbol rate than typical 32 Gbaud could actually results in performance loss in terms of reach increase, so exploiting low symbol rates have become of interest.
%  \cite{poggiolini2016analytical} further showed that the analitical results obtained through the EGN model are in good agreement with the simulation result obtained using split-step Fourier method. Other nonlinearity models, on the other hand, depart from the simulation results in low symbol rate scenarios. 

%  The same is true when we look at the WDM systems in the presence of SRS. To find an appropriate nonliearity model in C+L band systems, our model and two previously published models \cite{semrau2018gaussian, semrau2019modulation} are considered. We then examine these models at various symbol rates. To this end, a fixed WDM bandwidth (501 GHz) is chosen and broken up into different number of channels. We artificially inflate the Raman gain slope within this bandwidth, ensuring  significant power transfer due to the SRS. We plotted the normalized NLI variance falling over the center channel through three different nonlinearity models. As shown in this figure, all these models tend to converge to the GN model at very high symbol rates (small channel numbers). 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%









% \begin{figure*}[!t]
% \pgfplotsset{compat=1.3}
% \begin{center}
% \begin{tikzpicture}[scale=1]
% \begin{axis}[grid=major,
% width=9.35cm,height=7.5cm,
% %ymin=48,ymax=60,
% ylabel=Normalized NLI variance (dB), 
% xmin=1,xmax=51,
% xlabel=Number of Channels, title=PM-QPSK,legend style={at={(0.01,0.13)},anchor=west},
% xtick={1,11,21,31,41,51},xticklabels={
% $1$,
% $21$,
% $41$, 
% $61$, 
% $81$, 
% $101$,
% }, 
% ]
% %ymin=1,ymax=1.07, 
% %%%%ytick={16,18,20,22,24,26,28},
% %yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %},
% %\addplot [green, line width=0.4mm, solid, mark repeat=10, mark=*] table[x index=0,y index=1] {Dat/NLIN_QPSK_noSRS_100ch.dat};
% %\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_QPSK_15.dat};
% %\addplot [red, line width=0.4mm,dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_175.dat};
% %\addplot [red, line width=0.4mm, mark=*] table[x index=0,y index=1] {Dat/NLIN_QPSK_2.dat};
% \addplot [green, line width=0.4mm, solid, mark=*, mark repeat=10]table[x index=0,y index=1] {Dat/NLIN_QPSK_SRO.dat};
% \addplot[red, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_SRO_Dan.dat};
% \addplot [blue, line width=0.4mm, solid]table[x index=0,y index=1] {Dat/NLIN_Gaussian_SRO_Dan.dat};
% %\addplot [brown, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_275_QPSK_Sem_2019.dat};
% \legend{Our model, SCI+XPM model \cite{semrau2019modulation},SRS GN model \cite{semrau2018gaussian}}
% \end{axis}
% \end{tikzpicture}
% \hspace{-3mm}
% \begin{tikzpicture}[scale=1]
% \begin{axis}[grid=major,
% width=9.5cm,height=7.5cm,
% %ymin=48,ymax=60,
% xmin=0,xmax=51,
% xlabel=Number of Channels,title=PM-16QAM,legend style={at={(.1,0.13)},anchor=west},
% xtick={1,11,21,31,41,51},xticklabels={
% $1$,
% $21$,
% $41$, 
% $61$, 
% $81$, 
% $101$,
% }, 
% ]
% %ymin=1,ymax=1.07, 
% %%%%ytick={16,18,20,22,24,26,28},
% %yticklabels={
% %$16$,
% %$18$,
% %$20$, 
% %$22$, 
% %$24$, 
% %$26$,
% %$28$,  
% %},
% %\addplot [green, line width=0.4mm, solid, mark repeat=10, mark=*] table[x index=0,y index=1] {Dat/NLIN_16QAM_noSRS_100ch.dat};
% %\addplot [blue, line width=0.4mm, solid] table[x index=0,y index=1] {Dat/NLIN_QPSK_15.dat};
% %\addplot [red, line width=0.4mm,dashed]table[x index=0,y index=1] {Dat/NLIN_QPSK_175.dat};
% %\addplot [red, line width=0.4mm, mark=*] table[x index=0,y index=1] {Dat/NLIN_16QAM_2.dat};
% \addplot [green, line width=0.4mm, solid, mark=*, mark repeat=10]table[x index=0,y index=1] {Dat/NLIN_16QAM_SRO.dat};
% \addplot [red, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_16QAM_SRO_Dan.dat};
% \addplot [blue, line width=0.4mm, solid]table[x index=0,y index=1] {Dat/NLIN_Gaussian_SRO_Dan.dat};
% %\addplot [brown, line width=0.4mm, dashed]table[x index=0,y index=1] {Dat/NLIN_275_16QAM_Sem_2019.dat};
% \legend{Our model, SCI+XPM model \cite{semrau2019modulation},SRS GN model \cite{semrau2018gaussian}}
% \end{axis}
% \end{tikzpicture}

% %\\
% %\vspace*{2pt}
% %\ref{named}
% \end{center}
% \setlength{\belowcaptionskip}{-12pt}
% \caption{The normalized NLI variance obtined through three differrent models as a function of channel number after one span for 25 dBm spectrally flat launch power with PM-QPSK, PM-16QAM.} 
% \label{nlc_fig_discussion}
% \end{figure*}
% 
% In the following two sections, we are dealing with the properties of the nonlinear terms given in Table~\ref{DEFGH}, and how the SCI, XCI, and MCI terms can be obtained from (\ref{EGN_fixed}).






Fig.~\ref{nlc_fig} shows $\eta_\kappa$ as a function of channel number for standard single-mode fiber for systems with and without SRS. In that figure, the results presented in solid line were obtained using our model in \textit{Corollary} \ref{main.result.identical}, which are compared to the results in \cite{semrau2019modulation}. The reference given by SSFM simulations is represented by circle markers for PM-QPSK and PM-16QAM. The results for Gaussian modulation match the ones in \cite{semrau2018gaussian}, where they were already validated with SSFM simulations.   


As depicted in Fig.~\ref{nlc_fig}, changing the modulation format significantly impacts $\eta_\kappa$. For example, $\eta_\kappa$ for Gaussian modulation is approximately $3.9$ and $4.1$ dB higher than PM-QPSK for the $51$-th channel in the systems with and without SRS, respectively. This means the GN model presented in \cite{semrau2018gaussian} overestimates $\eta_\kappa$ due to the Gaussianity assumption of signal. The gap between PM-QPSK and PM-16QAM is approximately $1.6$ dB for no SRS. The origin of this deviation comes from the fact that PM-QPSK has the lowest excess kurtosis (given in Table~\ref{tab2}) among the exploited modulation formats. 
%These differences between $\eta_\kappa$ for different modulation formats can be explained by the values of $\Phi_b$ in Table~\ref{tab2}. When $\Phi_b$ is negative, the NLI is reduced in \eqref{EGN_fixed}. Therefore, since the lowest $\Phi_B$ is $-1$ for PM-QPSK, this modulation format experiences the lowest $\eta_\kappa$.



The modulation format dependence of $\eta_\kappa$ is well predicted by the model presented in this paper. The SSFM results are practically coinciding with the curves obtained using \textit{Corollary} \ref{main.result.identical} for both systems. The average gap between our model and SSFM simulations is approximately $0.18$ dB for PM-QPSK in the presence of SRS. The same match is not observed for the results using the model in \cite{semrau2019modulation}. For PM-16QAM in the presence of SRS, the model in \cite{semrau2019modulation} predicts $\eta_\kappa$ $2.8$ dB lower than SSFM simulation results for the $30$-th channel. For PM-QPSK, this gap increases to $3.2$ dB. This remarkable discrepancy stems from the fact that \cite{semrau2019modulation} considers only SCI (for Gaussian signal) and XPM (for no-Gaussian signal) nonlinear terms and ignores the other XCI and MCI terms, underestimating $\eta_\kappa$. Since XCI and MCI become dominant at small symbol rates, the results in \cite{semrau2019modulation} diverge from SSFM simulation for $10$ GBd, while our proposed model can still predict the SSFM results accurately.   








% Interpretation
%\input{Interpretation.tex}

==> Redan2.tex <==

\begin{figure*}%[!t]
\pgfplotsset{compat=1.3}
\begin{center}
\begin{tikzpicture}[x=0.2cm,y=0.2cm,scale=1]
\begin{groupplot}[group style={
group name=my plots, group size=2 by 2,horizontal sep=1.2cm,vertical sep=60pt},
%set layers=axis on top,
 %            axis line style={line width=1.5pt},
  %           every axis plot post/.append style={line width=1.5pt},
  %legend to name=leg,
%legend to name=Fig1,
grid,
 grid style = {
    dash pattern = on 0.05mm off 1mm,
    line cap = round,
    black,
    line width = 0.2mm
  },
 ylabel style={yshift=-0.15cm},
axis y line*=left,
axis x line*=bottom,
width=7cm,height=6cm]

\nextgroupplot
[
%legend to name=benchmarkfigc1,
%xticklabels={},
% ylabel={$\eta_\kappa \ [\text{dB} \ W^{-2}]$},
%grid=major,
%ymin=36,ymax=41, 
xmin=1,xmax=80,
%title=(a),
xlabel=Channel Number $n$, 
%title=16-point Constellations,
ylabel={$\eta_n$ [$\text{dB}W^{-2}$]},
%axis y line*=left,
%axis x line*=bottom,
%yticklabels={,,}
%($P_{\text{tot}}=25$ dBm),
%legend enteries={no SRS, $19$ dBm, $23$ dBm, $25$ dBm, $27.5$ dBm, $27.5$ dBm \cite{Semrau2019jlt}},
%legend to name=benchmarkfigc,
%xticklabels={},
%ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
%$16$,
%$18$,
%$20$, 
%$22$, 
%$24$, 
%$26$,
%$28$,  
%}, 
]

%\addplot [red, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_MAGNUSOptimized16_5span.dat};
%\addplot [green!60!black, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_QPSK.dat};%cube4_16,dicyclic4_16

%\addplot [mark=triangle, green!60!black, only marks, mark repeat=8]table[x index=0,y index=1] {Dat/NLIN_PMQPS.dat};

%\addplot [blue, line width=0.5mm]table[x index=0,y index=1] {Dat/NLIN_SO_PM_QPSK4_16.dat};

\addplot [blue, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_c4_16.dat};%1234/1423/1432/4132/4123/1432/1342/3142

\addplot [red, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_c4_16_4231.dat};%2431/4231

%\addplot [red, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_c4_16_4231.dat};


%\addplot [red, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_c4_16.dat};
%\addplot [blue, line width=0.5mm, solid, mark=circle,mark repeat=5]table[x index=0,y index=1] {Dat/Total_NLI_PPM4.dat};


%\addplot [purple, line width=0.5mm, solid,mark=triangle, mark repeat=5]table[x index=0,y index=1] {Dat/Total_NLI_orthogonal4.dat};

%\addplot [black, line width=0.5mm, solid,mark=triangle, mark repeat=5]table[x index=0,y index=1] {Dat/NLIN_var_orthogonal4_egn.dat};

%\addplot [blue, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_16point_10span.dat};

%\addplot [green, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_PMQPSK_5span.dat};



%\addplot [brown, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_SOPMQPSK_5span.dat};




%\addplot [blue, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_ps_qpsk__wdm_plot_50span_spacing_50ghz.dat};
%\addplot [green, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_64bin__wdm_plot_10span_spacing_50ghz.dat};

%\addplot [purple, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_64bin__wdm_plot_50span_spacing_50ghz.dat};

%\addplot [black, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_pm64__wdm_plot_10span_spacing_50ghz.dat};
%\addlegendentry{PM-16QAM (analytical \cite{Semrau2019jlt})}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\nextgroupplot
[
% legend style={at={(0.5,-0.435)},anchor=west,font=\footnotesize},
%legend columns=3,
%legend entries={PM-16QAM (EGN model), a4-256 (our model), voronoi4-256 (our model), a4-256 (EGN model), voronoi4-256 (EGN model)}, 
%legend to name=benchmarkfigc1,
%xticklabels={},
% ylabel={$\eta_\kappa \ [\text{dB} \ W^{-2}]$},
%grid=major,
%ymin=37,ymax=39.8, 
xmin=1,xmax=80,
%title=(a),
xlabel=Channel Number $n$, 
%title=256-point Constellations,
%title=With SRS,
ylabel={$\eta_n$ [$\text{dB} \ W^{-2}$]},
%axis y line*=left,
%axis x line*=bottom,
%yticklabels={,,}
%($P_{\text{tot}}=25$ dBm),
%legend enteries={no SRS, $19$ dBm, $23$ dBm, $25$ dBm, $27.5$ dBm, $27.5$ dBm \cite{Semrau2019jlt}},
%legend to name=benchmarkfigc,
%xticklabels={},
%ymax=26,
%ytick={36,38,40},yticklabels={
%$36\times 0.000001$,
%$38\times 0.000001$,
%$0.000040$, 
%$0.000042$, 
%$24$, 
%$26$,
%$28$,  
%}, 
]
\addplot [green!60!black, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_16QAM.dat};%QAM4_256

%\addplot [mark=triangle, green!60!black, only marks, mark repeat=8]table[x index=0,y index=1] {Dat/NLIN_PMQPS.dat};

%\addplot [blue, line width=0.5mm]table[x index=0,y index=1] {Dat/NLIN_QAM4_256.dat};

\addplot [blue, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_voronoi4_256.dat};



\addplot [red, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_w4_256.dat};%a4_256,ab4_256

%\addplot [brown, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_a4_256.dat};

%\addplot [magenta, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_ab4_256.dat};


%\addplot [red, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_w4_64.dat};%w4


%\addplot [black, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_w4_256_egn.dat};

%\addplot [cyan, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_w4_64_egn.dat};%ab4

%\addplot [blue, line width=0.5mm, solid, mark=circle,mark repeat=5]table[x index=0,y index=1] {Dat/Total_NLI_PPM4.dat};


%\addplot [purple, line width=0.5mm, solid,mark=triangle, mark repeat=5]table[x index=0,y index=1] {Dat/Total_NLI_orthogonal4.dat};

%\addplot [black, line width=0.5mm, solid,mark=triangle, mark repeat=5]table[x index=0,y index=1] {Dat/NLIN_var_orthogonal4_egn.dat};

%\addplot [blue, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_16point_10span.dat};

%\addplot [green, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_PMQPSK_5span.dat};



%\addplot [brown, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_SOPMQPSK_5span.dat};




%\addplot [blue, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_ps_qpsk__wdm_plot_50span_spacing_50ghz.dat};
%\addplot [green, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_64bin__wdm_plot_10span_spacing_50ghz.dat};

%\addplot [purple, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_64bin__wdm_plot_50span_spacing_50ghz.dat};

%\addplot [black, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_pm64__wdm_plot_10span_spacing_50ghz.dat};
%\addlegendentry{PM-16QAM (analytical \cite{Semrau2019jlt})}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\nextgroupplot
[
% legend style={at={(0.5,-0.435)},anchor=west,font=\footnotesize},
%legend columns=3,
%legend entries={PM-16QAM (EGN model), a4-256 (our model), voronoi4-256 (our model), a4-256 (EGN model), voronoi4-256 (EGN model)}, 
%legend to name=benchmarkfigc1,
%xticklabels={},
% ylabel={$\eta_\kappa \ [\text{dB} \ W^{-2}]$},
%grid=major,
%ymin=37,ymax=39.8, 
xmin=1,xmax=80,
%title=(a),
xlabel=Channel Number $n$, 
%title=256-point Constellations,
%title=With SRS,
ylabel={$\eta_n$ [$\text{dB} \ W^{-2}$]},
%axis y line*=left,
%axis x line*=bottom,
%yticklabels={,,}
%($P_{\text{tot}}=25$ dBm),
%legend enteries={no SRS, $19$ dBm, $23$ dBm, $25$ dBm, $27.5$ dBm, $27.5$ dBm \cite{Semrau2019jlt}},
%legend to name=benchmarkfigc,
%xticklabels={},
%ymax=26,
%ytick={36,38,40},yticklabels={
%$36\times 0.000001$,
%$38\times 0.000001$,
%$0.000040$, 
%$0.000042$, 
%$24$, 
%$26$,
%$28$,  
%}, 
]
\addplot [green!60!black, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_16QAM.dat};%QAM4_256

%\addplot [mark=triangle, green!60!black, only marks, mark repeat=8]table[x index=0,y index=1] {Dat/NLIN_PMQPS.dat};

%\addplot [blue, line width=0.5mm]table[x index=0,y index=1] {Dat/NLIN_QAM4_256.dat};

\addplot [blue, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_voronoi4_256.dat};



\addplot [red, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_w4_256.dat};%a4_256,ab4_256

%\addplot [brown, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_a4_256.dat};

%\addplot [magenta, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_ab4_256.dat};


%\addplot [red, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_w4_64.dat};%w4


%\addplot [black, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_w4_256_egn.dat};

%\addplot [cyan, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_w4_64_egn.dat};%ab4

%\addplot [blue, line width=0.5mm, solid, mark=circle,mark repeat=5]table[x index=0,y index=1] {Dat/Total_NLI_PPM4.dat};


%\addplot [purple, line width=0.5mm, solid,mark=triangle, mark repeat=5]table[x index=0,y index=1] {Dat/Total_NLI_orthogonal4.dat};

%\addplot [black, line width=0.5mm, solid,mark=triangle, mark repeat=5]table[x index=0,y index=1] {Dat/NLIN_var_orthogonal4_egn.dat};

%\addplot [blue, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_16point_10span.dat};

%\addplot [green, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_PMQPSK_5span.dat};



%\addplot [brown, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_SOPMQPSK_5span.dat};




%\addplot [blue, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_ps_qpsk__wdm_plot_50span_spacing_50ghz.dat};
%\addplot [green, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_64bin__wdm_plot_10span_spacing_50ghz.dat};

%\addplot [purple, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_64bin__wdm_plot_50span_spacing_50ghz.dat};

%\addplot [black, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_pm64__wdm_plot_10span_spacing_50ghz.dat};
%\addlegendentry{PM-16QAM (analytical \cite{Semrau2019jlt})}
%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\nextgroupplot
[
% legend style={at={(0.5,-0.435)},anchor=west,font=\footnotesize},
%legend columns=3,
%legend entries={PM-16QAM (EGN model), a4-256 (our model), voronoi4-256 (our model), a4-256 (EGN model), voronoi4-256 (EGN model)}, 
%legend to name=benchmarkfigc1,
%xticklabels={},
% ylabel={$\eta_\kappa \ [\text{dB} \ W^{-2}]$},
%grid=major,
%ymin=37,ymax=39.8, 
xmin=1,xmax=80,
%title=(a),
xlabel=Channel Number $n$, 
%title=256-point Constellations,
%title=With SRS,
ylabel={$\eta_n$ [$\text{dB} \ W^{-2}$]},
%axis y line*=left,
%axis x line*=bottom,
%yticklabels={,,}
%($P_{\text{tot}}=25$ dBm),
%legend enteries={no SRS, $19$ dBm, $23$ dBm, $25$ dBm, $27.5$ dBm, $27.5$ dBm \cite{Semrau2019jlt}},
%legend to name=benchmarkfigc,
%xticklabels={},
%ymax=26,
%ytick={36,38,40},yticklabels={
%$36\times 0.000001$,
%$38\times 0.000001$,
%$0.000040$, 
%$0.000042$, 
%$24$, 
%$26$,
%$28$,  
%}, 
]
\addplot [green!60!black, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_16QAM.dat};%QAM4_256

%\addplot [mark=triangle, green!60!black, only marks, mark repeat=8]table[x index=0,y index=1] {Dat/NLIN_PMQPS.dat};

%\addplot [blue, line width=0.5mm]table[x index=0,y index=1] {Dat/NLIN_QAM4_256.dat};

\addplot [blue, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_voronoi4_256.dat};



\addplot [red, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_w4_256.dat};%a4_256,ab4_256

%\addplot [brown, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_a4_256.dat};

%\addplot [magenta, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/NLIN_ab4_256.dat};


%\addplot [red, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_w4_64.dat};%w4


%\addplot [black, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_w4_256_egn.dat};

%\addplot [cyan, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_w4_64_egn.dat};%ab4

%\addplot [blue, line width=0.5mm, solid, mark=circle,mark repeat=5]table[x index=0,y index=1] {Dat/Total_NLI_PPM4.dat};


%\addplot [purple, line width=0.5mm, solid,mark=triangle, mark repeat=5]table[x index=0,y index=1] {Dat/Total_NLI_orthogonal4.dat};

%\addplot [black, line width=0.5mm, solid,mark=triangle, mark repeat=5]table[x index=0,y index=1] {Dat/NLIN_var_orthogonal4_egn.dat};

%\addplot [blue, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_16point_10span.dat};

%\addplot [green, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_PMQPSK_5span.dat};



%\addplot [brown, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_SOPMQPSK_5span.dat};




%\addplot [blue, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_ps_qpsk__wdm_plot_50span_spacing_50ghz.dat};
%\addplot [green, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_64bin__wdm_plot_10span_spacing_50ghz.dat};

%\addplot [purple, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_64bin__wdm_plot_50span_spacing_50ghz.dat};

%\addplot [black, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_pm64__wdm_plot_10span_spacing_50ghz.dat};
%\addlegendentry{PM-16QAM (analytical \cite{Semrau2019jlt})}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5



\end{groupplot}
%\draw[->,>=stealth,thin] (60.5-18.5-22.5-11.4+4,20.5-6.8-9+1.1+2.5) -- (60.5-18.5-22.5-11.4+4,26-2.8-9+0.5+5.7);
%\node at (58-18.75-22.5-11.4+5.2-1+4,23-5.3+1.7-9+0.5+1.2+4) {\footnotesize{$2.8$}};


\draw[->,>=stealth,thin] (60.5-18.5-22.5-11.4-0.5+3.5+2.4,20.5-6.8-9+1.1+2.3+5+0.9) -- (60.5-18.5-22.5-11.4-0.5+3.5+2.4,26-2.8-9+0.5-4.8+3.85+5+1.2);
\node at (58-18.75-22.5-11.4+5.2-1.5-4+1+3.3+2.4,23-5.3+1.7-9+0.5+1.2-5+5.2+5+0.9) {\scriptsize{$1.68$}};

%\draw[->,>=stealth,thin] (60.5-18.5-22.5-11.4-0.5+3.5+31.5,20.5-6.8-9+1.1+2.3+4.9) -- (60.5-18.5-22.5-11.4-0.5+3.5+31.5,26-2.8-9+0.5-4.8+3.85+1.55);
%\node at (58-18.75-22.5-11.4+5.2-1.5-4+1+3.3+31.6,23-5.3+1.7-9+0.5+1.2-5+5.2+2) {\scriptsize{$0.3$}};

%\draw[->,>=stealth,thin] (60.5-18.5-22.5-11.4-0.5+3.5+31.5+1,20.5-6.8-9+1.1+2.3+4.9) -- (60.5-18.5-22.5-11.4-0.5+3.5+31.5+1,26-2.8-9+0.5-4.8+3.85+1.55+2.6);
%\node at (58-18.75-22.5-11.4+5.2-1.5-4+1+3.3+31.6+4,23-5.3+1.7-9+0.5+1.2-5+5.2+4.4) {\scriptsize{$0.6$}};

\draw[<-,>=stealth,thin] (60.5-18.5-22.5-11.4-0.5+25.5-16.9+37,20.5-6.8-9+1.1+4.5-23.5+26) -- (60.5-18.5-22.5-11.4-0.5+25.5-16.9+37,26-2.8-9+0.5-4.8+4.75-22+25.5);
\node at (58-18.75-22.5-11.4+5.2-1.5-4+25.5+1.3-16.9+37,23-5.3+1.7-9+0.5+1.2-5.3+5-23+26) {\scriptsize{$0.7$}};
%\draw [->] %(60.5-18.5-22.5-11.4-0.5+25.5,26-2.8-9+0.5-4.8+1.75) arc (-90:-10:-12pt);

\node at (1.4,21) {\small{(a)}};
\node at (1.4+33,21) {\small{(b)}};

\node at (1.4,21-32.5) {\small{(c)}};
\node at (1.4+33,21-32.5) {\small{(d)}};

%\node at (1.4,21-65) {\small{(e)}};
%\node at (1.4+33,21-65) {\small{(f)}};
%\node at (1.4,-6.5) {\footnotesize{(b)}};
%%%
%\node at (1.4+30.5,21) {\footnotesize{(c)}};
%\node at (1.4+30.5,-6.5) {\footnotesize{(d)}};
%%%
%\node at (1.4+61,21) {\footnotesize{(e)}};
%\node at (1.4+61,-6.5) {\footnotesize{(f)}};
%\node at (1.4,15-31.5) {\footnotesize{(c)}};
%\node at (1.4+21.9,15-31.5) {\footnotesize{(d)}};
%%%
%\node at (1.4,15-31.5-31.5) {\footnotesize{(e)}};
%\node at (1.4+21.9,15-31.5-31.5) {\footnotesize{(f)}};
%\draw[->,>=stealth,thin] (60.5-18.5-22.5-11.4-0.5+1.5,20.5-6.8-9+1.1+2.5) -- (60.5-18.5-22.5-11.4-0.5+1.5,26-2.8-9+0.5-4.8);
%\node at (58-18.75-22.5-11.4+5.2-1.5-4+6.5,23-5.3+1.7-9+0.5+1.2-5+1.8) {\scriptsize{$0.62$ dB}};
%\draw[->,>=stealth,thick] (61.5,20.5) -- (61.5,31.5);
%\node at (58+6.15,29) {\footnotesize{$2.5$ dB}};
%\draw[->,>=stealth,thick] (43-22.5,17.65-3.9) -- (43-22.5,19.7-4);
%\node at (45-22.5,11.5) {\footnotesize{$0.4$ dB}};
%\draw [->] (43-22.5,14.5) arc (90:-10:10pt);
\end{tikzpicture}
%\\
%\vspace*{7pt}
%\ref{leg}
\end{center}
\setlength{\belowcaptionskip}{-12pt}
\vspace*{-2mm}
\caption{{The top row illustrates $\eta_n$, defined in \eqref{eta_n},
as a function of channel number $n$ after 10 spans, while the bottom row illustrates the SNR of our channel of interest, i.e.,  $\text{SNR}_{40}$, as a function of launch power after 10 spans. The coordinates of all constellations are available online in the database of sphere packings \cite{Erik.database}. To benchmark our results against previous works, $\eta_n$ is computed through our model (\eqref{main.result}--\eqref{final.variance.total.main} and Table~\ref{kerr.terms}~(a)) and EGN model (\eqref{main.result}--\eqref{final.variance.total.main} and Table~\ref{kerr.terms}~(b)).
%SSFM simulations are represented by circle markers and numerical results using \textit{Corollary }\ref{main.result.identical} are represented by solid lines.
}} 
\label{nlc_fi6}
\end{figure*}

  \multirow{3}{*} {Term} & \multicolumn{2}{c|} {Expression} \\
   \cline{2-3} 
   &\multicolumn{1}{c|} {\bf(a)}& \multicolumn{1}{c|} {\bf(b)}\\
   % \cline{2-3}
    &\multicolumn{1}{c|}{4D model}&\multicolumn{1}{c|}{EGN model}\\
    \hline
    \hline
   $\displaystyle \Psi_1$ &
$\varphi_1-12\varphi_2+24+2\varphi_3+\varphi_4-12\varphi_5$ &
%%%%%%%%%%%%%%5
$\varphi_1-9\varphi_2+12$
\\
    \hline
    $\displaystyle \Psi_2$ &
$5\varphi_2-15+
%%
5\varphi_5
$&$5\varphi_2-10
$
\\
    \hline
    $\displaystyle \Psi_3$ &
$\varphi_2-3+\varphi_5$&$\varphi_2-2$
\\
    \hline  
  %  $\displaystyle \Psi_4$ &
%$3$&$3$
%\\
   % \hline      
%%%%%%%%%%%%%%%%%55
\hline
$\displaystyle \Phi_1$ &  $
5\varphi_6-15+
5\varphi_7
$&$
5\varphi_6-10
$
\\
%\hline
%$\displaystyle \Phi_2$ &  $ 6$&$6$
%\\
    \hline
    \end{tabular}

==> redundant.tex <==
and therefore the four dimensional summation over $h,k,h',k'$ given in \eqref{second.ter.nli.contri} can be written as
\begin{align}
    \label{four.dimesional.summ}
   &\sum_{h,k,h',k'}\mathbb{E}\{b_{h,\text{x}}b_{k,\text{x}}^*b_{h',\text{x}}^*b_{k',\text{y}}\}\text{e}^{i(w_1h-w_2k-w_1'h'+w_2'k')}=\nonumber\\&
   %%
   \mathbb{E}\{|b_{\text{x}}|^2b_{\text{x}}^*b_{\text{y}}\}\sum_{h}\text{e}^{i(w_1-w_2-w_1'+w_2')hT}+\nonumber\\&
   %%
   \mathbb{E}\{b_{\text{x}}\}\mathbb{E}\{{b_{\text{x}}^*}^2b_{\text{y}}\}\sum_{h\neq k}\text{e}^{iw_1h}\text{e}^{i(-w_2-w_1'+w_2')k}+
  %%
 \nonumber\\&\mathbb{E}\{b_{\text{x}}^*\}\mathbb{E}\{|b_{\text{x}}|^2b_{\text{y}}\}\sum_{h\neq k}\text{e}^{-iw_2k}\text{e}^{i(w_1-w_1'+w_2')h}+
  %%
  \nonumber\\&\mathbb{E}\{b_{\text{x}}^*\}\mathbb{E}\{|b_{\text{x}}|^2b_{\text{y}}\}\sum_{h\neq h'}\text{e}^{-iw_1'h'}\text{e}^{i(w_1-w_2+w_2')h}
+
  %%
  \nonumber\\&\mathbb{E}\{b_{\text{x}}^*\}\mathbb{E}\{|b_{\text{x}}|^2b_{\text{y}}\}\sum_{h\neq k'}\text{e}^{iw_2'k'}\text{e}^{i(w_1-w_2-w_1')k}
  +
  %%
  \nonumber\\&\mathbb{E}\{|b_{\text{x}}|^2\}\mathbb{E}\{b_{\text{x}}^*b_{\text{y}}\}\sum_{h\neq h'}\text{e}^{i(w_1-w_2)h}\text{e}^{i(-w_1'+w_2')h'}+
  %%
  \nonumber\\&\mathbb{E}\{|b_{\text{x}}|^2\}\mathbb{E}\{b_{\text{x}}^*b_{\text{y}}\}\sum_{h\neq k}\text{e}^{i(w_1-w_1')h}\text{e}^{i(-w_2+w_2')k}+
  %%
  \nonumber\\&\mathbb{E}\{{b_{\text{x}}^{*}}^2\}\mathbb{E}\{b_{\text{x}}b_{\text{y}}\}\sum_{h\neq k}\text{e}^{(iw_1+w_2')h}\text{e}^{i(-w_2-w_1')k}+
  %%
  \nonumber\\&\mathbb{E}\{|b_{\text{x}}|^2\}\mathbb{E}\{b_{\text{x}}^*\}\mathbb{E}\{b_{\text{y}}\}\sum_{h\neq h'\neq k'}\text{e}^{i(w_1-w_2)h}\text{e}^{-iw_1h'}\text{e}^{iw_2'k'}+
  %%
  \nonumber\\&\mathbb{E}\{{b_{\text{x}}^*}^2\}\mathbb{E}\{b_{\text{x}}\}\mathbb{E}\{b_{\text{y}}\}\sum_{h\neq k\neq h'}\text{e}^{i(-w_2-w_1')k}\text{e}^{iw_1h}\text{e}^{iw_2'k'}+
    %%
  \nonumber\\&\mathbb{E}\{b_{\text{x}}^*b_{\text{y}}\}\mathbb{E}\{b_{\text{x}}\}\mathbb{E}\{b_{\text{x}}^*\}\sum_{h\neq k\neq h'}\text{e}^{i(w_2'-w_1')h'}\text{e}^{iw_1h}\text{e}^{-iw_2k}+
  %%
  \nonumber\\&\mathbb{E}^2\{b_{\text{x}}^*\}\mathbb{E}\{b_{\text{x}}\}\mathbb{E}\{b_{\text{y}}\}\sum_{h\neq k\neq h'\neq k'}\text{e}^{iw_1h}\text{e}^{-iw_2k}\text{e}^{-iw_1'h'}\text{e}^{iw_2'k'},
\end{align}
where the triple summation in the ninth term can be written as
\begin{align}
    \label{3.sum.9th.term}
    &\sum_{h\neq h'\neq k'}\text{e}^{i(w_1-w_2)h}\text{e}^{-iw_1'h'}\text{e}^{iw_2'k'}=\nonumber\\&\sum_{h,h', k'}\text{e}^{i(w_1-w_2)h}\text{e}^{-iw_1'h'}\text{e}^{iw_2'k'}-\sum_{h, k'}\text{e}^{i(w_1-w_2-w_1')h}\text{e}^{iw_2'k'}-\nonumber\\&\sum_{h, h'}\text{e}^{i(w_1-w_2)h}\text{e}^{i(w_2'-w_1')h'}-\sum_{h, h'}\text{e}^{i(w_1-w_2+w_2')h}\text{e}^{-iw_1'h'}+\nonumber\\&\sum_{h}\text{e}^{i(w_1-w_2-w_1'+w_2')h}.
\end{align}
Using \eqref{identity.delta}, we can write  \eqref{3.sum.9th.term} as
\begin{align}
    \label{3.sum.9th.term.alt}
    &\sum_{h\neq h'\neq k'}\text{e}^{i(w_1-w_2)h}\text{e}^{-iw_1'h'}\text{e}^{iw_2'k'}=\delta(w_1-w_2)\delta(w_1')\delta(w_2')\nonumber\\&-\delta(w_1-w_2-w_1')\delta(w_2')-\delta(w_1-w_2)\delta(w_2'-w_1')-\nonumber\\&\delta(w_1-w_2+w_2')\delta(w_1')+\delta(w_1-w_2-w_1'+w_2').
\end{align}
The same procedure is true for the 10th, 11th, and 12th terms. The four dimensional summation in the last term of \eqref{four.dimesional.summ} is 
\begin{align}
    \label{four.d.sum.last.term}
    &\sum_{h\neq k \neq h'\neq k'}\text{e}^{iw_1h}\text{e}^{-iw_2k}\text{e}^{-iw_1'h'}\text{e}^{iw_2'k'}=\nonumber\\& \sum_{h,k,h',k'}\text{e}^{iw_1h}\text{e}^{-iw_2k}\text{e}^{-iw_1'h'}\text{e}^{iw_2'k'}-\nonumber\\&
    %%
    \sum_{h,h',k'}\text{e}^{i(w_1-w_2)h}\text{e}^{-iw_1'h'}\text{e}^{iw_2'k'}-\nonumber\\&
    %%
    \sum_{h,k,k'}\text{e}^{i(w_1-w_1')h}\text{e}^{-iw_2k}\text{e}^{iw_2'k'}-\nonumber\\&
    %%
    \sum_{h,k,h'}\text{e}^{i(w_1+w_2')h}\text{e}^{-iw_2k}\text{e}^{-iw_1'h'}-\nonumber\\&
    %%
    \sum_{h,k,k'}\text{e}^{iw_1h}\text{e}^{-i(w_2+w_1')k}\text{e}^{iw_2'k'}-\nonumber\\&
    %%
    \sum_{h,k,h'}\text{e}^{iw_1h}\text{e}^{-i(w_2-w_2')k}\text{e}^{-iw_1'h'}-\nonumber\\&
    %%
    \sum_{h,k,h'}\text{e}^{iw_1h}\text{e}^{-iw_2k}\text{e}^{-i(w_1'-w_2')h'}+
    %%
    \sum_{h,k}\text{e}^{iw_1h}\text{e}^{i(-w_2-w_1'+w_2')k}+\nonumber\\&
    %%
    \sum_{h,k}\text{e}^{-iw_2k}\text{e}^{i(w_1-w_1'+w_2')h}+
    %%
    \sum_{h,h'}\text{e}^{i(w_1-w_2+w_2')h}\text{e}^{-iw_1'h'}+\nonumber\\&
    %%
    \sum_{h,k'}\text{e}^{i(w_1-w_2-w_1')h}\text{e}^{iw_2'k'}-
    %%
    \sum_{h}\text{e}^{i(w_1-w_2-w_1'+w_2')h},
\end{align}
which, considering \eqref{identity.delta}, can be written as
\begin{align}
  \label{four.d.sum.last.term.alt.delta}
    &\sum_{h\neq k \neq h'\neq k'}\text{e}^{iw_1h}\text{e}^{-iw_2k}\text{e}^{-iw_1'h'}\text{e}^{iw_2'k'}=\nonumber\\&\delta(w_1)\delta(w_2)\delta(w_1')\delta(w_2')
    %%
    -\delta(w_1-w_2)\delta(w_1')\delta(w_2')-\nonumber\\&
    %%
    \delta(w_1-w_1')\delta(w_2)\delta(w_2')-
    %%
    \delta(w_1+w_2')\delta(w_2)\delta(w_1')-\nonumber\\&
    %%
    \delta(w_1)\delta(w_2+w_1')\delta(w_2')-
    %%
    \delta(w_1)\delta(w_2-w_2')\delta(w_1')-\nonumber\\&
    %%
    \delta(w_1)\delta(w_2)\delta(w_1'-w_2')+
    %%
    \delta(w_1)\delta(w_2'-w_2-w_1')+\nonumber\\&
    \delta(w_2)\delta(w_1-w_1'+w_2')+
    %%
    \delta(w_1-w_2+w_2')\delta(w_1')+\nonumber\\&
    %%
    \delta(w_1-w_2-w_1')\delta(w_2')-\delta(w_1-w_2-w_1'+w_2').
\end{align}
Considering \eqref{double.sum.l.l'.alt2}, \eqref{3.sum.9th.term.alt}, and \eqref{four.d.sum.last.term.alt.delta}, \eqref{second.ter.nli.contri} is expressed as
\begin{align}
    \label{2nd.total.cont}
       &\sigma_{\text{NLI},\text{x},2nd}^2=
       %%
       \frac{64}{81}\gamma^2\rho(w_1,w_2,w_3)\rho^*(w_1',w_2',w_3')\nonumber\\&\cdot
       %%
       \Big[(\mathbb{E}\{a_{\text{x}}a_{\text{y}}^*\}-\mathbb{E}\{a_{\text{x}}\}\mathbb{E}\{a_{\text{y}}^*\})\frac{2\pi}{T}\delta(w_3-w_3')+\nonumber\\&\mathbb{E}\{a_{\text{x}}\}\mathbb{E}\{a_{\text{y}}^*\}\frac{4\pi^2}{T^2}\delta(w_3)\delta(w_3')\Big]\nonumber\\&
       \cdot
       \Big[\mathbb{E}\{|b_{\text{x}}|^2b_{\text{x}}^*b_{\text{y}}\}\delta(w_1-w_2-w_1'+w_2')+\nonumber\\&
   %%
   \mathbb{E}\{b_{\text{x}}\}\mathbb{E}\{{b_{\text{x}}^*}^2b_{\text{y}}\}\nonumber\\&\cdot\left(\delta(w_1)\delta(-w_2-w_1'+w_2')-\delta(w_1-w_2-w_1'+w_2')\right)+
  %%
 \nonumber\\&\mathbb{E}\{b_{\text{x}}^*\}\mathbb{E}\{|b_{\text{x}}|^2b_{\text{y}}\}\nonumber\\&
 \cdot\left(\delta(w_2)\delta(w_1-w_1'+w_2')-\delta(-w_2+w_1-w_1'+w_2')\right)+
  %%
  \nonumber\\&\mathbb{E}\{b_{\text{x}}^*\}\mathbb{E}\{|b_{\text{x}}|^2b_{\text{y}}\}\nonumber\\&\cdot
  \left(\delta(w_1')\delta(w_1-w_2+w_2')-\delta(-w_1'+w_1-w_2+w_2')\right)
+
  %%
  \nonumber\\&\mathbb{E}\{b_{\text{x}}^*\}\mathbb{E}\{|b_{\text{x}}|^2b_{\text{y}}\}\nonumber\\&\cdot\left(\delta(w_2')\delta(w_1-w_2-w_1')-\delta(w_2'+w_1-w_2-w_1')\right)
  +
  %%
  \nonumber\\&\mathbb{E}\{|b_{\text{x}}|^2\}\mathbb{E}\{b_{\text{x}}^*b_{\text{y}}\}\nonumber\\&
  \left(\delta(w_1-w_2)\delta(-w_1'+w_2')-\delta(w_1-w_2-w_1'+w_2')\right)+
  %%
  \nonumber\\&\mathbb{E}\{|b_{\text{x}}|^2\}\mathbb{E}\{b_{\text{x}}^*b_{\text{y}}\}\nonumber\\&
  \left(\delta(w_1-w_1')\delta(-w_2+w_2')-\delta(w_1-w_2-w_1'+w_2')\right)+
  %%
  \nonumber\\&\mathbb{E}\{{b_{\text{x}}^{*}}^2\}\mathbb{E}\{b_{\text{x}}b_{\text{y}}\}\nonumber\\&
  \left(\delta(w_1+w_2')\delta(-w_2-w_1')-\delta(w_1-w_2-w_1'+w_2')\right)+
  %%
  \nonumber\\&\mathbb{E}\{|b_{\text{x}}|^2\}\mathbb{E}\{b_{\text{x}}^*\}\mathbb{E}\{b_{\text{y}}\}\nonumber\\&
  \cdot\Big(\delta(w_1-w_2)\delta(w_1')\delta(w_2')\nonumber\\&-\delta(w_1-w_2-w_1')\delta(w_2')-\delta(w_1-w_2)\delta(w_2'-w_1')-\nonumber\\&\delta(w_1-w_2+w_2')\delta(w_1')+\delta(w_1-w_2-w_1'+w_2')\Big)+
  %%
  \nonumber\\&\mathbb{E}\{{b_{\text{x}}^*}^2\}\mathbb{E}\{b_{\text{x}}\}\mathbb{E}\{b_{\text{y}}\}\nonumber\\&\cdot
  \Big(\delta(-w_2-w_1')\delta(w_1)\delta(w_2')\nonumber\\&-\delta(w_1-w_2-w_1')\delta(w_2')-\delta(-w_2-w_1')\delta(w_1+w_2')-\nonumber\\&\delta(w_1-w_2-w_1')\delta(w_2')+\delta(w_1-w_2-w_1'+w_2')\Big)+
    %%
  \nonumber\\&\mathbb{E}\{b_{\text{x}}^*b_{\text{y}}\}\mathbb{E}\{b_{\text{x}}\}\mathbb{E}\{b_{\text{x}}^*\}\nonumber\\&
  \cdot
  \Big(\delta(w_2'-w_1')\delta(w_1)\delta(w_2)\nonumber\\&-\delta(w_2'-w_1'+w_1)\delta(w_2)-\delta(w_2'-w_1')\delta(w_1-w_2)-\nonumber\\&\delta(w_2'-w_1'-w_2)\delta(w_1)+\delta(w_1-w_2-w_1'+w_2')\Big)+
  %%
  \nonumber\\&\mathbb{E}^2\{b_{\text{x}}^*\}\mathbb{E}\{b_{\text{x}}\}\mathbb{E}\{b_{\text{y}}\}\nonumber\\&\cdot\Big(\delta(w_1)\delta(w_2)\delta(w_1')\delta(w_2')
    %%
    -\delta(w_1-w_2)\delta(w_1')\delta(w_2')-\nonumber\\&
    %%
    \delta(w_1-w_1')\delta(w_2)\delta(w_2')-
    %%
    \delta(w_1+w_2')\delta(w_2)\delta(w_1')-\nonumber\\&
    %%
    \delta(w_1)\delta(w_2+w_1')\delta(w_2')-
    %%
    \delta(w_1)\delta(w_2-w_2')\delta(w_1')-\nonumber\\&
    %%
    \delta(w_1)\delta(w_2)\delta(w_1'-w_2')+
    %%
    \delta(w_1)\delta(w_2'-w_2-w_1')+\nonumber\\&
    \delta(w_2)\delta(w_1-w_1'+w_2')+
    %%
    \delta(w_1-w_2+w_2')\delta(w_1')+\nonumber\\&
    %%
    \delta(w_1-w_2-w_1')\delta(w_2')-\delta(w_1-w_2-w_1'+w_2')\Big)\Big]
%\end{align}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxx































By putting \eqref{momentum.expansion.2} and \eqref{cross-polarization NLI.2} into \eqref{Csp} and \eqref{Cxp}, resp., and then insert them into \eqref{G_x.noBias} we get
 \eqlab{G_x.noBias.2}
{
&\mathbb{E}\bigl\{|I_{i,l}|^2\bigr\}=\frac{64}{81}f_0^{3}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}( \\&\nonumber \delta_{\kappa_1-\kappa_2}\delta_{\kappa_2-\kappa+l}\cdot A_6
   +\\&\nonumber
   %%
\delta_{\kappa_2-\kappa+l}\cdot B_{4,2}+\\&\nonumber
   %%\\&\nonumber
\delta_{\kappa_2-\kappa+l}\cdot C_{4,2}+\\&\nonumber
   %%
\delta_{\kappa_1-\kappa_2}\cdot D_{4,2}\\&\nonumber+
   %%
\delta_{\kappa_1-\kappa+l}\cdot E_{4,2}+\\&\nonumber
   %%
\delta_{\kappa_1-\kappa+l}\cdot F_{4,2}+\\&\nonumber
%%
\cdot
G_{2,2,2}+\\&\nonumber
%%
\cdot H_{2,2,2}+\\&\nonumber
%%
\delta_{\kappa_2-\kappa+l}'{X}_{1}+\\&\nonumber+
%%
\delta_{\kappa_2-\kappa+l}{X}_{2}),
}










\indent {\bf{Product of fourth and second order moments:}}
Regarding Appendix~\ref{fourth.second. moments.lneql'}, the following moments should be taken into account.
\begin{itemize}
\item{
\begin{align}
\label{first.exp.l.l.7}
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\big\}.
\end{align}}
To form the fourth and second order moment, 
%%
\item{
\begin{align}\label{first.exp.l.l.9}
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_2'},p'}\xi_{\text{x},\small{\kappa_2},p}\big\},
\end{align}}
%%
\item{
\begin{align}
 \label{first.exp.l.l.11}
 &\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\big\},   
\end{align}
}
%%
\item{
\begin{align}
    \label{first.exp.l.l.13}
    &\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\big\},
\end{align}
}
%%
\item{
\begin{align}
    \label{first.exp.l.equal.l'.15}
    &\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_2'},p'}\xi_{\text{x},\small{\kappa_2},p}\big\}.
\end{align}
}
\end{itemize}


\indent{\bf{Product of second order moments:}} Considering Appendix~\ref{second.order.moments.l.neq.l'}, we should take into account the following situations.
\begin{itemize}
    \item {
       \begin{align}\label{second.order.first.term.l.l.1}
       &\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}
       \end{align}
    }
    %%
     \item {
  \begin{align}\label{second.order.first.term.l.l.2}&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\big\} 
  \end{align}
       }
          
\end{itemize}










which gives rise to
       \eqlab{self.pol.exp.sixth.order.moment}{ \mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},n}\xi_{\text{x},\small{\kappa_1},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1},n'}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}.
 }
   



















Due to the bias or non-fluctuating terms and using the fact that $\mathbb{E}\big\{\xi^2_{\text{x},\small{\kappa_1},m}\big\}=0$,
we find that for evaluating \eqref{self.pol.exp}, we must consider the following two situations 
\begin{align}
&\label{cond_el.1}\kappa_1=\kappa_1',\quad \kappa_2=\kappa_2',\\&
\label{cond_el.6}
\kappa_1=\kappa_2',\quad \kappa_2=\kappa_1'.
\end{align}
For the first situation \eqref{cond_el.1}, \eqref{Csp} can be written as 
 \eqlab{G_x.noBias.nosum.prime.first}
{
&C_{\text{sp}}=\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\nonumber\\&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\nonumber\\&\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}.
}
To evaluate the self-polarization expectation term
\eqlab{first.situation.self.pol.exp}{
\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\},
}
we need to take into consideration the following situations
\begin{align}
&\label{five.situations.first.term.1}\kappa_1\neq \kappa_1+\kappa_2-\kappa+l, \quad \kappa_2\neq \kappa_1+\kappa_2-\kappa+l,\quad \kappa_1\neq \kappa_2,\\&
\label{five.situations.first.term.2}\kappa_1= \kappa_1+\kappa_2-\kappa+l, \quad \kappa_1\neq \kappa_2,\\&
\label{five.situations.first.term.3}\kappa_2= \kappa_1+\kappa_2-\kappa+l, \quad \kappa_1\neq \kappa_2,\\&
\label{five.situations.first.term.4}\kappa_1\neq \kappa_1+\kappa_2-\kappa+l, \quad \kappa_1= \kappa_2,\\&
\label{five.situations.first.term.5}\kappa_1= \kappa_1+\kappa_2-\kappa+l, \quad \kappa_1= \kappa_2,
\end{align}
where for the first situation \eqref{five.situations.first.term.1}, \eqref{first.situation.self.pol.exp} has the following form
\eqlab{first.situation.self.pol}{
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},m'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\big\}\nonumber\\&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}.
}
Using the second order moment given in \cite[Appendix~E]{carena2014accuracy}, \eqref{first.situation.self.pol} is reduced to
\begin{equation}\label{d'}
\begin{split}
&R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m-m'}R|S(nf_0)|^{2}\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n-n'}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p-p'}=D',
\end{split}
\end{equation}
and we call this term as $D'$. 
For the second situation \eqref{five.situations.first.term.2}, we can write \eqref{first.situation.self.pol.exp} as
\eqlab{second.situation.self.pol}{
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi^{*}_{\text{x},\small{\kappa_1},n}\xi_{\text{x},\small{\kappa_1},n'}\big\}
\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\},
}
and using the second and fourth order moments given in \cite[Appendix~E]{carena2014accuracy}, we can write \eqref{second.situation.self.pol} as
\begin{equation}\label{e'}
\begin{split}
&\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mn'm'n}\delta_{m-m'}\delta_{n-n'}+\\&Rf_0U_{mn'm'n}\delta_{m-n-m'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\Big)\\&\Big(R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p-p'}\Big)=E',
\end{split}
\end{equation}
and we call this term as $E'$, in which
\begin{equation}\label{P_e'}
\begin{split}
&U_{mn'm'n}=S_{\kappa_1}(mf_0)S^*_{\kappa_1}(nf_0)S^*_{\kappa_1}(m'f_0)S_{\kappa_1}(n'f_0).
\end{split}
\end{equation}
For the third situation \eqref{five.situations.first.term.3}, we can write \eqref{first.situation.self.pol.exp} as
\eqlab{third.situation.self.pol}{
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},m'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_2},n}\xi_{\text{x},\small{\kappa_2},n'}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\},
}
and following the same procedure that we did in \eqref{second.situation.self.pol}, \eqref{third.situation.self.pol} is expressed as
\eqlab{f'}{
&\Big(R|S(mf_0)|^{2}\mathbb{E}\{|b_{x,\kappa_1}|^{2}\}\delta_{m-m'}\Big)\nonumber\\&\Big(R^{2}\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}U_{pn'p'n}\delta_{p-p'}\delta_{n-n'}+\\&Rf_0U_{pn'p'n}\delta_{p-n-p'+n'}\Big[\mathbb{E}\{|b_{x,\kappa_2}|^{4}\}-2\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}\Big]\Big)=F',
}
and we call this term as $F'$, where
\begin{equation}\label{P_f'}
\begin{split}
&U_{pn'p'n}=S_{\kappa_2}(pf_0)S^{*}_{\kappa_2}(nf_0)S^*_{\kappa_2}(p'f_0)S_{\kappa_2}(n'f_0).
\end{split}
\end{equation}
For the fourth situation \eqref{five.situations.first.term.4}, \eqref{first.situation.self.pol.exp} can be written as
\eqlab{fourth.situation.self.pol}{
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1},p}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}\nonumber\\&\cdot
\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\big\},
}
and following the same procedure that we did in \eqref{second.situation.self.pol} and \eqref{third.situation.self.pol}, we get
\begin{equation}\label{g'}
\begin{split}
&\Big(2R^{2}\mathbb{E}^{2}\{|b_{x,\kappa_1}|^{2}\}U_{mp'm'p}\delta_{m-m'}
\delta_{p-p'}+\\&R f_0U_{mp'm'p}\delta_{m-m'-p'+p}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2Rf_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\Big)\\&\Big(R|S(nf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n-n'}\Big)=G',
\end{split}
\end{equation}
and we call this term as $G'$. For the last situation \eqref{five.situations.first.term.5}, \eqref{first.situation.self.pol.exp} can be written as
\begin{equation}\label{h'}
\begin{split}
&H'=\Big(2R^{3}\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mnpm'n'p'}\delta_{m-m'}\delta_{n-n'}\delta_{p-p'}\Big)+\\&\Big(R^{2}f_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]U_{mnpm'n'p'}\\&
(4\delta_{m-m'}\delta_{p-n+n'-p'}+\delta_{n-n'}\delta_{m+p-m'-p'})\Big)+\Big(Rf_0\\&\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}-9\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}+12\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\\&U_{mnpm'n'p'}\delta_{m-n+p-m'+n'-p'}\Big),
\end{split}
\end{equation}
where
\begin{equation}\label{P_ell}
\begin{split}
&U_{mnpm'n'p'}=\nonumber\\&
S_{\kappa_1}(mf_0)S^*_{\kappa_1}(nf_0)S_{\kappa_1}(pf_0)S^*_{\kappa_1}(m'f_0)S_{\kappa_1}(n'f_0)S^*_{\kappa_2}(p'f_0).
\end{split}
\end{equation}
Putting all these terms together (\eqref{d'}, \eqref{e'}, \eqref{f'}, \eqref{g'}, and \eqref{h'}), we can express \eqref{first.situation.self.pol.exp} as
\begin{equation}\label{fo1}
\begin{split}
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}\\&=\\&\delta'_{\kappa_1-\kappa+l}\delta'_{\kappa_2-\kappa+l} \delta'_{\kappa-\kappa_2}D'+
\delta_{\kappa_2-\kappa+l}\delta'_{\kappa_1-\kappa_2}E'\\&+\delta_{\kappa_1-\kappa+l}\delta'_{\kappa_1-\kappa_2}F'+
\delta_{\kappa_1-\kappa_2}\delta'_{\kappa_1-\kappa+l}G'+\\&\delta_{\kappa_1-\kappa_2}\delta_{\kappa_1-\kappa_2-\kappa+l}H'.
\end{split}
\end{equation}

We proceed by evaluating  the second situation \eqref{cond_el.6}. For this situation, \eqref{G_x.noBias} can be written as 
 \eqlab{G_x.noBias.nosum.prime.second}
{
&G_{\text{\small{NLI}},\text{x},\kappa}(f)=\frac{64}{81}f_0^{3}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\nonumber\\&\sum_{i=-\infty}^{+\infty}\delta \big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p')\nonumber\\&\Big(\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\nonumber\\&\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}\Big),
}
and the self-polarization expectation term is equal to
\eqlab{first.situation}{
&
\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},m'}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}.
}
Following the same procedure that we did for the first situation \eqref{cond_el.1}, \eqref{first.situation} is equal to 
\begin{equation}\label{fo}
\begin{split}
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},m'}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}\\&=\\&\delta'_{\kappa_1-\kappa+l}\delta'_{\kappa_2-\kappa+l} \delta'_{\kappa-\kappa_2}{D}''+
\delta_{\kappa_2-\kappa+l}\delta'_{\kappa_1-\kappa_2}{E}''\\&+\delta_{\kappa_1-\kappa+l}\delta'_{\kappa_1-\kappa_2}{F}''+
\delta_{\kappa_1-\kappa_2}\delta'_{\kappa_1-\kappa+l}{G}'+\\&\delta_{\kappa_1-\kappa_2}\delta_{\kappa_1-\kappa_2-\kappa+l}{H}',
\end{split}
\end{equation}
where 
\begin{equation}\label{d''}
\begin{split}
&{D}''=R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m-p'}R|S(nf_0)|^{2}\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n-n'}R|S(pf_0)|^{2}\delta_{p-m'}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\},
\end{split}
\end{equation}
\begin{equation}\label{e''}
\begin{split}
&{E}''=\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mnp'n'}\delta_{m-p'}\delta_{n-n'}+\\&Rf_0U_{mnp'n'}\delta_{m-n-p'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\Big)\\&\Big(R|S(pf_0)|^{2}\mathbb{E}\{|b_{x,\kappa_2}|^{2}\}\delta_{p-m'}\Big)
\end{split}
\end{equation}
in which
\begin{equation}\label{P_e''}
\begin{split}
&U_{mnp'n'}=S(mf_0)S^*_{\kappa_1}(nf_0)S^{*}(p'f_0)S(n'f_0),
\end{split}
\end{equation}
and
\begin{equation}\label{f''}
\begin{split}
&{F}''=\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}U_{pnm'n'}\delta_{p-m'}\delta_{n-n'}+\\&Rf_0U_{pnm'n'}\delta_{p-n-m'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}\Big]\Big)\\&\Big(R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m-p'}\Big),
\end{split}
\end{equation}
in which
\begin{equation}\label{P_f''}
\begin{split}
&U_{pnm'n'}=S(pf_0)S^*(nf_0)S^{*}(m'f_0)S(n'f_0).
\end{split}
\end{equation}
\subsubsection{Cross-polarization NLI contributions}\label{ap_b}
For analysis of the cross polarization NLI effects, i.e., 
  \eqlab{G_x.noBias.cross.pol.tot}
{
&G_{\text{\small{NLI}},\text{x},\kappa}(f)=\frac{64}{81}f_0^{3}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{\kappa_1'=1}^{M}\sum_{\kappa_2'=1}^{M}\sum_{l=-1}^{1}\nonumber\\&\sum_{i=-\infty}^{+\infty}\delta \big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1',\kappa_2',\kappa}(m',n',p')\nonumber\\&\mathbb{E}\big\{\xi^{*}_{y,\kappa_1,m}\xi_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi_{y,\kappa_1',m'}\xi^{*}_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\&\cdot
\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}.
}
To evaluate
\eqlab{srtm}{
&\mathbb{E}\big\{\xi^{*}_{y,\kappa_1,m}\xi_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi_{y,\kappa_1',m'}\xi^{*}_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\&\cdot
\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\},
}
we must evaluate just a non zero situation, namely
\eqlab{}
{
\kappa_1=\kappa'_1,\quad \kappa_2=\kappa'_2,
}
and, hence,  \eqref{srtm} is expressed as
\eqlab{c}{
&\mathbb{E}\big\{\xi^{*}_{y,\kappa_1,m}\xi_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi_{y,\kappa_1,m'}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n'}\big\}\nonumber\\&\cdot
\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2,p'}\big\}.
}
Using the second and fourth order moments of $\xi$, we can express \eqref{c} as \eqlab{xcross.pol.term}{\delta'_{\kappa_2-\kappa+l}{X}_{\text{x}}+\delta_{\kappa_2-\kappa+l}{X}_{\text{x}}',
}
where
\eqlab{Xx}
{
&{X}_{\text{x}}=R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}\delta_{m-m'}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{y},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n-n'}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p-p'},
}
and
\eqlab{Xx'}
{
&{X}_{\text{x}}'=\Big(R^2 \mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}|S(mf_0)|^2|S(nf_0)|^2\delta_{m-m'}\delta_{n-n'}+\nonumber\\&Rf_0U_{mnm'n'}\delta_{m'-m-n'+n}\Big[\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\Big]\Big)\nonumber\\&\Big(R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p-p'}\Big),
}
where
\begin{equation}\label{P_e''}
\begin{split}
&U_{mnm'n'}=S(m'f_0)S^{*}(mf_0)S^{*}(n'f_0)S(nf_0).
\end{split}
\end{equation}
We can therefore write \eqref{G_x.noBias.cross.pol.tot} as
\eqlab{G_x.noBias.cross.pol.tot.sec}
{
&G_{\text{\small{NLI}},\text{x},\kappa}(f)=\frac{64}{81}f_0^{3}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{\kappa_1'=1}^{M}\sum_{\kappa_2'=1}^{M}\sum_{l=-1}^{1}\nonumber\\&\sum_{i=-\infty}^{+\infty}\delta \big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\nonumber\\&\delta'_{\kappa_2-\kappa+l}{X}_{\text{x}}+\delta_{\kappa_2-\kappa+l}{X}_{\text{x}}'.
}
\subsubsection{Total NLI PSD within polarization x}
Adding these NLI contributions (\eqref{fo1}, \eqref{fo}, and \eqref{xcross.pol.term}), we can write \eqref{G_x.noBias} as
\eqlab{G_x_d}
{
&G_{\text{\small{NLI},x},\kappa}(f)=\frac{64}{81}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\nonumber\\&\Big(\delta'_{\kappa_1-\kappa+l}\delta'_{\kappa_2-\kappa+l} \delta'_{\kappa_1-\kappa_2}\hat{D}+
\delta_{\kappa_2-\kappa+l}\delta'_{\kappa_1-\kappa_2}\hat{E}+\delta_{\kappa_1-\kappa+l}\nonumber\\&\delta'_{\kappa_1-\kappa_2}\hat{F}+
\delta_{\kappa_1-\kappa_2}\delta'_{\kappa_1-\kappa+l}\hat{G}+\delta_{\kappa_1-\kappa_2}\delta_{\kappa_1-\kappa+l}\hat{H}\Big),
}
where
\eqlab{DD'}
{
&\hat{D}=f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{D'}+\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p')\cdot{D''}+\nonumber\\&
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{\text{x}}\Bigg],
}
and
\eqlab{EE'}
{
&\hat{E}=f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{E'}+\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p')\cdot{E''}+\nonumber\\&
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{\text{x}}'\Bigg],
}
and
\eqlab{FF'}
{
&\hat{F}=f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{F'}+\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p')\cdot{F''}+\nonumber\\&
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{\text{x}}\Bigg],
}
and
\eqlab{GG'}
{
&\hat{G}=f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{G'}+\nonumber\\&
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{\text{x}}\Bigg],
}
and
\eqlab{HH'}
{
&\hat{H}=f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{H'}+\nonumber\\&
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{\text{x}}'\Bigg].
}
We can remove the summation over $(m',n',p')$ in \eqref{DD'} and, hence, we have
\eqlab{D.hat'.alt}
{
&\hat{D}=\Big[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot\Big( R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\Big]+\nonumber\\&
\Big[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n,m)\nonumber\\&\cdot\Big( 
R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Big]+\nonumber\\&
\Big[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&
R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{y},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big].
}
Since the single period of channel $h$ signal ${\boldsymbol{p}}_h(t)$ introduced in (\ref{PeriodicSignal_x}) and \eqref{PeriodicSignal_y} is chosen enough large, i.e., $f_0\rightarrow 0$, one may use in the limit continuous integral replacing discrete summation as
\eqlab{rim}
{
\lim_{f_0\rightarrow0}f_0\sum_{m}\Lambda(mf_0)=\int\text{d}f \Lambda(f).
}
Considering \eqref{PowerX/Y} and using the fact that $\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)=\varsigma_{\kappa_2,\kappa_1,\kappa}(p,n,m)$, we can rewrite \eqref{D.hat'.alt} in the continuous domain as
\eqlab{D.hat'.alt.continuous}
{
&\hat{D}=3\times\Big[\int_{-R/2}^{R/2}\text{d}f'\delta\big(f-f'-(\kappa-l)R\big)\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f'+f_2,f_2)|^2\nonumber\\&\cdot\Big( R|S(f_1)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}R|S(f_1-f'+f_2)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(f_2)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\Big].
}
Using the delta function property $A(f)\delta(f-f_0)=A(f_0)\delta(f-f_0)$, we get
\eqlab{D.hat'.alt.continuous.delta}
{
\hat{D}=&3\times\Big[\frac{P_{\kappa_1}}{2}\cdot \frac{P_{\kappa_1+\kappa_2-\kappa+l}}{2}\cdot \frac{P_{\kappa_2}}{2}\cdot R^3\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+f_2+(\kappa-l)R,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+f_2+(\kappa-l)R)|^{2}|S(f_2)|^{2}
\Big].
}
We can write \eqref{EE'} as
\eqlab{E.hat'.alt}
{
&\hat{E}=\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&\cdot R^2f_0U_{mn'm'n}|S(pf_0)|^{2}\delta_{m-n-m'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n,m)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m,n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n',p')\nonumber\\&\cdot R^2f_0U_{mnp'n'}|S(pf_0)|^{2}\delta_{m-n-p'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{y},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&R^2f_0U_{mnm'n'}|S(pf_0)|^{2}\delta_{m-n-m'+n'}\nonumber\\&\Big[\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\Big]\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg].
}

Considering \eqref{PowerX/Y} and using the fact that $\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)=\varsigma_{\kappa_2,\kappa_1,\kappa}(p,n,m)$, %and Letting $f_0\rightarrow 0$, \eqref{E.hat'.alt} is expressed as
we get
\eqlab{E.hat'.alt.integral.form}
{
&\hat{E}=\Bigg[\Big(3f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\nonumber\\&+\Big(2f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&\cdot R^2f_0U_{mn'm'n}|S(pf_0)|^{2}\delta_{m-n-m'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m,n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n',p')\nonumber\\&\cdot R^2f_0U_{mnp'n'}|S(pf_0)|^2\delta_{m-n-p'+n'}\nonumber\\&\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg].
}
Letting $f_0\rightarrow 0$, we get
\eqlab{E.hat'.alt.integral.form2}
{
&\hat{E}=\Bigg[\Big(3\times\Big[\frac{P_{\kappa_1}}{2}\cdot \frac{P_{\kappa_1+\kappa_2-\kappa+l}}{2}\cdot \frac{P_{\kappa_2}}{2}\cdot R^3\int_{-R/2}^{R/2}\text{d}f_1\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_2\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+f_2+(\kappa-l)R,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+f_2+(\kappa-l)R)|^{2}|S(f_2)|^{2}
\Big]
    \Big)\nonumber\\&+\Bigg[\Big(2\times\frac{P_{\kappa_1}^2}{4}\cdot\frac{P_{\kappa_2}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_1'\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot S(f_1)S(f_1-f+(\kappa-l)R+f_2)^*S(f_1')^*\nonumber\\&\cdot S(f_1'-f+(\kappa-l)R+f_2)|S(f_2)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&
\Big(\frac{P_{\kappa_1}^2}{4}\frac{P_{\kappa_2}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(f_2,f_2-f+(\kappa-l)R+f_2',f_2')\nonumber\\&\cdot S(f_1)S(f_1-f+(\kappa-l)R+f_2)^*S(f_2')^*\nonumber\\&\cdot S(f_2-f+(\kappa-l)R+f_2')|S(f_2)|^2\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)\Bigg],
}
and so we can write \eqref{E.hat'.alt.integral.form2} as
\eqlab{E.hat'.alt.integral.form3}
{
&\hat{E}=\Bigg[\Big(3\times\Big[\frac{P_{\kappa_1}^2}{4}\cdot \frac{P_{\kappa_2}}{2}\cdot R^3\int_{-R/2}^{R/2}\text{d}f_1\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_2\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+f_2+(\kappa-l)R,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+f_2+(\kappa-l)R)|^{2}|S(f_2)|^{2}
\Big]
    \Big)\nonumber\\&+\Bigg[\Big(3\times\frac{P_{\kappa_1}^2}{4}\cdot\frac{P_{\kappa_2}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_1'\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot S(f_1)S(f_1-f+(\kappa-l)R+f_2)^*S(f_1')^*\nonumber\\&\cdot S(f_1'-f+(\kappa-l)R+f_2)|S(f_2)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)\Bigg].
}

We can write \eqref{FF'} as
\eqlab{F.hat'.alt}
{
&\hat{F}=\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m}\sum_{p}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}^2\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{p'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n',p')\nonumber\\&\cdot R^2f_0U_{pn'p'n}|S(mf_0)|^{2}\delta_{p-n-p'+n'}\mathbb{E}\{|b_{x,\kappa_1}|^{2}\}\nonumber\\&\cdot\Big[\mathbb{E}\{|b_{x,\kappa_2}|^{4}\}-2\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}\Big]\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m}\sum_{p}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n,m)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}^2\{|b_{\text{x},\kappa_2}|^{2}\}
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',m)\nonumber\\&\cdot R^2f_0U_{pnm'n'}|S(mf_0)|^{2}\delta_{p-n-m'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}\Big]\cdot \mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m}\sum_{p}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}\nonumber\\&\mathbb{E}\{|b_{\text{y},\kappa_2}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}
\Bigg].
}
Considering \eqref{PowerX/Y} and using the fact that $\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)=\varsigma_{\kappa_2,\kappa_1,\kappa}(p,n,m)$, for $f_0\rightarrow 0$ we have
\eqlab{F.hat'.alt.integral.form}
{
&\hat{F}=\Bigg[3\times\Big(\frac{P_{\kappa_2}^2}{4}\cdot \frac{P_{\kappa_1}}{2}\cdot R^3 \int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+(\kappa-l)R+f_2)|^{2}|S(f_2)|^{2}
\Bigg]\nonumber\\&+\Bigg[\frac{P_{\kappa_2}^2}{4}\cdot \frac{P_{\kappa_1}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_2'\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2',f_2') \nonumber\\&\cdot S(f_2)S(f_1-f+(\kappa-l)R+f_2)^* S(f_2')^*\nonumber\\&\cdot S(f_1-f+(\kappa-l)R+f_2')|S(f_1)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{x,\kappa_2}|^{4}\}}{\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}}-2\Big]\Bigg]\nonumber\\&+
\Bigg[\frac{P_{\kappa_2}^2}{4}\frac{P_{\kappa_1}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(f_1',f_1-f+(\kappa-l)R+f_1,f_1)\nonumber\\&\cdot S(f_2)S(f_1-f+(\kappa-l)R+f_2)^*S(f_1')^*\nonumber\\&S(f_1'-f+(\kappa-l)R+f_1)|S(f_1)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}}-2\Big]\Bigg].
}
Since the second and third integral terms are the same, we can rewrite \eqref{F.hat'.alt.integral.form} as 
\eqlab{F.hat'.alt.integral.form2}
{
&\hat{F}=\Bigg[3\times\Big(\frac{P_{\kappa_2}^2}{4}\cdot \frac{P_{\kappa_1}}{2}\cdot R^3 \int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+(\kappa-l)R+f_2)|^{2}|S(f_2)|^{2}\Big)
\Bigg]\nonumber\\&+\Bigg[2\times\Big(\frac{P_{\kappa_2}^2}{4}\cdot \frac{P_{\kappa_1}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_2'\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2',f_2') \nonumber\\&\cdot S(f_2)S(f_1-f+(\kappa-l)R+f_2)^* S(f_2')^*\nonumber\\&\cdot S(f_1-f+(\kappa-l)R+f_2')|S(f_1)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{x,\kappa_2}|^{4}\}}{\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}}-2\Big]\Big)\Bigg].
}

We now deal with \eqref{GG'}, which can be expressed as
\eqlab{GG'.expansion}
{
&\hat{G}=\Bigg[\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\cdot
2R^{3}\mathbb{E}^{2}\{|b_{x,\kappa_1}|^{2}\}\nonumber\\&\cdot\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}|S(mf_0)|^2|S(pf_0)|^2|S(nf_0)|^{2}\Big)+\nonumber\\&\Big(f_0^{4}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n,p')\nonumber\\&\cdot R^2 S(mf_0)S(m'f_0)^*S(p'f_0)^*S(pf_0)|S(nf_0)|^{2}\delta_{m-m'-p'+p}\nonumber\\&\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2Rf_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\Big)\Bigg]\nonumber\\&+
\Bigg[f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\cdot R^3|S(mf_0)|^{2}\nonumber\\&\cdot |S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{y},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Bigg].
}
Letting $f_0\rightarrow 0$ and considering \eqref{PowerX/Y}, we get
\eqlab{GG'.expansion.integral}
{
&\hat{G}=\Bigg[3\times\Big(\frac{P_{\kappa_1}^2}{4}\cdot\frac{P_{\kappa_1+\kappa_2-\kappa+l}}{2}\cdot R^{3}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\cdot
\nonumber\\&\cdot|S(f_1)|^2|S(f_2)|^2|S(f_1-f+(\kappa-l)R+f_2)|^{2}\Big)\Bigg]+\\&\Bigg[\frac{P_{\kappa_1}^2}{4}\cdot\frac{P_{\kappa_1+\kappa_2-\kappa+l}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1-f+(\kappa-l)R+f_2,f_1-f_1'+f_2)\cdot S(f_1)\nonumber\\&\cdot  S(f_1')^*S(f_1-f_1'+f_2)^*S(f_2)|S(f_1-f+(\kappa-l)R+f_2)|^{2}\nonumber\\&\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Bigg].
}
 
We will now express the last term, i.e., \eqref{HH'} in the continues form. Eq.~\eqref{HH'} is therefore expressed as
\eqlab{HH'.expansion}
{
&\hat{H}=\Bigg[\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\nonumber\\&\cdot
2R^{3}\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}|S(mf_0)|^2|S(nf_0)|^2|S(pf_0)|^2\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{p'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n',p')\nonumber\\&\cdot R^{2}f_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]U_{mnpm'n'p'}\nonumber\\&
\cdot4\delta_{m-m'}\delta_{p-n+n'-p'}\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n,p')\nonumber\\&\cdot R^{2}f_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]U_{mnpm'n'p'}\nonumber\\&\cdot\delta_{n-n'}\delta_{m+p-m'-p'})\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\sum_{p'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p') Rf_0\nonumber\\&\cdot\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}-9\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}+12\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\nonumber\\&U_{mnpm'n'p'}\delta_{m-n+p-m'+n'-p'}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\nonumber\\&\cdot
R^3 \mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}|S(mf_0)|^2|S(nf_0)|^2|S(pf_0)|^{2}\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&\cdot Rf_0U_{mnm'n'}\delta_{m-n-m'+n'}\Big[\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\Big]\nonumber\\&R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p-p'}\Big)\Bigg].
}
Letting $f_0\rightarrow 0$ and considering \eqref{PowerX/Y}, we get
\eqlab{HH'.expansion.integral}
{
&\hat{H}=\Bigg[3\times\Big(\frac{P_{\kappa_1}^3}{8}\cdot R^{3}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\nonumber\\&\cdot
|S(f_1)|^2|S(f_1-f+(\kappa-l)R+f_2)|^2|S(f_2)|^2\Big)+\nonumber\\&4\times\Big(\cdot\frac{P_{\kappa_1}^3}{8}\cdot R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2',f_2')\nonumber\\&\cdot |S(f_1)|^2S(f_2)S(f_1-f+(\kappa-l)R+f_2)^*\nonumber\\&S(f_1-f+(\kappa-l)R+f_2')S(f_2')^*\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&\Big(\frac{P_{\kappa_1}^3}{8}\cdot R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1-f+(\kappa-l)R+f_2,f_1+f_2-f_1')\nonumber\\&\cdot |S(f_1-f+(\kappa-l)R+f_2)|^2S(f_1)S(f_1')^*\nonumber\\&S(f_2)S(f_1+f_2-f_1')^*\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&\Big(\frac{P_{\kappa_1}}{8}\cdot R\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2',f_2')\nonumber\\& S(f_1)S(f_1')^*S(f_2)S(f_2')^*S(f_1-f+(\kappa-l)R+f_2)\nonumber\\&S(f_1'-f+(\kappa-l)R+f_2')^* \nonumber\\&\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}}{\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}}-9\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}+12\Big]\Big)\Bigg]+\nonumber\\&
\Bigg[\frac{P_{\kappa_1}^3}{8}R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot S(f_1)S^*(f_1')S^*(f_1-f+(\kappa-l)R+f_2)\nonumber\\&S(f_1'-f+(\kappa-l)R+f_2)|S(f_2)|^{2}\Big[\frac{\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}}-2\Big]\Bigg].
}
Since the second integral term is the same as the last integral term, we can rewrite \eqref{HH'.expansion.integral} as
\eqlab{HH'.expansion.integral2}
{
&\hat{H}=\Bigg[3\times\Big(\frac{P_{\kappa_1}^3}{8}\cdot R^{3}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\nonumber\\&\cdot
|S(f_1)|^2|S(f_1-f+(\kappa-l)R+f_2)|^2|S(f_2)|^2\Big)+\nonumber\\&5\times\Big(\cdot\frac{P_{\kappa_1}^3}{8}\cdot R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2',f_2')\nonumber\\&\cdot |S(f_1)|^2S(f_2)S(f_1-f+(\kappa-l)R+f_2)^*\nonumber\\&S(f_1-f+(\kappa-l)R+f_2')S(f_2')^*\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&\Big(\frac{P_{\kappa_1}^3}{8}\cdot R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1-f+(\kappa-l)R+f_2,f_1+f_2-f_1')\nonumber\\&\cdot |S(f_1-f+(\kappa-l)R+f_2)|^2S(f_1)S(f_1')^*\nonumber\\&S(f_2)S(f_1+f_2-f_1')^*\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&\Big(\frac{P_{\kappa_1}}{8}\cdot R\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1-f+(\kappa-l)R+f_2,f_2')\nonumber\\& S(f_1)S(f_1')^*S(f_2)S(f_2')^*S(f_1-f+(\kappa-l)R+f_2)\nonumber\\&S(f_1'-f+(\kappa-l)R+f_2')^* \nonumber\\&\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}}{\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}}-9\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}+12\Big]\Big)\Bigg].
}

==> redundant2.tex <==
The constellation for this format is shown in Fig.~\ref{simplex_constellation}.
\tikzset{split fill/.style args={#1 and #2}{path picture={
    \fill [#1] (path picture bounding box.south west)
      rectangle (path picture bounding box.north);
    \fill [#2] (path picture bounding box.south)
      rectangle (path picture bounding box.north east);
}}}
\begin{figure}
\begin{tikzpicture}
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,thick},
  xmin=-5.5,xmax=5.5,ymin=-5.5,ymax=5.5,
   xticklabels={},
 yticklabels={},
  xlabel=$I$,
  ylabel=$Q$,
  title={x-pol},
  width=5.5cm,height=5.5cm,
 % grid=major,
  %grid style={thin,densely dotted,black!20}
  ]
\end{axis}

\fill[blue] (1.95+1.2,1.95) circle (0.15cm);

  \path[split fill=red and green] 
    (1.95-0.5,1.95+1.4) circle [radius=0.15cm]; 

  \path[split fill=purple and yellow] 
    (1.95-0.5,1.95-1.4) circle [radius=0.15cm]; 




\end{tikzpicture}
%%
\hspace{4pt}
\begin{figure}
\begin{tikzpicture}
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,thick},
  xmin=-5.5,xmax=5.5,ymin=-5.5,ymax=5.5,
   xticklabels={},
 yticklabels={},
  xlabel=$I$,
  ylabel=$Q$,
  title={x-pol},
  width=5.5cm,height=5.5cm,
 % grid=major,
  %grid style={thin,densely dotted,black!20}
  ]
\end{axis}
\fill[red] (1.95,1.98) circle (0.15cm);
%%
%%
\fill[blue] (1.95+1.2,1.98+1.2) circle (0.15cm);
%%
\fill[blue] (1.95+1.2,1.98-1.2) circle (0.15cm);
%%
\fill[blue] (1.95-1.2,1.98-1.2) circle (0.15cm);
%%
\fill[blue] (1.95-1.2,1.98+1.2) circle (0.15cm);
\end{tikzpicture}
%%
\hspace{4pt}
\begin{tikzpicture}
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,thick},
  xmin=-5.5,xmax=5.5,ymin=-5.5,ymax=5.5,
  xlabel=$I$,
  ylabel=$Q$,
  title={y-pol},
  width=5.5cm,height=5.5cm,
  xticklabels={},
  yticklabels={}
 % grid=major,
  %grid style={thin,densely dotted,black!20}
  ]
\end{axis}
\fill[blue] (1.95,1.98) circle (0.15cm);
%
\fill[red] (1.95+1.2,1.98+1.2) circle (0.15cm);
%
\fill[red] (1.95+1.2,1.98-1.2) circle (0.15cm);
%
\fill[red] (1.95-1.2,1.98-1.2) circle (0.15cm);
%
\fill[red] (1.95-1.2,1.98+1.2) circle (0.15cm);
\end{tikzpicture}
\caption{Constellation for PS-QPSK modulation format. Two different colors represent 4D symbols.}
\label{ps_qpsk_constellation}
\end{figure}
\begin{tikzpicture}
\begin{axis}[
  axis lines=middle,
  axis line style={Stealth-Stealth,thick},
  xmin=-5.5,xmax=5.5,ymin=-5.5,ymax=5.5,
  xlabel=$I$,
  ylabel=$Q$,
  title={y-pol},
  width=5.5cm,height=5.5cm,
  xticklabels={},
  yticklabels={}
 % grid=major,
  %grid style={thin,densely dotted,black!20}
  ]
\end{axis}
\fill[blue] (1.95,1.98) circle (0.15cm);
\fill[red] (1.95+1.4,1.98+1.4) circle (0.15cm);
\fill[green] (1.95-1.4,1.98-1.4) circle (0.15cm);
\fill[yellow] (1.95-1.4,1.98+1.4) circle (0.15cm);
\fill[purple] (1.95+1.4,1.98-1.4) circle (0.15cm);
\end{tikzpicture}
\caption{Constellation for PS-QPSK modulation format. Each color represents an individual 4D symbol.}
\label{simplex_constellation}
\end{figure}
\begin{ProofLemma}
 In \textit{Lemma}~\ref{multiple.span.extention}, we ignore the triplets $(m,n,p)$ in which $m=n$ or $p=n$, as these terms create a constant phase shift and can be interpreted as bias or non-fluctuating terms \cite{Mecozzi2012,Pontus_JLT_modeling_2013,carena2014egn}, and thus, irrelevant for the noise variance we would like to compute. The set $\mathcal{S}_{i,l}'$ can therefore be written as 
 \begin{align}\label{sil}
\mathcal{S}_{i,l}=&\Big\{(m,n,p)\in\mathbb{Z}^3: m-n+p=i,\; m\neq n,\nonumber\\&  p \neq n, \;  
-\frac{R}{2}\leq (m-n+p)f_0-lR\leq +\frac{R}{2} \Big\}.
\end{align}
The total nonlinear electrical field given in \eqref{NLI_elec_tot_detail} has the form
\eqlab{tot.nli.fild.periodic}{
E_{\text{x},\kappa}^{(1)}(L,f)=\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}I_{i,l}\cdot\delta(f-if_0-(\kappa-l)R)
}
where
%\eqlab{i.second}{
%&I_{i,l}=\imath \frac{8f_0^{3/2}}{9}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{m,n,p\in \mathcal{S}_{i,l}}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\nonumber\\&\cdot\xi_{\text{x},\kappa_2,p}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,p}
%\Big)\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p),
%}
\eqlab{i.second}{
&I_{i,l}=\imath \frac{8f_0^{3/2}}{9}\sum_{\kappa_1,\kappa_2 \in \mathcal{T}_{\kappa,l}}\sum_{m,n,p\in \mathcal{S}_{i,l}}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\nonumber\\&\cdot\xi_{\text{x},\kappa_2,p}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,p}
\Big)\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p),
} 
and $\mathcal{T}_{\kappa,l} = \{(\kappa_1,\kappa_2) \in \{1,\ldots,M\}^2: 1\le \kappa_1+\kappa_2-\kappa+l \le M\}
$. Considering \cite[Eqs.~(60), (61), (62)]{Poggiolini_analytical_model_2011}, we find that the power spectral density of \eqref{tot.nli.fild.periodic} can be expressed as 
\eqlab{psd.tot.nli.fild.periodic.f.final2}{
&G_{\text{\small{NLI}},\text{x},\kappa}(f)=
\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\mathbb{E}\bigl\{|I_{i,l}|^2\bigr\}\delta(f-if_0-(\kappa-l)R),
}
% in which
  %\eqlab{G_x_lequall'.nonbias}
%{
%&\mathbb{E}\bigl\{|I_{i,l}|^2\bigr\}=\frac{64}{81}f_0^{3}\sum_{\kappa_1,\kappa_2 \in \mathcal{T}_{\kappa,l}}\sum_{\kappa_1',\kappa_2' \in \mathcal{T}_{\kappa,l}}(C_{\text{sp}}+C_{\text{xp}}).
%}
Using the fact that the symbols in the y polarization are independent from those in the x polarization, we obtain from \eqref{i.second} 
\eqlab{G_x}
{
&\mathbb{E}\bigl\{|I_{i,l}|^2\bigr\}=\frac{64}{81}f_0^{3}\sum_{\kappa_1,\kappa_2 \in \mathcal{T}_{\kappa,l}}\sum_{\kappa_1',\kappa_2' \in \mathcal{T}_{\kappa,l}}\nonumber\\
&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1',\kappa_2',\kappa}(m',n',p')\nonumber\\
&\Big(\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\nonumber\\
%%%
&+\mathbb{E}\big\{\xi_{\text{x},\kappa_1,m}\xi^{*}_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\
%%
&+\mathbb{E}\big\{\xi^{*}_{\text{x},\kappa'_1,m'}\xi_{\text{x},\kappa'_1+\kappa'_2-\kappa+l,n'}\xi^{*}_{\text{x},\kappa'_2,p'}\xi_{\text{x},\kappa_2,p}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\big\}\nonumber\\
%%
& +\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}\Big).
} 
The expectation terms
\begin{align}\label{second.term.I.I*}
&\mathbb{E}\big\{\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\},
\end{align}
and  
\begin{align}\label{third.term.I.I*}
&\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\big\},
\end{align}
given in \eqref{G_x} are equal to zero.
Using \eqref{FourierSerisCoef1} we can express \eqref{second.term.I.I*} as
\begin{align}\label{independent.xi}
  & \mathbb{E}\big\{\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}=\\&\nonumber f_0S^*(m' f_0)S(n' f_0)\sum_{w_1=1}^{W}\sum_{w_2=1}^{W}\mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}{{b}}_{\text{y},{\kappa_1'+\kappa_2'-\kappa+l},w_2}\}\\&\nonumber\cdot\text{e}^{\imath\frac{2\pi}{W}(m'w_1-n'w_2)}.
\end{align}
To evaluate \eqref{independent.xi}, the following three situations should be taken into consideration.
\begin{enumerate}
    \item {when $\kappa_1'\neq \kappa_1'+\kappa_2'-\kappa+l$, the expectation term in \eqref{independent.xi} is equal to zero, namely
    \begin{align}
    &\mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}{{b}}_{\text{y},{\kappa_1'+\kappa_2'-\kappa+l},w_2}\}=\\&\nonumber\mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}\}\mathbb{E}\big\{{{b}}_{\text{y},{\kappa_1'+\kappa_2'-\kappa+l},w_2}\}=0,
    \end{align}so \eqref{independent.xi} becomes zero.}
    %%
      \item {when $\kappa_1'= \kappa_1'+\kappa_2'-\kappa+l$ and $m'\neq n'$,  \eqref{independent.xi} is 
\begin{align}\label{independent.xi.k1equalk2}
  &f_0S^*(m' f_0)S(n' f_0)\sum_{w_1=1}^{W}\sum_{w_2=1}^{W}\mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}{{b}}_{\text{y},{\kappa_1'},w_2}\}\\&\nonumber\cdot\text{e}^{\imath\frac{2\pi}{W}(m'w_1-n'w_2)},
\end{align}
    in which for $w_1\neq w_2$ we have \begin{align}
  \mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}{{b}}_{\text{y},{\kappa_1'},w_2}\}=\mathbb{E}\big\{b^{*}_{\text{y},{\kappa_1'},w_1}\}\cdot\mathbb{E}\big\{b_{\text{y},{\kappa_1'},w_2}\}=0.
\end{align}
    Eq.~\eqref{independent.xi.k1equalk2} is therefore equal to
    \begin{align}\label{independent.xi.k1equalk2.w1equalw2}
  &f_0S^*(m' f_0)S(n' f_0)\mathbb{E}\big\{|{{b}}_{\text{y},{\kappa_1'}}|^2\}\cdot\sum_{w_1=1}^{W}\text{e}^{\imath\frac{2\pi}{W}(m'-n')w_1},
\end{align}
where we assume that the channel is stationary, i.e., $\mathbb{E}\big\{|{{b}}_{\text{y},{\kappa_1'}}|^2\}=\mathbb{E}\big\{|{{b}}_{\text{y},{\kappa_1'},w_i}|^2\}$. The summation term in \eqref{independent.xi.k1equalk2.w1equalw2} is equal to
\begin{align}
    \sum_{w_1=1}^{W}\text{e}^{\imath\frac{2\pi}{W}(m'-n')w_1}=
\left\{ \begin{array}{l}
    0 \quad m'\neq n' \;\;\text{and}\;\; m'-n'\neq pW\\
    W \quad m'-n'=pW
  \end{array} \right.
\end{align}
where $p$ is an integer. This implies that there is correlation between spectral lines which are $pWf_0=pR$ apart, namely multiples of symbol rate. Since for the Nyquist case there is no two spectral lines which are $R$ apart, we find that $p=0$. This means Eq.~\eqref{independent.xi.k1equalk2.w1equalw2} is always equal to zero as $m'\neq n'$.
    }
    %%
          \item {when $\kappa_1'= \kappa_1'+\kappa_2'-\kappa+l$ and $m'=n'$, the situation is interpreted as a constant phase shift and does not belong to set $\mathcal{S}_{i,l}$
 given in \eqref{sil}, and should be ignored. 
    }
\end{enumerate}
The same procedure holds for $\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\big\}$ given in \eqref{third.term.I.I*}. We hence find that these expectation terms are zero and \eqref{psd.tot.nli.fild.periodic.f.final2} is then equal to 
\eqlab{psd.tot.nli.fild.periodic.f.final}{
&G_{\text{\small{NLI}},\text{x},\kappa}(f)=
\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\delta(f-if_0-(\kappa-l)R)\nonumber\\&\cdot\frac{64}{81}f_0^{3}\sum_{\kappa_1,\kappa_2 \in \mathcal{T}_{\kappa,l}}\sum_{\kappa_1',\kappa_2' \in \mathcal{T}_{\kappa,l}}\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\nonumber\\&\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1',\kappa_2',\kappa}(m',n',p')(C_{\text{sp}}+C_{\text{xp}}),
}
where
 \eqlab{Csp}
{
&C_{\text{sp}}=\nonumber\\
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\},
}
and
\eqlab{Cxp}
{
&C_{\text{xp}}=\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\
&
\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\},
}
\end{ProofLemma}



 %In the following lemma we deal with the bias and non-fluctuating terms. 
%\begin{lemma}\label{bias.terms}
%The NLI contributions resulted from situations in which $m=n$ or $p=n$ are of no consequence for transmission. In this regard, without loss of generality we consider the nonlinear electrical field at the end of the first span.
%The electrical field resulted form these terms is given by
% \eqlab{NLIN_expression_mn_f}
%{
%E_{\text{x},\kappa}^{(1)}(L_{1},f)&=-\imath\gamma\frac{8}{9}E_{\text{x}}^{(0)}(L_{s},f)P_{\text{tot},{|z=L_{s}}},
%}
%which causes phase shift terms and should not be taken into %\end{lemma}
 
 %\begin{IEEEproof}
% One can find that there exist situations,
%\eqlab{situ}
%{
%\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\delta_{m,n}\quad \text{or} \quad\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\delta_{p-n},
%}
%for instance, for $\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\delta_{m,n}$, where $\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}$ implies that $\kappa_1=\kappa_1+\kappa_2-\kappa+l$, \eqref{NLI_elec_tot_detail}
%(\ref{Zeta_ENL})
%is equal to
% \eqlab{NLI_elec_tot_detail.mn}
%{
%&E_{\text{x},\kappa}^{(1)}(L,f)=-\imath\frac{8}{9}f_0^{3/2}\sum_{\kappa_1=1}^{M}\sum_{m=-\infty}^{\infty}(|\xi_{\text{x},\kappa_1,m}|^2+|\xi_{\text{y},\kappa_1,m}|^2)\nonumber\\&\sum_{\kappa_2=1}^{M}\sum_{i=-\infty}^{\infty}\xi_{\text{x},\kappa_2,i}\cdot\delta(f-if_0-\kappa_2R)
%\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(m,i),
%}
%where we are using the fact that $i=p$ and
%\eqlab{varsigma.mn}{
%\varsigma_{\kappa_1,\kappa_2,\kappa}(m,i)=\sum_{s=1}^{N}\Xi^{(s)}_{\kappa_1,\kappa_2,\kappa}(m,i)\cdot\zeta^{(s)}_{\kappa_1,\kappa_2,\kappa}(m),
%}
%in which
%\begin{align}\label{Xi.mn}
%&\Xi^{(s)}_{\kappa_1,\kappa_2,\kappa}(m,i)=\Bigg[\prod_{s'=1}^{s-1}g_{s'}^{3/2}\cdot \rho(L_{s'},mf_0+\kappa_1 R)\nonumber\\&
%\cdot \sqrt{\rho(L_{s'},if_0+\kappa_2 R)}\nonumber\\&\cdot
 %   \prod_{s'=s}^{N}g_{s'}^{1/2}\sqrt{\rho(L_{s'},if_0+\kappa_2R)} \nonumber\\&\cdot\prod_{s'=1}^{N}\text{exp}\Big([\imath 2\pi^{2}\beta_{2,{s'}} (if_0+\kappa_2R)^{2}+\nonumber\\&\imath\frac{4}{3}\pi^3 \beta_{3,{s'}}(if_0+\kappa_2R)^3]L_{s'}\Big)\Bigg],
%\end{align}
%and
%\eqlab{zeta.s.mn}{
%&\zeta^{(s)}_{\kappa_1,\kappa_2,\kappa}(m)=\int_{0}^{L_{s}}\text{d}z'\sqrt{\rho(z',mf_0+\kappa_1 R)}.
%}
%Considering \eqref{E_input}, we find that \eqref{NLI_elec_tot_detail.mn} is equal to
% \eqlab{NLI_elec_tot_detail.mn.input}
%{
%&E_{\text{x},\kappa}^{(1)}(L,f)=-\imath\frac{8}{9}f_0\sum_{\kappa_1=1}^{M}\sum_{m=-\infty}^{\infty}(|\xi_{\text{x},\kappa_1,m}|^2+|\xi_{\text{y},\kappa_1,m}|^2)\nonumber\\&E_{\text{x}}(0,f)
%\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(m,i),
%}
%\end{IEEEproof}
\subsubsection{Evaluation of \eqref{Csp}} 
To evaluate \eqref{Csp}, the sixth, fourth and second order moments need to be considered, namely \eqref{Csp} can be written as 
\begin{align}\label{momentum.expansion}
   &\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\} \\&\nonumber=\\&\nonumber
   \delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\\&\nonumber\cdot
   \mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},n}\xi_{\text{x},\small{\kappa_1},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1},n'}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_2'}\delta_{\kappa_2,\kappa_1'}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},n}\xi_{\text{x},\small{\kappa_1},n'}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},m'}\big\}+\\&\nonumber
   %%\\&\nonumber
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},n}\xi_{\text{x},\small{\kappa_1},n'}\xi^{*}_{\text{x},\small{\kappa_1},m'}\big\}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi_{\text{x},\small{\kappa_1},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}\mathbb{E}\\&\nonumber\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\big\}\\&\nonumber+
%%%%%%%%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},n}\xi_{\text{x},\small{\kappa_2},n'}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},m'}\big\}+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_2'}\delta_{\kappa_2,\kappa_1'}\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},n}\xi^{*}_{\text{x},\small{\kappa_2},m'}\xi_{\text{x},\small{\kappa_2},n'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1},p'}\xi_{\text{x},\small{\kappa_1},m}\big\}+\\&\nonumber
%%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\bar{\delta}_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\\&\nonumber\cdot
\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},m'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\big\}\\&\nonumber\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}+\\&\nonumber
%%
\delta_{\kappa_1,\kappa_2'}\delta_{\kappa_2,\kappa_1'}\bar{\delta}_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},m'}\big\},
\end{align}
where $\bar{\delta}_{i,j}$ implies that $i\neq j$.
Using the sixth, fourth, and second order moments given in \cite[Eq.~(105)]{carena2014accuracy}, \cite[Eq.~(100)]{carena2014accuracy}, and \cite[Eq.~(95)]{carena2014accuracy}, resp., and removing the bias terms from them we can write \eqref{momentum.expansion} as
\begin{align}\label{momentum.expansion.2}
   &\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\} \\&\nonumber=\\&\nonumber
   \delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\cdot A_6
   +\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_2'}\delta_{\kappa_2,\kappa_1'}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\cdot B_{4,2}+\\&\nonumber
   %%\\&\nonumber
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\cdot C_{4,2}+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\cdot  D_{4,2}+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\cdot E_{4,2}+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_2'}\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\cdot F_{4,2}+\\&\nonumber
%%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\bar{\delta}_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\cdot
G_{2,2,2}+\\&\nonumber
%%
\delta_{\kappa_1,\kappa_2'}\delta_{\kappa_2,\kappa_1'}\bar{\delta}_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\cdot H_{2,2,2},
\end{align}
in which
 \begin{table*}[t]
    %\renewcommand{\arraystretch}{2.5}
    \footnotesize
    \centering
    \caption{Integral expressions for the terms used in \textit{Lemma}~\ref{Lemma.psd}.}
    \label{A6}
    \begin{tabular}{|c|l|}
    \hline
    
    \hline
    Term & Integral Expression \\
    \hline
    
    \hline
$\displaystyle A_6$ &  $\Big(2R^{3}\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mnpm'n'p'}\delta_{m,m'}\delta_{n,n'}\delta_{p,p'}\Big)+\Big(R^{2}f_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]U_{mnpm'n'p'}(4\delta_{m,m'}\delta_{p-n+n'-p',0}$\\&$+\delta_{n,n'}\delta_{m+p-m'-p',0})\Big)+\Big(Rf_0\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}-9\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}+12\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}\Big] U_{mnpm'n'p'}\delta_{m-n+p-m'+n'-p',0}\Big)$
\\
\hline
$\displaystyle B_{4,2}$ &  $\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mn'p'n}\delta_{m,p'}\delta_{n,n'}+Rf_0U_{mn'p'n}\delta_{m-n-p'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\Big)\Big(R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,m'}\Big)$
\\
\hline
$\displaystyle C_{4,2}$ &
$\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mn'm'n}\delta_{m,m'}\delta_{n,n'}+Rf_0U_{mn'm'n}\delta_{m-n-m'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\Big)\Big(R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,p'}\Big)$
\\
\hline
$\displaystyle D_{4,2}$ &
$\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mm'p'p}\delta_{m,m'}\delta_{p,p'}+Rf_0U_{mm'p'p}\delta_{m-m'-p'+p,0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\Big)$\\&$\cdot\Big(R|S(nf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n,n'}\Big)$
\\
\hline
$\displaystyle E_{4,2}$ &
$\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}U_{pn'p'n}\delta_{p,p'}\delta_{n,n'}+Rf_0U_{pn'p'n}\delta_{p-n-p'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}\Big]\Big)\Big(R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m,m'}\Big)$
\\
\hline
$\displaystyle F_{4,2}$ &$\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}U_{npm'n'}\delta_{p,m'}\delta_{n,n'}+Rf_0U_{npm'n'}\delta_{p-n-m'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}\Big]\Big)\Big(R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m,p'}\Big)$
\\
\hline
$\displaystyle G_{2,2,2}$ &$R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m,m'}R|S(nf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n,n'}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,p'}$
\\
\hline
$\displaystyle H_{2,2,2}$ &$R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m,p'}R|S(nf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n,n'}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,m'}$
\\
\hline
$\displaystyle U_{mnpm'n'p'}$ &$
S(mf_0)S^*(nf_0)S(pf_0)S^*(m'f_0)S(n'f_0)S^*(p'f_0)$
\\
\hline
    \end{tabular}
\end{table*}
%%%%%%%%%%%%%%
\subsubsection{Evaluation of \eqref{Cxp}} For analysis of \eqref{Cxp}, the non-zero situations should be evaluated.
We use the second and fourth order moments provided in \cite[Appendix~E, Eqs.~(95) and (100)]{carena2014accuracy} and remove the bias terms form them, and  rewrite \eqref{Cxp} as
\begin{align}\label{cross-polarization NLI.2}
&\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\
&
\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}=\\&\nonumber   \delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\cdot X_1
   +\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\cdot X_1+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\cdot  X_2+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\cdot X_2+\\&\nonumber
%%
\delta_{\kappa_1,\kappa_1'}\bar{\delta}_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\cdot
X_2,
\end{align}
where
\eqlab{X1}
{
&{X}_{1}=\Big(R^2 \mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}|S(mf_0)|^2|S(nf_0)|^2\delta_{m,m'}\delta_{n,n'}+\nonumber\\&Rf_0U_{mnm'n'}\delta_{m'-m-n'+n,0}\Big[\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\Big]\Big)\nonumber\\&\Big(R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,p'}\Big),
}
and
\eqlab{X2}
{
&{X}_{2}=R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}\delta_{m,m'}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{y},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n,n'}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,p'}.
}
%%%%%%%%%%%%%


By substituting \eqref{momentum.expansion.2} and \eqref{cross-polarization NLI.2} into \eqref{Csp} and \eqref{Cxp}, resp, and then inserting them into \eqref{psd.tot.nli.fild.periodic.f.final} the total nonlinear PSD can be written as
\eqlab{G_x_d}
{
&G_{\text{\small{NLI}},\text{x},\kappa}(f)=\frac{64}{81}\sum_{\kappa_1,\kappa_2,l \in \mathcal{T}_{\kappa}}\nonumber\\&\Big(\bar{\delta}_{\kappa_2,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l} \bar{\delta}_{\kappa_1,\kappa_2}\hat{D}+\\&\nonumber
\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\hat{E}+\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\hat{F}\\&\nonumber+
\delta_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_1+\kappa_2-\kappa+l}\hat{G}+\delta_{\kappa_1,\kappa_2}\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\hat{H}\Big),
}
where $\hat{D}$, $\hat{E}$, $\hat{F}$, $\hat{G}$, and $\hat{H}$ are given in Table~\ref{hat.DEFGH}.
 \begin{table*}[t]
    %\renewcommand{\arraystretch}{2.5}
    \footnotesize
    \centering
    \caption{Integral expressions for the terms used in \textit{Lemma}~\ref{Lemma.psd}.}
    \label{hat.DEFGH}
    \begin{tabular}{|c|l|}
    \hline
    
    \hline
    Term & Integral Expression \\
    \hline
    
    \hline
$\displaystyle \hat{D}$ &  $f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{G_{2,2,2}}+\sum_{m,n,p\in \mathcal{S}_{i,l}}$\\&$\cdot\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p')\cdot{H_{2,2,2}}+
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{2}\Bigg]$
\\
\hline
$\displaystyle \hat{E}$ &  $f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p'){B_{4,2}}+\sum_{m,n,p\in \mathcal{S}_{i,l}}$\\&$\cdot\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p'){C_{4,2}}+
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p'){X}_{1}\Bigg]$
\\
\hline
$\displaystyle \hat{F}$ &
$f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p'){E_{4,2}}+\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}$\\&$\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p'){F_{4,2}}+
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p'){X}_{2}\Bigg]
$
\\
\hline
$\displaystyle \hat{G}$ &
$f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{D_{4,2}}+$\\&$\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{2}\Bigg]$
\\
\hline
$\displaystyle \hat{H}$ &
$f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{A_{6}}+$\\&$
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{1}\Bigg]$
\\
\hline
    \end{tabular}
\end{table*}
We can remove the summation over $(m',n',p')$ in \eqref{DD'} because of $\delta_{m,m'}$, $\delta_{n,n'}$, $\delta_{p,p'}$ that exist in \eqref{G'.2.2.2}, \eqref{H.2.2.2} and \eqref{X2}. We therefore have
\eqlab{D.hat'.alt}
{
&\hat{D}=\Big[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot\Big( R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\Big]+\nonumber\\&
\Big[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n,m)\nonumber\\&\cdot\Big( 
R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Big]+\nonumber\\&
\Big[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&
R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{y},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big].
}
Since the single period of channel $h$ signal ${\boldsymbol{p}}_h(t)$ introduced in (\ref{PeriodicSignal_x}) and \eqref{PeriodicSignal_y} is chosen enough large, i.e., $f_0\rightarrow 0$, one may use in the limit continuous integral replacing discrete summation as
\eqlab{rim}
{
\lim_{f_0\rightarrow0}f_0\sum_{m}\Lambda(mf_0)=\int\text{d}f \Lambda(f).
}
Considering \eqref{PowerX/Y} and using the fact that $\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)=\varsigma_{\kappa_2,\kappa_1,\kappa}(p,n,m)$, we can rewrite \eqref{D.hat'.alt} in the continuous domain as
\eqlab{D.hat'.alt.continuous}
{
&\hat{D}=3\times\Big[\int_{-R/2}^{R/2}\text{d}f'\delta\big(f-f'-(\kappa-l)R\big)\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f'+f_2,f_2)|^2\nonumber\\&\cdot\Big( R|S(f_1)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}R|S(f_1-f'+f_2)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(f_2)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\Big].
}
Using the delta function property $A(f)\delta(f-f_0)=A(f_0)\delta(f-f_0)$, we get \eqref{D.bar.alt.continuous.delta}.
We can write \eqref{EE'} as
\eqlab{E.hat'.alt}
{
&\hat{E}=\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&\cdot R^2f_0U_{mn'm'n}|S(pf_0)|^{2}\delta_{m-n-m'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n,m)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m,n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n',p')\nonumber\\&\cdot R^2f_0U_{mnp'n'}|S(pf_0)|^{2}\delta_{m-n-p'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{y},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&R^2f_0U_{mnm'n'}|S(pf_0)|^{2}\delta_{m-n-m'+n',0}\nonumber\\&\Big[\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\Big]\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg].
}

Considering \eqref{PowerX/Y} and using the fact that $\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)=\varsigma_{\kappa_2,\kappa_1,\kappa}(p,n,m)$, %and Letting $f_0\rightarrow 0$, \eqref{E.hat'.alt} is expressed as
we get
\eqlab{E.hat'.alt.integral.form}
{
&\hat{E}=\Bigg[\Big(3f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\nonumber\\&+\Big(2f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&\cdot R^2f_0U_{mn'm'n}|S(pf_0)|^{2}\delta_{m-n-m'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m,n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n',p')\nonumber\\&\cdot R^2f_0U_{mnp'n'}|S(pf_0)|^2\delta_{m-n-p'+n',0}\nonumber\\&\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg].
}
Letting $f_0\rightarrow 0$, we get
\eqlab{E.hat'.alt.integral.form2}
{
&\hat{E}=\Bigg[\Big(3\times\Big[\frac{P_{\kappa_1}}{2}\cdot \frac{P_{\kappa_1+\kappa_2-\kappa+l}}{2}\cdot \frac{P_{\kappa_2}}{2}\cdot R^3\int_{-R/2}^{R/2}\text{d}f_1\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_2\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+f_2+(\kappa-l)R,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+f_2+(\kappa-l)R)|^{2}|S(f_2)|^{2}
\Big]
    \Big)\nonumber\\&+\Bigg[\Big(2\times\frac{P_{\kappa_1}^2}{4}\cdot\frac{P_{\kappa_2}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_1'\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot S(f_1)S(f_1-f+(\kappa-l)R+f_2)^*S(f_1')^*\nonumber\\&\cdot S(f_1'-f+(\kappa-l)R+f_2)|S(f_2)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&
\Big(\frac{P_{\kappa_1}^2}{4}\frac{P_{\kappa_2}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(f_2,f_2-f+(\kappa-l)R+f_2',f_2')\nonumber\\&\cdot S(f_1)S(f_1-f+(\kappa-l)R+f_2)^*S(f_2')^*\nonumber\\&\cdot S(f_2-f+(\kappa-l)R+f_2')|S(f_2)|^2\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)\Bigg],
}
and so we can write \eqref{E.hat'.alt.integral.form2} as \eqref{E.bar.alt.integral.form3}.

We can write \eqref{FF'} as
\eqlab{F.hat'.alt}
{
&\hat{F}=\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m}\sum_{p}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}^2\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{p'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n',p')\nonumber\\&\cdot R^2f_0U_{pn'p'n}|S(mf_0)|^{2}\delta_{p-n-p'+n',0}\mathbb{E}\{|b_{x,\kappa_1}|^{2}\}\nonumber\\&\cdot\Big[\mathbb{E}\{|b_{x,\kappa_2}|^{4}\}-2\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}\Big]\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m}\sum_{p}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n,m)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}^2\{|b_{\text{x},\kappa_2}|^{2}\}
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',m)\nonumber\\&\cdot R^2f_0U_{pnm'n'}|S(mf_0)|^{2}\delta_{p-n-m'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}\Big]\cdot \mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m}\sum_{p}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}\nonumber\\&\mathbb{E}\{|b_{\text{y},\kappa_2}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}
\Bigg].
}
Considering \eqref{PowerX/Y} and using the fact that $\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)=\varsigma_{\kappa_2,\kappa_1,\kappa}(p,n,m)$, for $f_0\rightarrow 0$ we have
\eqlab{F.hat'.alt.integral.form}
{
&\hat{F}=\Bigg[3\times\Big(\frac{P_{\kappa_2}^2}{4}\cdot \frac{P_{\kappa_1}}{2}\cdot R^3 \int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+(\kappa-l)R+f_2)|^{2}|S(f_2)|^{2}
\Bigg]\nonumber\\&+\Bigg[\frac{P_{\kappa_2}^2}{4}\cdot \frac{P_{\kappa_1}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_2'\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2',f_2') \nonumber\\&\cdot S(f_2)S(f_1-f+(\kappa-l)R+f_2)^* S(f_2')^*\nonumber\\&\cdot S(f_1-f+(\kappa-l)R+f_2')|S(f_1)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{x,\kappa_2}|^{4}\}}{\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}}-2\Big]\Bigg]\nonumber\\&+
\Bigg[\frac{P_{\kappa_2}^2}{4}\frac{P_{\kappa_1}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(f_1',f_1-f+(\kappa-l)R+f_1,f_1)\nonumber\\&\cdot S(f_2)S(f_1-f+(\kappa-l)R+f_2)^*S(f_1')^*\nonumber\\&S(f_1'-f+(\kappa-l)R+f_1)|S(f_1)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}}-2\Big]\Bigg].
}
Since the second and third integral terms are the same, we can rewrite \eqref{F.hat'.alt.integral.form} as \eqref{F.bar.alt.integral.form2}.

We now deal with \eqref{GG'}, which can be expressed as
\eqlab{GG'.expansion}
{
&\hat{G}=\Bigg[\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\cdot
2R^{3}\mathbb{E}^{2}\{|b_{x,\kappa_1}|^{2}\}\nonumber\\&\cdot\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}|S(mf_0)|^2|S(pf_0)|^2|S(nf_0)|^{2}\Big)+\nonumber\\&\Big(f_0^{4}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n,p')\nonumber\\&\cdot R^2 S(mf_0)S(m'f_0)^*S(p'f_0)^*S(pf_0)|S(nf_0)|^{2}\delta_{m-m'-p'+p,0}\nonumber\\&\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2Rf_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\Big)\Bigg]\nonumber\\&+
\Bigg[f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\cdot R^3|S(mf_0)|^{2}\nonumber\\&\cdot |S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{y},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Bigg].
}
Letting $f_0\rightarrow 0$ and considering \eqref{PowerX/Y}, we get \eqref{GG'.expansion.integral}.
 
We will now express the last term, i.e., \eqref{HH'} in the continues form. Eq.~\eqref{HH'} is therefore expressed as
\eqlab{HH'.expansion}
{
&\hat{H}=\Bigg[\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\nonumber\\&\cdot
2R^{3}\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}|S(mf_0)|^2|S(nf_0)|^2|S(pf_0)|^2\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{p'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n',p')\nonumber\\&\cdot R^{2}f_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]U_{mnpm'n'p'}\nonumber\\&
\cdot4\delta_{m,m'}\delta_{p-n+n'-p',0}\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n,p')\nonumber\\&\cdot R^{2}f_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]U_{mnpm'n'p'}\nonumber\\&\cdot\delta_{n,n'}\delta_{m+p-m'-p',0})\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\sum_{p'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p') Rf_0\nonumber\\&\cdot\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}-9\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}+12\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\nonumber\\&U_{mnpm'n'p'}\delta_{m-n+p-m'+n'-p',0}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\nonumber\\&\cdot
R^3 \mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}|S(mf_0)|^2|S(nf_0)|^2|S(pf_0)|^{2}\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&\cdot Rf_0U_{mnm'n'}\delta_{m-n-m'+n',0}\Big[\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\Big]\nonumber\\&R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,p'}\Big)\Bigg].
}
Letting $f_0\rightarrow 0$ and considering \eqref{PowerX/Y}, we get
\eqlab{HH'.expansion.integral}
{
&\hat{H}=\Bigg[3\times\Big(\frac{P_{\kappa_1}^3}{8}\cdot R^{3}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\nonumber\\&\cdot
|S(f_1)|^2|S(f_1-f+(\kappa-l)R+f_2)|^2|S(f_2)|^2\Big)+\nonumber\\&4\times\Big(\cdot\frac{P_{\kappa_1}^3}{8}\cdot R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2',f_2')\nonumber\\&\cdot |S(f_1)|^2S(f_2)S(f_1-f+(\kappa-l)R+f_2)^*\nonumber\\&S(f_1-f+(\kappa-l)R+f_2')S(f_2')^*\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&\Big(\frac{P_{\kappa_1}^3}{8}\cdot R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1-f+(\kappa-l)R+f_2,f_1+f_2-f_1')\nonumber\\&\cdot |S(f_1-f+(\kappa-l)R+f_2)|^2S(f_1)S(f_1')^*\nonumber\\&S(f_2)S(f_1+f_2-f_1')^*\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&\Big(\frac{P_{\kappa_1}}{8}\cdot R\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2',f_2')\nonumber\\& S(f_1)S(f_1')^*S(f_2)S(f_2')^*S(f_1-f+(\kappa-l)R+f_2)\nonumber\\&S(f_1'-f+(\kappa-l)R+f_2')^* \nonumber\\&\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}}{\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}}-9\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}+12\Big]\Big)\Bigg]+\nonumber\\&
\Bigg[\frac{P_{\kappa_1}^3}{8}R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot S(f_1)S^*(f_1')S^*(f_1-f+(\kappa-l)R+f_2)\nonumber\\&S(f_1'-f+(\kappa-l)R+f_2)|S(f_2)|^{2}\Big[\frac{\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}}-2\Big]\Bigg].
}
Since the second integral term is the same as the last integral term, we can rewrite \eqref{HH'.expansion.integral} as \eqref{HH'.expansion.integral2}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%


Considering \eqref{G_x.noBias_Def} and using the fact that $G_{\text{NLI},\text{x},\kappa}(f)=G_{\text{NLI},\text{y},\kappa}(f)$, we find that the total NLI PSD within channel $\kappa$ is given by
\eqlab{G_x.noBias_Def.end}
{
&G_{\text{NLI},\kappa}(f)=G_{\text{NLI},\text{x},\kappa}(f)+G_{\text{NLI},\text{y},\kappa}(f)=2G_{\text{NLI},\text{x},\kappa}(f),
}
where $G_{\text{NLI},\text{x},\kappa}(f)$ was expressed in \eqref{G_x_d}. Finally, using \eqref{NLI_Power_Channel_Kappa} and \eqref{G_x.noBias_Def.end}, we get the total NLI power within channel $\kappa$, given by Theorem~\ref{main.result}.


%\begin{IEEEproof}

% \end{IEEEproof}
%As seen in this equation, the three spectral components $mf_0$, $pf_0$, and $mf_0+pf_0-if_0$ located in channels $\kappa_1$, $\kappa_2$, $\kappa_1+\kappa_2-\kappa+l$, respectively, interact with each other and produce the nonlinear interference at $if_0$. The efficiency of this non-degenerate four wave mixing (FWM), denoted by \eqref{Zeta_ENL}, is taking place among these spectral components.
%\section{Derivation of the NLI power}\label{AppendixB}
%This appendix addresses derivation of the the NLI power of a certain channel, starting from the NLI PSD on polarization x 
%\eqlab{G_x_Def}
%{
%G_{\text{\small{NLI}},\text{x},\kappa}(f)=\mathbb{E}\big\{E_{\text{NLI,x},\kappa}(f)\text{e}^{*}_{\text{NLI,x},\kappa}(f)\big\}.
%}
%\subsection{Nonlinear PSD}

%\section{why $l=l'$ in \eqref{average.autocorrelation.2.T0.infty..after.limitation}}\label{lequall'}

\section{Proof of Corollary \ref{main.result.identical}}\label{AppendixG}

If the loss of each frequency is exactly compensated for at the end of the corresponding span, we have 
\eqlab{GL}{
\prod_{s'=1}^{s-1}g_{s'}^{3/2}\cdot \sqrt{\rho(L_{s'},f_1)}
     \sqrt{\rho(L_{s'},f_1-f+f_2)}\sqrt{\rho(L_{s'},f_2)}=1,
}
and
\eqlab{GLraman}{
\prod_{s'=s}^{N}g_{s'}^{1/2}\sqrt{\rho(L_{s'},f)}=1,
}
and, hence, $\Upsilon(\cdot)$ in Table~\ref{terms.different} can be written as
\eqlab{Upsilon_mltp_idtcl}{
&\Upsilon(f_1,f_2,f)=
\sum_{s=1}^{N}\gamma_{s}\mu(f_1,f_2,f)\nonumber\\
&{\text{e}^{\imath 4\pi^{2}(f_1-f)(f_2-f)\sum_{s'=1}^{s-1}(\beta_{2,s'}L_{s'}+\pi(f_1+f_2)\beta_{3,s'}L_{s'})}}.
}
For multiple identical spans of homogeneous fiber ($\alpha_1=\ldots =\alpha_N=\alpha$, $L_{s}=\ldots =L_N= L$, $\gamma_1=\ldots =\gamma_N=\gamma$, $\beta_{2,{s'}}=\ldots =\beta_{2,N}=\beta_2$, $\beta_{3,{s'}}=\ldots =\beta_{3,N}=\beta_3$), \eqref{Upsilon_mltp_idtcl} is equal to
\eqlab{Upsilon_mltp_idtcl_2}{
&\Upsilon(f_1,f_2,f)=
\gamma\mu(f_1,f_2,f)\nonumber\\
&[1+\text{e}^{\imath 4\pi^{2}(f_1-f)(f_2-f)(\beta_{2}L+\pi(f_1+f_2)\beta_{3})L}+\nonumber\\&\text{e}^{\imath 4\pi^{2}(f_1-f)(f_2-f)(\beta_{2}L+\pi(f_1+f_2)\beta_{3})2L}+\ldots+\nonumber\\&\text{e}^{\imath 4\pi^{2}(f_1-f)(f_2-f)(\beta_{2}L+\pi(f_1+f_2)\beta_{3})(N-1)L}],
}
where using the fact that
\eqlab{Ts}{
1+\text{e}^{\imath x}+\text{e}^{2\imath x}+\cdots+\text{e}^{\imath (N_s-1)x}=&\sum_{h=0}^{N_s-1}(\text{e}^{\imath x})^{h}
=\frac{1-\text{e}^{\imath N_sx}}{1-\text{e}^{\imath x}}
%=\text{e}^{(N_s-1)\imath x/2}\frac{\sin(N_sx/2)}{\sin(x/2)},
}
\eqref{Upsilon_mltp_idtcl_2} can be written as
\eqlab{Upsilon_mltp_idtcl_final}{
&\Upsilon(f_1,f_2,f)=\gamma\mu(f_1,f_2,f)\nonumber\\&
\cdot\frac{1-\text{e}^{4\pi^{2}(f_1-f)(f_2-f)NL[\beta_2+\pi\beta_3(f_1+f_2)]}}{1-\text{e}^{4\pi^{2}(f_1-f)(f_2-f)L[\beta_2+\pi\beta_3(f_1+f_2)]}}
%\frac{\sin(2\pi^{2}(f_1-f)(f_2-f)NL[\beta_2+\pi\beta_3(f_1+f_2)])}{\sin(2\pi^{2}(f_1-f)(f_2-f)L[\beta_2+\pi\beta_3(f_1+f_2)])},
}
which is equivalent to $\Upsilon(\cdot)$ given in Table~\ref{terms.identical}. 
%\section{Relevant moments}
%To make the paper self contained, in this section we express the second, fourth and sixth order moments that are being used in . To find the detailed derivation of these moments readers are referred to \cite{carena2014accuracy}.
%\subsection{Second order moment}

%We first start with second order moment $\mathbb{E}\{\xi_{\text{x},\kappa,m}\xi_{\text{x},\kapap,n}^*\}$ which is equal to
%\eqlab{second.moment}{
%\mathbb{E}\{\xi_m\xi_n^*\}=R |S(mf_0)|^{2}\mathbb{E}\{|b|^2\}(\delta_{m-n+hW})_{W=0,\pm 1,\cdots}
%}
%where for notational convenience we dropped indices x and $\kappa$. For Nyquist rectangular spectral shape channels $h=0$ and hereafter we ignore the spectral components that are $hR$ apart.

%\subsection{Fourth order moment}

%The fourth order moment of $\xi$ is given by
%\eqlab{fourth.moment}{
%&\mathbb{E}\{\xi_m\xi_n^*\xi_{m'}^*\xi_{n'}\}=R\mathbb{E}^2\{|b|^2\}U_{mnm'n'}\big(\delta_{m,n}\delta_{n'-m'}+\nonumber\\&\delta_{m,m'}\delta_{n'-n}\big)+Rf_0\Big[\mathbb{E}\{|b|^4\}-2\mathbb{E}^{2}\{|b|^2\}\Big]U_{mnm'n'}\nonumber\\&\delta_{m-n-m'+n',0}
%}

%\subsection{Sixth order moment}

%The sixth order moment of $\xi$ is equal to
%\eqlab{sixth.moment}{
%&\mathbb{E}\{\xi_m\xi_n^*\xi_{k}\xi_{m'}^*\xi_{n'}\xi_{l}^*\}=Rf_0^2\mathbb{E}^3\{|b|^2\}\Big[\mathbb{E}\{|b|^6\}/\mathbb{E}^3\{|b|^2\}\nonumber\\&-9\mathbb{E}\{|b|^4\}/\mathbb{E}^2\{|b|^2\}+12\Big]U_{mnkm'n'l}\delta_{m-n+p-m'+n'-l}\nonumber\\&Rf_0^2\mathbb{E}^3
%\{|b|^2\}\Big[\mathbb{E}\{|b|^4\}/\mathbb{E}^2\{|b|^2\}-2\Big]U_{mnkm'n'l}\nonumber\\&\delta_{m-n+p-m'+n'-l}\Big(\delta_{m,n}\delta_{k-m'+n'_l}+\delta_{m,m'}\delta_{p-n+n'-l}+\nonumber\\&\delta_{m-n'}\delta_{p-n-m'+n',0}+\delta_{p-n}\delta_{m-m'+n'-l}+\delta_{k-m'}\delta_{m-n+n'-l}\nonumber\\&+\delta_{k-l}\delta_{m-n-m'+n',0}+\delta_{n,n'}\delta_{m+p-m'-l}\nonumber\\&+\delta_{n'-m'}\delta_{m-n+p-l}+\delta_{n'-l}\delta_{m-n+p-m'}\Big)+R^2\mathbb{E}^3\{|b|^2\}\nonumber\\&U_{mnkm'n'l}\Big(\delta_{m,n}\delta_{k-m'}\delta_{n'-l}+\delta_{m,n}\delta_{k-l}\delta_{n'-m'}+\nonumber\\&
%\delta_{m,m'}\delta_{p-n}\delta_{n'-l}+\delta_{m,m'}\delta_{k-l}\delta_{n'-n}+\nonumber\\&\delta_{m-l}\delta_{p-n}\delta_{n'-m'}+\delta_{m-l}\delta_{k-m'}\delta_{n'-n}\Big).
%}

\begin{figure*}[!t]
\pgfplotsset{compat=1.3}
\begin{center}
\begin{tikzpicture}[x=0.2cm,y=0.2cm,scale=1]
\begin{groupplot}[group style={
group name=my plots, group size=2 by 1,horizontal sep=1.15cm,vertical sep=8.5pt},
%set layers=axis on top,
 %            axis line style={line width=1.5pt},
  %           every axis plot post/.append style={line width=1.5pt},
legend columns=1,
legend entries={{PM-QPSK}, Optimized 16-point \cite{Magnus.4d.2010}, SO-PM-QPSK \cite{Sjodin2013}},   
%legend to name=Fig1,
grid,
 grid style = {
    dash pattern = on 0.05mm off 1mm,
    line cap = round,
    black,
    line width = 0.2mm
  },
 ylabel style={yshift=-0.15cm},
%axis y line*=left,
%axis x line*=bottom,
width=9.5cm,height=8.5cm]

\nextgroupplot
[
%legend to name=benchmarkfigc1,
%xticklabels={},
% ylabel={$\eta_\kappa \ [\text{dB} \ W^{-2}]$},
%grid=major,
ymin=36,ymax=40, 
xmin=1,xmax=80,
title=(a),
xlabel=Channel Number $n$, 
legend style={at={(0.502,0.135)},anchor=west,font=\footnotesize},
%title=With SRS,
ylabel={$\eta_n$ [$\text{dB} \ W^{-2}$]},
%axis y line*=left,
%axis x line*=bottom,
%yticklabels={,,}
%($P_{\text{tot}}=25$ dBm),
%legend enteries={no SRS, $19$ dBm, $23$ dBm, $25$ dBm, $27.5$ dBm, $27.5$ dBm \cite{Semrau2019jlt}},
%legend to name=benchmarkfigc,
%xticklabels={},
%ymax=26,ytick={16,18,20,22,24,26,28},yticklabels={
%$16$,
%$18$,
%$20$, 
%$22$, 
%$24$, 
%$26$,
%$28$,  
%}, 
]

%\addplot [red, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_MAGNUSOptimized16_5span.dat};
\addplot [red, line width=0.2mm, solid, mark=triangle, mark repeat=8]table[x index=0,y index=1] {Dat/Total_NLI_sim5.dat};

\addplot [red, line width=0.2mm, solid, mark=square, mark repeat=15]table[x index=0,y index=1] {Dat/Total_NLI_biortho4_8.dat};%=c4_8,L4_8

\addplot [blue, line width=0.5mm, solid, mark=diamond, mark repeat=15]table[x index=0,y index=1] {Dat/Total_NLI_tetra4_9.dat};

\addplot [purple, line width=0.5mm, solid, mark=diamond, mark repeat=15]table[x index=0,y index=1] {Dat/Total_NLI_spm4_128.dat};

\addplot [green, line width=0.5mm, solid, mark=diamond, mark repeat=15]table[x index=0,y index=1] {Dat/Total_NLI_cross4_512.dat};

\addplot [brown, line width=0.5mm, solid, mark=diamond, mark repeat=15]table[x index=0,y index=1] {Dat/Total_NLI_l4_25.dat};%c4_25

\addplot [black, line width=0.5mm, solid, mark=diamond, mark repeat=15]table[x index=0,y index=1] {Dat/Total_NLI_b4_64.dat};%c4_25

\addplot [orange, line width=0.5mm, solid, mark=diamond, mark repeat=15]table[x index=0,y index=1] {Dat/Total_NLI_b4_4096.dat};%c4_25

%\addplot [blue, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_16point_10span.dat};

%\addplot [green, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_PMQPSK_5span.dat};



%\addplot [brown, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_SOPMQPSK_5span.dat};

%\addplot [green, line width=0.5mm, dotted]table[x index=0,y index=1] {Dat/Total_NLI_SOPMQPSK_10span.dat};
%\addplot [blue, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_ps_qpsk__wdm_plot_50span_spacing_50ghz.dat};
%\addplot [green, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_64bin__wdm_plot_10span_spacing_50ghz.dat};

%\addplot [purple, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_64bin__wdm_plot_50span_spacing_50ghz.dat};

%\addplot [black, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_pm64__wdm_plot_10span_spacing_50ghz.dat};
%\addlegendentry{PM-16QAM (analytical \cite{Semrau2019jlt})}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot
[
%legend to name=benchmarkfigc1,
%xticklabels={},
% ylabel={$\eta_\kappa \ [\text{dB} \ W^{-2}]$},
%grid=major,
ymin=3,ymax=18, 
xmin=1,xmax=41,
title=(b),
xlabel={Launch Power [dBm]}, 
legend style={at={(.502,0.215)},anchor=west,font=\footnotesize},
%title=With SRS,
ylabel={$\text{SNR}_{40}$ [dB]},
%axis y line*=left,
%axis x line*=bottom,
%yticklabels={,,}
%($P_{\text{tot}}=25$ dBm),
%legend enteries={no SRS, $19$ dBm, $23$ dBm, $25$ dBm, $27.5$ dBm, $27.5$ dBm \cite{Semrau2019jlt}},
%legend to name=benchmarkfigc,
%xticklabels={},
%ymax=26,
xtick={1,6,11,16,21,26,31,36,41},xticklabels={
$-15$,
$-12.5$,
$-10$,
$-7.5$,
$-5$,
$-2.5$,
$0$, 
$2.5$,
$5$, 
%$26$,
%$28$,  
}, 
]

%\addplot [red, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_MAGNUSOptimized16_5span.dat};
\addplot [red, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/SNR_PMQPSK.dat};

\addplot [blue, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/SNR_16point.dat};

%\addplot [green, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_PMQPSK_5span.dat};



%\addplot [brown, line width=0.5mm, solid]table[x index=0,y index=1] {Dat/Total_NLI_SOPMQPSK_5span.dat};

\addplot [green, line width=0.5mm, dotted]table[x index=0,y index=1] {Dat/SNR_SOPMQPSK.dat};


%\addplot [blue, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_ps_qpsk__wdm_plot_50span_spacing_50ghz.dat};
%\addplot [green, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_64bin__wdm_plot_10span_spacing_50ghz.dat};

%\addplot [purple, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_64bin__wdm_plot_50span_spacing_50ghz.dat};

%\addplot [black, line width=0.5mm, dashed]table[x index=0,y index=1] {Dat/NLIN_var_pm64__wdm_plot_10span_spacing_50ghz.dat};
%\addlegendentry{PM-16QAM (analytical \cite{Semrau2019jlt})}













\end{groupplot}
%\draw[->,>=stealth,thick] (60.5-18.5-22.5,20.5-6.8) -- (60.5-18.5-22.5,26-2.8);
%\node at (58-18.75-22.5,23-5.3+1.7) {\footnotesize{$1.68$ dB}};

%\draw[->,>=stealth,thick] (61.5,20.5) -- (61.5,31.5);
%\node at (58+6.15,29) {\footnotesize{$2.5$ dB}};
%\draw[->,>=stealth,thick] (43-22.5,17.65-3.9) -- (43-22.5,19.7-4);
%\node at (45-22.5,11.5) {\footnotesize{$0.4$ dB}};
%\draw [->] (43-22.5,14.5) arc (90:-10:10pt);
\end{tikzpicture}
%\\
%\vspace*{7pt}
%\ref{Fig1}
\end{center}
\setlength{\belowcaptionskip}{-12pt}
\vspace*{-5mm}
\caption{(a) illustrates $\eta_n$  as a function of channel number $n$ after 10 spans for PM-QPSK, SO-PM-QPSK, and optimized 16-point modulation formats and (b) illustrates the SNR of the channel located in the middle of spectrum, i.e.,  $\text{SNR}_{40}$, as a function of launch power after 10 spans for the same formats.
%SSFM simulations are represented by circle markers and numerical results using \textit{Corollary }\ref{main.result.identical} are represented by solid lines.
} 
\label{nlc_fig4}
\end{figure*}
